DiSCoMaT: Distantly Supervised Composition Extraction from Tables in Materials Science Articles

A crucial component in the curation of KB for a scientific domain (e.g., materials science, foods & nutrition, fuels) is information extraction from tables in the domain's published research articles. To facilitate research in this direction, we define a novel NLP task of extracting compositions of materials (e.g., glasses) from tables in materials science papers. The task involves solving several challenges in concert, such as tables that mention compositions have highly varying structures; text in captions and full paper needs to be incorporated along with data in tables; and regular languages for numbers, chemical compounds and composition expressions must be integrated into the model. We release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present a strong baseline DISCOMAT, that combines multiple graph neural networks with several task-specific regular expressions, features, and constraints. We show that DISCOMAT outperforms recent table processing architectures by significant margins.

==> sections/8_1_acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:checklist}

% This document has been adapted
% by Steven Bethard, Ryan Cotterell and Rui Yan
% from the instructions for earlier ACL and NAACL proceedings, including those for 
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan, 
% NAACL 2017 by Margaret Mitchell, 
% ACL 2012 by Maggie Li and Michael White, 
% ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
% ACL 2002 by Eugene Charniak and Dekang Lin, 
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections_old/0_abstract.tex <==
%Tables in scientific articles carry important information (often numeric), which must be adequately extracted for a comprehensive machine understanding of an article. Our paper studies information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction.  Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also develop \sys, a strong baseline for the task, which combines graph neural networks with several problem-specific regular expressions, features and constraints. Our experiments evaluate the contribution of each model component in the final performance. We release our code and data for further research.
A crucial component in the curation of KB for a scientific domain is information extraction from tables in the domain's published articles  -- tables carry important information (often numeric), which must be adequately extracted for a comprehensive machine understanding of an article. Existing table extractors assume prior knowledge of table structure and format, which may not be known in scientific tables. We study a specific and challenging table extraction problem: extracting compositions of materials (e.g., glasses, alloys). We first observe that materials science researchers organize similar compositions in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction. Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present \sys, a strong baseline geared towards this specific task, which combines multiple graph neural networks with several task-specific regular expressions, features, and constraints. We show that \sys{} outperforms recent table processing architectures by significant margins. 
%Our experiments also assess the value of additional modifications on the final performance of the model. 
We release our code and data for further research.

%Most of the work on table extraction assumes prior knowledge on the table structure and format---a scenario that may not hold true for tables from scientific literature. A generic framework that can mine information from tables is crucial for the development of knowledge bases in several engineering and scientific domains. To address this challenge, we take a holistic view on information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction. Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present a strong baseline for the task, \sys, which combines graph neural networks with several problem-specific regular expressions, features, and constraints. We show that \sys outperforms other existing models. Our experiments also evaluate how additional modifications can enhance the final performance of the model. We release our code and data for further research.

%-- progress on the task will hopefully lead to the construction of a large repository of materials (and subsequently their properties) known to mankind.

%Vast amount of Materials Science-specific information like compositions and properties is stored in tables, images and text of research publications. Since property extraction can only be performed after composition extraction, we focus on extracting compositions from tables.
% missing motivation to extract compositions from tables instead of text
%This paper is a first attempt to solve this problem and no annotated datasets are publicly available.
%First, we formally define a new problem to the ML community.
%Second, to motivate the problem, we perform extensive analysis of the ways in which compositions are reported and highlight various facets of the problem.
%Third, we share a dataset comprising of 4408 distantly supervised training tables, along with 738 and 737 manually annotated dev and test tables respectively.
%Fourth, we propose a strong baseline model based on Graph Attention Networks (GATs) \cite{velickovic2018graph} and MatSciBERT \cite{gupta_matscibert_2022} (pre-trained BERT-based Language Model).
% can mention results, bert based based baseline
%\footnote{Code and data are available at: \url{https://github.com/}.}
%\end{comment}

==> sections_old/1_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\label{sec:intro}

Advanced knowledge of a science or engineering domain is typically found in published research papers from that domain. Information extraction (IE) from scientific articles develops ML methods to automatically extract this knowledge for curating large-scale  domain-specific KBs (e.g., \cite{ernst-bmc15,hope-naacl21}). These KBs have a variety of uses: they lead to ease of information access by domain researchers \cite{tsatsaronis-bmc15,hamon-sw17}, provide data for development of domain-specific ML models \cite{nadkarni-akbc21}, and potentially help in accelerating scientific discoveries \cite{materials_project, challenges_21}. Significant research exists on IE from text of research papers (see \cite{nasar-scientometrics18} for survey), but less attention is given to extracting information (often, numeric) conveyed in tables. Tables may express performance of an algorithm on a dataset, report quantitative results of clinical trials, or describe compositions and properties of  materials studied in a paper. Due to the importance of such information, we posit that IE from tables is essential for a comprehensive machine understanding of a given paper, and for increasing the coverage of resulting KBs.

Tables of specific interest are the ones which mention the composition and properties of an entity. Such tables are ubiquitous in various fields of physics, chemistry, materials, and biology and form the cornerstone of the scientific discovery elucidated in the paper. Further, the extraction of these compositions, often ranging to millions in a specific sub-field, is a tedious and time-consuming task. Therefore, we are motivated to curate a KB of all materials known to mankind (such as glasses, alloys), along with their properties. A preliminary analysis of materials science (MatSci) papers reveals that around 85\% of material compositions and their associated quantitative properties (e.g., hardness, viscosity, conductivity) are reported in tables. Our paper studies the first part of this IE problem -- extraction of materials (IDs used in the paper), along with their constituents and relative percentages. For instance, Fig. \ref{fig:three comp_tables}a should output four materials (A1-A4), where ID A1 is associated with three constituents (MoO$_3$, Fe$_2$O$_3$, and P$_2$O$_5$) and their percentages, 5, 38, and 57, respectively. While not our focus, this extraction problem is also relevant for several other domains such as biomedical (drug compositions), environmental science (aerosols, air pollution, solid waste), and chemistry (polymers, colloids).

% \begin{figure}[t]
% \begin{center}
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{multi_cell_comp_table_1_S0022309303003624.png}
%         \label{fig:multi_cell_comp_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{\scriptsize Glass compositions in the paper: $20La_2S_3-(80 - x)Ga_2S_3-xCsCl$.}
%         \includegraphics[width=\textwidth]{partial_info_table_1_S0022309399000617.png}
%         \label{fig:partial_info_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{single_cell_S0022459614003995.png}
%         \label{fig:single_cell_comp_table}
%     \end{subfigure}
%     \vspace{-0.3cm}
%     \caption{\small Examples of composition tables (a) Multi-cell complete-info composition table (b) Multi-cell partial-info composition table (c) Single-cell composition table }
%     \label{fig:three comp_tables}
%     \vspace{-0.6cm}
% \end{center}
% \end{figure}

\begin{figure*}[t]
\begin{center}
    \centering
    \includegraphics[width=\textwidth]{figure_1.png}
    \caption{Examples of composition tables (a) Multi-cell complete-info composition table \cite{fig_1a_mcc_all} (b) Multi-cell partial-info composition table \cite{fig_1b_mcc_pi} (c) Single-cell composition table \cite{fig_1c_scc}}
    \label{fig:three comp_tables}
    \vspace{-0.6cm}
\end{center}
\end{figure*}

Our preliminary analysis of composition tables reveals that MatSci researchers express compositions in a wide-variety of table styles. Two main types are \emph{multi-cell compositions} (MCC), where material composition and constituents are on two axes %\todo{T: constituents are not always on the same axes. M: how will you describe differently. T: all constituents and their contribution are in table} 
and each cell represents the percentage (Fig.~\ref{fig:three comp_tables}a), and \emph{single-cell compositions} (SCC), where the full composition is mentioned in a single cell as an expression (see Fig.~\ref{fig:three comp_tables}c). However, there are several other types -- sometimes, the table has incomplete information and other default constituents are listed in caption or text (Fig.~\ref{fig:three comp_tables}b). Additionally, there can be four units for specifying the percentage -- mol \%, mol fraction, weight \% or weight fraction, requiring normalization (see App.~\ref{sec:problem} for detailed discussion on challenges in composition extraction from tables). %Interestingly, some researchers write percentages such that they add to numbers less than or more than 100, and expect the reader to re-normalize. 
All these and more make the problem of extracting material compositions from scientific tables a challenging problem. 
 \vspace{-1ex}

In response, we first harvest a distantly supervised training dataset. Existing table processing literature is not well-suited for our task, because it generally assumes prior knowledge of table structure and format, understanding which, as described above, is a key challenge for our task. In response, our baseline system \sys\ uses a pipeline of a domain-specific language model \cite{gupta_matscibert_2022}, and two graph neural networks (GNNs), along with several hand-coded features and constraints. We evaluate our system on accuracy metrics for various subtasks, including ID prediction, tuple-level prediction, material-level complete prediction. 
We find that \sys\ with constraints and features obtains upto 14 point  increase in various accuracy numbers, compared to a model that uses vanilla GNNs. Our GNN-based architecture outperforms a recent table processor, which linearizes the table for prediction by a language model \cite{herzig-etal-2020-tapas}, by a wide margin. 
Subsequent analysis reveals common sources of \sys\ errors, which will inform future research.
We release all our data and code for further research on the challenge task.

% pleas use these short forms in the paper
%\begin{table}
 %   \centering
  %  \begin{tabular}{ll} 
   %     \toprule
    %    Table Type & Meaning \\
     %   \midrule
      %  SCC table & Single-cell composition table \\
       % MCC-CI table & Multi-cell composition complete-info table \\
       % MCC-PI table & Multi-cell composition partial-info table \\
       % NC table & Non-composition table \\
    %    \bottomrule
    %\end{tabular}
%\end{table}


==> sections_old/2_related_work.tex <==
% !TEX root = main.tex
\section{Related work} 
\label{sec:related_work}
%Information extraction (IE) is instrumental for knowledge base creation. 
%While most of the earlier works on information extraction (IE) focusses on rule-based approaches \cite{chiticariu-etal-2013-rule}, large datasets, computational efficiency, and success of neural models lead to machine learning-based IE systems\cite{chiticariu-etal-2013-rule}.


Recent work has developed neural models for various NLP tasks based on tabular data, for instance, tabular natural language inference \cite{tnli_orihuela2021natural, xinfotabs}, QA over one or a corpus of tables \cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr, chemmengath-emnlp21}, table orientation classification\cite{deeptable_habibi2020,nishida2017understanding}, and relation extraction from tables \cite{relation_ex_tables_2013, neurel_relex_2}.
Several papers study QA models. For instance, 
\textsc{TaPas} \cite{herzig-etal-2020-tapas} linearizes a table and passes it to a BERT-based model pre-trained on Wikipedia tables -- it answers natural language (NL) questions over tables by selecting table cells and aggregation operators. \textsc{TaBERT} \cite{yin-etal-2020-tabert} uses a different pre-training objective and model architecture to jointly learn NL sentence and table representations. Row and column intersection (RCI) model \cite{feifei_row_col_interact} predicts the probability of finding the answer to a given question in each row and column of a table independently, without any pre-training on tables. \textsc{TaPEx} \cite{tapex} uses a BART encoder-decoder architecture, pre-trained via synthetic executable programs to mimic the behaviour of SQL execution engine. \textsc{TABBIE} \cite{tabbie} consists of two transformers that encode rows and columns independently and is pre-trained using the corrupt-cell objective. 
%TABBIE performs better than other models on table-based tasks such as column type prediction. 
Similar to our work, tables have also been modeled as graphs for sequential question answering over tables \cite{muller_acq_2019}. However, all these works generally assume a fixed and known structure of tables with the same orientation, with the top row being the header row in all cases -- an assumption violated in our setting. 
%The table orientation and header row are assumed to be fixed for this problem. 

{\bf Orientation and semantic structure classification:} %of tables has also been attempted using neural models. 
DeepTable \cite{deeptable_habibi2020} is a permutation-invariant neural model, which classifies tables into three orientations, while TabNet \cite{nishida2017understanding} uses RNNs and CNNs in a hybrid fashion to classify web tables into five different types of orientations. InfoTabS \cite{infotabs}  studies natural language inference on tabular data. Here, concatenated premise-hypothesis pair is sent through language models to classify whether the premise (info-box) entails, contradicts, or is unrelated to a given hypothesis. 
%However, these info-boxes are special type of tables containing two columns: first containing keys and other containing values. 
This has been extended to the multilingual setting \cite{xinfotabs}, and has been combined with knowledge graphs \cite{transkblstm}. 
%Extending this, Minhas et al. \cite{xinfotabs} released a multilingual TNLI dataset comprising of info-boxes from ten different languages.  Further, TransKBLSTM model was proposed by Varun et al. \cite{transkblstm} to augment TNLI models with knowledge graphs. 
Some earlier works also focused on annotating column types, cells with entity IDs, pair of columns with binary relations, based on rule-based and other ML approaches, given a catalog consisting of types, entities and relations \cite{sunita_iitb}.


%There has also been work on annotating column types, cells with entity IDs, pair of columns with binary relations, etc given a catalog consisting of types, entities and relations \cite{sunita_iitb}. But again in this work, they take simple tables with fixed header and no merged rows or columns. 

%But their graph structure is different than ours as the table orientation and header row is fixed for their dataset.

%Distant Supervision, proposed by Mintz et al. \cite{mintz-etal-2009-distant}, is an approach to create a noisy dataset and does not require labelled data. This method is generally used to annotate any given sentence with the relations it might express. In our work, we use a similar approach where we use the Interglad database to annotate our training set.

%{\bf NLP for materials literature:} After the success of BERT \cite{devlin2018bert}, numerous domain-specific language models have been released for  public-use. For MatSci domain, researchers have contributed language models like MatSciBERT \cite{gupta_matscibert_2022}, MatBERT \cite{matbert_2022}, and BatteryBERT \cite{batterybert_2022}. MatBERT \cite{matbert_2022} highlights the advantages of materials domain-specific pre-training on the NER task. BatteryBERT  exhibits superior performance on battery related downstream tasks. MatSciBERT  yields state of the art performance on downstream tasks of abstract classification, NER, and relation classification, and we use it in our work. Wang et al. \cite{wang_automated_2022} recently develop a rule-based NER and relation extraction to create a pipeline for extracting superalloy data from text and tables. There also exists a table extraction tool that takes input HTML or XML of MatSci research papers, and uses regular expression based parser for extracting compositions, scientific units, and related information \cite{mit_table_parser}. However, the regexs used in these works are highly specific and will require significant modifications for different classes of materials.  Despite the availability of MatSci language models, deep neural models have not been explored for IE from materials tables -- the focus of this work.


% Information extraction (IE) is instrumental for knowledge base creation. The transition from rule based IE systems to machine learning IE systems became possible due to availability of large datasets and computational efficiency\cite{chiticariu-etal-2013-rule}. IE from text and tabular data has witnessed tools like WOE\cite{wu-weld-2010-open}, ReVerb\cite{ReVerb2011}, OLLIE\cite{mausam-etal-2012-open}, TaPaS\cite{herzig-etal-2020-tapas}, TaBERT \cite{yin-etal-2020-tabert}, and TabNet\cite{tabnet_Arik_Pfister_2021} to name a few. Specifically, neural models capable of semantically parsing tabular information are jointly pre-trained over natural language queries and structured and semi-structured tables\cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr}. 
% Information extraction from MS literature is an emerging field because accurately creating, maintaining, and updating material compositions and property databases is a humanly difficult task. Researchers have developed specialised tools for extracting information like extracting inorganic material synthesis routes using word embedding, named entity recognition a\cite{kim_we_ner_cvae, kim_virtual_2017}, and generating database of Curie and Néel temperatures by using a combination of text parsing, table parsing, relation extraction on XMLs and HTMLs of relevant scientific documents\cite{court_auto-generated_2018}, and rule based NER and relation extraction for creating superalloys database\cite{wang_automated_2022}.

% For IE from MS tables, researchers have developed a table extraction tool which takes input of HTML or XML of material science research papers, and uses regex based parser for extracting compositions, scientific units, and related information\cite{mit_table_parser}. This tool was used to extract data related to zeolites\cite{mit_table_parser}, cementitious materials\cite{mit_cement_uvegi}, and aluminum alloys\cite{elsa_aluminium}. ChemDataExtractor is another tool which is capable of extracting complete chemical compositions, but, only from the full information tables present in research papers\cite{chemdataextractor_v1,chemdataextractor_v2}. However, these existing tools are quite specific and can not understand the different structures of MS tables posing special challenges in information extraction as discussed in section 2.1. 

% Recently, researchers have developed materials science language models like MatSciBERT\cite{gupta_matscibert_2022}, MatBERT\cite{matbert_2022}, and BatteryBERT\cite{batterybert_2022}. MatSciBERT\cite{gupta_matscibert_2022} yielded state of the art performance on downstream tasks of abstract classification, named entity recognition, and relation classification, MatBERT\cite{matbert_2022} authors achieved state of the art results on NER tasks, and BatteryBERT\cite{batterybert_2022} was used to enhance battery materials database by LM based question answering downstream task.


==> sections_old/3_problem_defn.tex <==
% !TEX root = main.tex
\section{Challenges in composition extraction from tables} 
\label{sec:problem}

% \begin{figure}[!htb]
% \begin{center}
%     \centering
%     \includegraphics[scale=0.6]{multi_cell_comp_table_1_S0022309303003624.png}
%     \caption{Example of a composition table found in MS research papers}
%     \label{fig:multi_cell_comp_table_1}
% \end{center}
% \end{figure}

%Figure \ref{fig:multi_cell_comp_table_1} shows cropped version of a composition table taken from \cite{mogus-milankovic_spectroscopic_2003}. First column contains the material IDs such as F40, A1, A2, etc. This is followed by compounds such as Mo$O_3$, Fe$_2$O$_3$, SrO and P$_2$O$_5$, which form the individual components of the material composition mentioned. The composition can be expressed as $n$-tuples consisting of {(material ID), (component name), (percentage of the component present in the composition)}. For example, a glass composition A1 from Figure \ref{fig:multi_cell_comp_table_1} can represented as $\{(A1, MoO_3, 5, mol), (A1, Fe_2O_3, 38, mol), (A1, P_2O_5, 57, mol)\}$.

%\subsection{Challenges}
We analyze numerous composition tables in  MatSci research papers (see Figures \ref{fig:three comp_tables}, \ref{fig:regex_var_comp_table} and \ref{fig:two_comp_tables_2} for examples), and find that the task has several facets, with many table styles for similar compositions. We now describe the key challenges involved in the task of composition extraction from tables.
\begin{enumerate}[topsep=0pt,itemsep=-0.5ex,partopsep=0ex,parsep=0.8ex]
    \item \textbf{Distractor rows and columns}: Additional information such as material properties, molar ratios, std errors in the same table. E.g., Figure \ref{fig:three comp_tables}a, last three rows are distractor rows. % For a non-composition table, all rows and columns are distractor rows and columns.

    \item \textbf{Orientation of tables}: Table shown in Figure \ref{fig:two_comp_tables_2}a is a row oriented table---different compositions are written in different rows. Table in Figure \ref{fig:three comp_tables}a is a column oriented table.
    
    \item \textbf{Different units}: Compositions can be in different units such as mol\%, weight\%,  mol fraction, weight fraction. Some tables express a composition in both molar and mass units.
    
    \item \textbf{Material IDs}: Authors refer to different materials in their publication by assigning them unique IDs. These material IDs may not be specified every time, (e.g., Fig.~\ref{fig:three comp_tables}c). % ID extraction is essential for linking between text (or other tables) and composition tables.
    
    \item \textbf{Single-cell compositions (SCC)}: In Fig.~\ref{fig:three comp_tables}a, all compositions are present in multiple table cells. Some authors report the entire composition in single table cell, as shown in Fig. \ref{fig:three comp_tables}c.
    
    \item \textbf{Percentages exceeding 100:} Sum of coefficients may exceed 100, and re-normalization is needed. A common case is when a dopant is used; its amount is reported in excess.
    
    \item \textbf{Percentages as variables}: Contributions of constituents may be expressed using variables like $x, y$. In figure \ref{fig:regex_var_comp_table}, x represents the mol\% of (GeBr$_4$) and the 2$^{\rm{nd}}$ row contains its value.
    %that $x$ can take for each of these cases.
    
    \item \textbf{Partial-information tables}: It is also common to have percentages of only some constituents in the table; the remaining composition is to be inferred based on paper text or table caption,  
    e.g., Figure \ref{fig:three comp_tables}b. Another example: if the paper is on silicate glasses, then SiO$_2$ is assumed.
    
    \item \textbf{Other corner cases}: There are several other corner cases like percentages missing from the table, compounds with variables (e.g., R$_2$O in header; value of R to be inferred from material ID), and highly unusual placement of information (some examples in appendix). 
    
%    \item \textbf{Nominal and experimental}: Sometimes during sample preparation, the expected/nominal composition of a material changes. Therefore, it is not infrequent to report two compositions for one sample like in figure \ref{fig:nom_exp_table}, where EDS (experiment) is used to measure the actual composition.
    
\end{enumerate}

% \begin{wrapfigure}{r}{0.4\textwidth}
%     \vspace{-8.5ex}
%     \centering
%     \includegraphics[width=0.4\textwidth, height=3cm]{regex_var_S0022309301007906.png}
%     \caption{Percentages as variables \cite{fig_2_regex}}
%     \label{fig:regex_var_comp_table}
%     \vspace{-4ex}
% \end{wrapfigure}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.35\textwidth, height=2.5cm]{regex_var_S0022309301007906.png}
    \caption{Percentages as variables \cite{fig_2_regex}}
    \label{fig:regex_var_comp_table}
    \vspace{-2ex}
\end{figure}

% \begin{figure}[!htb]
% \begin{center}
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{regex_var_S0022309301007906.png}
%         \label{fig:regex_var_comp_table}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.5\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{nom_exp_S0022309306011677.png}
%         \label{fig:nom_exp_table}
%     \end{subfigure}
%     \vspace{-0.3cm}
%     \caption{\small (a) Composition table with percentages expressed using a variable (b) Composition table having both nominal and experimental compositions}
%     \label{fig:two_comp_tables}
%     \vspace{-0.6cm}
% \end{center}
% \end{figure}


==> sections_old/4_model.tex <==
% !TEX root = main.tex
\section{\sys\ architecture} 
\label{sec:model}

To address automated extraction of material compositions from tables, we present an ML formulation of the problem.  Formally, given a table $T$, its caption, and the complete text of publication in which $T$ occurs, we aim to extract compositions expressed in $T$, in the form $\{(id, c_k^{id}, p_k^{id}, u_k^{id} )\}_{k=1}^{K^{id}}$. Here, $id$ represents the material ID, as defined in the paper. Material IDs are defined by MatSci researchers to succinctly refer to that composition in text and other tables. $c_k^{id}$ is a constituent element or compound present in the material, $K^{id}$ is the total number of constituents in the material, $p_k^{id} > 0$ denotes the percentage contribution of $c_k^{id}$ in its composition, and $u_k^{id}$ is the unit of $p_k^{id}$ (either mole\% or weight\%).

% \begin{wrapfigure}{l}{0.55\textwidth}
%     \vspace{-3ex}
%     \centering
%     \includegraphics[width=0.55\textwidth, height=4cm]{flowchart.png}
%     \caption{The design of \sys}
%     \label{fig:comp_table_cls}
%     \vspace{-1ex}
% \end{wrapfigure}
\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.45\textwidth, height=3cm]{flowchart.png}
    \caption{The design of \sys}
    \label{fig:comp_table_cls}
    \vspace{-1ex}
\end{figure}

Figure \ref{fig:comp_table_cls} illustrates the basic pipeline for extraction in \sys. We find that the simplest task is to identify whether the table $T$ is an SCC table, owing to a distinctive presence of multiple numbers, and compounds in single cells. \sys{} first runs a GNN-based SCC predictor, which classifies $T$ as an SCC table or not. For SCC table, it uses a standalone rule-based composition parser. For the other category, \sys{} runs a second GNN (GNN$_2$), and first labels rows and columns of $T$ as compositions, material IDs,  constituents, and others. If no constituents or composition predictions are found, then $T$ is deemed to be a non-composition (NC) table. Or else, it is an MCC table, for which \sys{} predicts whether it has all information in $T$ or some information is missing (partial-information predictor). If it is complete information table, then GNN$_2$'s predictions are post-processed into compositions. If not, the caption and text of paper are also processed, along with GNN$_2$'s predictions lead to final composition extraction. We note that our system ignores statistically infrequent corner cases, such as single-cell partial information tables -- we discuss this further in our error analysis. We now describe each component, one by one.

%We propose to classify all MS Tables as shown in Figure \ref{fig:comp_table_cls}. At the first level, we classify tables as Single-cell composition tables and Multi-cell composition tables \& Non-composition tables. Both, Single-cell and Multi-cell composition tables are further classified as to whether complete information is present inside tables to extract compositions, or only partial compositions reside inside tables. We also depict an example of each type of table in Figure \ref{fig:comp_table_cls}. Single-cell partial information tables occur very rarely in our dataset, hence we do not consider this class in the remaining paper.


\subsection{Graph neural networks for table processing}
\label{sec:gnn}

At the core of \sys\ are two GNNs that learn representations for each cell, row, column and the whole table. Let table $T$ has $R$ rows, $C$ columns, and text at $(i,j)^{th}$ cell be $t_{ij}$, where $1\leq i\leq R$, and $1\leq j\leq C$. We construct a graph 
$G_T = (V_T, E_T)$, where $V_T$ has a node for each cell $(i,j)$, one additional node for each row and column, denoted by $(i,0)$ and $(0,j)$, respectively, and one node for the whole table represented by $(0,0)$. The edges in $E_T$ are directed. There are edges between a pair of nodes (in both directions) if they have the same row or same column. All the cell nodes have directed edges to the table node and also their corresponding row and column nodes. 
We initialize the embeddings $\overrightarrow{x_{ij}}$ for each node $(i,j)$ as follows. The table, row and column embeddings are randomly-initialized with a common vector, which gets trained during learning. Other nodes are associated with text $t_{ij}$ -- their embeddings are initialized by running a language model $LM$ over $t_{ij}$.

As constructed, $G_T$ is permutation-invariant, i.e., if we permute rows or columns, we get the same graph and same embeddings. However, initial rows/columns can be semantically different, since they often represent headings for the subsequent list. For instance, material IDs are generally mentioned in first one or two rows/columns of the table. So, we additionally define \emph{index embeddings} $\overrightarrow{p_{i}}$ to represent a row/column numbered $i$. We use the same index embeddings for rows and columns so that our model stays transpose-invariant. We also observe that while first few indices are different, the semantics is generally uniform for indices higher than 3. So, to allow \sys\ to handle large tables, we simply use $\overrightarrow{p_{i}}=\overrightarrow{p_{3}}~ \forall i > 3$. 
Finally, some manually-defined features may be added to each node. The feature values are embedded as $\overrightarrow{f}$ and concatenated to the cell embeddings. Combining all ideas, a cell embedding is initialized as: 
%\begin{equation}
\[
\overrightarrow{x_{ij}} =  \overrightarrow{f_{ij}} \;||\; \left( LM_{CLS}(\langle CLS ~~ t_{ij} ~~ SEP \rangle) + \overrightarrow{p_{i}} + \overrightarrow{p_{j}} \right) \] \[(1\leq i \leq R, 1 \leq j \leq C). 
\]
%\end{equation}

Here,  $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token after running a $LM$ over the sentence inside $\langle\rangle$. Message passing is run on the graph $G_T$ using a GNN, which computes a learned feature vector $\overrightarrow{h}$ for every node: \[\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN\left(\{\overrightarrow{x_{ij}}\}_{i,j=(0,0)}^{(R,C)}\right).\]


\subsection{Single-cell composition tables}
\label{sec:single_cell_table}

In its pipeline, \sys\ first classifies whether $T$ is an SCC table. 
For that, it runs a GNN (named GNN$_1$) on $T$, as discussed above, with two manually defined features (discussed below). 
It then implements a Multi-layer Perceptron MLP$_1$ over the table-level feature vector $\overrightarrow{h_{00}}$  to make the prediction. Additionally, GNN$_1$ also feeds row and column vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$ through another MLP (MLP$_2$) to predict whether they contain material IDs  or not. If $T$ is predicted as an SCC table, then one with the highest MLP$_2$ probability is deemed as material ID row/column (provided that probability > 0.5), and its contents are extracted as potential material IDs. If all row and column probabilities are less than 0.5, then table is predicted to not have Material IDs, as in Figure \ref{fig:three comp_tables}c.

% \begin{wrapfigure}{r}{0.46\textwidth}
%   \vspace{-2ex}
%     \centering
% \FramedBox{3cm}{6.2cm}
% {CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
% PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
% ~\\
% CST$_1$ = NUM? W CPD\\
% CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
% CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
% CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
% }
% \caption{Regexes in composition parser}
%     \label{fig:comp_parser}
%     \vspace{-2ex}
% \end{wrapfigure}
\begin{figure}[hbt]
    \centering
\FramedBox{2.5cm}{5.3cm}
{\small{CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
~\\
CST$_1$ = NUM? W CPD\\
CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
}}
\caption{Regexes in composition parser}
    \label{fig:comp_parser}
    \vspace{-2ex}
\end{figure}

%Single-cell composition tables or others (Multi-cell and Non-composition tables). Then, we use Regular Expressions to extract compositions (set of tuples) from the predicted Single-cell composition tables.

% \subsubsection{RegEx baseline model}
% \label{sub_sec:regex}
% First, we use create a simple Regular Expression based model (RegEx) to identify Single-cell composition tables. We notice that single cell compositions are written in a form that can be matched and parsed using regular expressions (REs). We write different REs for compositions having elements and compounds. This is because in general coefficients succeed compounds and precede elements. After error analysis, we added some more types of RE which can parse compositions involving multiplication of coefficients like $(Ge_{0.25}Ga_{0.10}S_{0.65})_{0.9}-Br_{0.1}$ and $(50-x)Bi_2O_3 * (50-x)B_2O_3 * 2x(AgI-AgBr)$. In total, we write six different types of REs. These REs also handle the case when percentage contribution of compounds is an arithmetic expression having multiplication and division operators. The compounds may be separated by various special characters like $*, -, :, +$ or space or may not be separated. We also created a list of common elements and compounds which are required by the REs in order to parse compositions. RegEx Model predicts a table to be Single-cell composition table if any of the table cell matches with any of the six REs.


%\subsubsection{Classifying Single-cell composition tables vs Others}
%\label{sec:gat_single_cell_table}

%We use a Graph Neural Networks ($GNN$) to predict whether a table is Single-cell composition table or not. We represent table as a graph, where each table cell is a graph node. Formally, let $T$ be the table, $R$ and $C$ be the number of rows and columns in $T$. We represent the table graph by $G_T = (V_T, E_T)$. Here, $V_T = \{(i, j) \; | \; 0 \leq i \leq R, 0 \leq j \leq C\}$ is the set of all nodes/vertices in $G_T$. Note that these also include row nodes of the form $(i, 0)$, column nodes of the form $(0, j)$, and table node $(0, 0)$. We include the row and column nodes to identify the row or column containing material IDs and table node to perform classification at the table level. 
%We connect two table cells by an edge if they share same row or same column. All the table cells also have edges directed to the table node and their corresponding row and column nodes. Hence the set of edges is
%\[ E_T = \{((i_1, j_1), (i_2, j_2)) \; | \; i_1 = i_2 \;or\; j_1 = j_2, \; 1 \leq i_1, i_2 \leq R, 1 \leq j_1, j_2 \leq C\} \; \cup \; \]
%\[ \{((i, j), (i, 0)) \; | \; 1 \leq i \leq R, 0 \leq j \leq C\} \; \cup \; \{((i, j), (0, j)) \; | \; 0 \leq i \leq R, 1 \leq j \leq C\} \; \cup \; \]
%\[ \{((i, j), (0, 0)) \; | \; 1 \leq i \leq R, 1 \leq j \leq C\} \]

%Let $t_{ij}$ and $\overrightarrow{x_{ij}}$ be the text and initial node features for table cell $(i, j)$ respectively. Using a pre-trained Language Model ($LM$) as the text encoder, we get
%\[ \overrightarrow{x_{ij}} = LM_{CLS}(CLS \;||\; t_{ij} \;||\; SEP) \; \forall \; 1 \leq i \leq R, 1 \leq j \leq C\]
%where $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token, which is representative of $t_{ij}$. Embeddings of row nodes, column nodes and table node are initialized with a random vector, which gets learned during training.
%It can be observed from the examples of composition tables presented till now that generally material IDs occur in the initial part of table. To make the model aware of this, we augment our model with row/column index embeddings.
%\[ \overrightarrow{z_{ij}} = \overrightarrow{x_{ij}} + \overrightarrow{p_{i}} + \overrightarrow{p_{j}} \]
%Here, $\overrightarrow{p_{i}}$ is randomly initialized embedding for row $i$ and similarly $\overrightarrow{p_{j}}$ is the embedding for column $j$ having the same size as that of $\overrightarrow{x_{ij}}'s$. We use the same index embeddings for row and column so that our model stays transpose-invariant. To handle the large tables and because of relatively small size of our dataset, we take $\overrightarrow{p_{3}} = \overrightarrow{p_{i}}$ for all $i > 3$.
%Then, $\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN(\{\overrightarrow{z_{ij}}\}_{i,j=(0,0)}^{(R,C)})$ are the output node features in the context of complete table.
%We then feed row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$, to a Multi-layer Perceptron $MLP_1$ to predict whether each row and column contains material IDs or not. If more than one row/column are predicted to have material IDs, then we select the one with highest probability. Finally, we pass $\overrightarrow{h_{00}}$ through another Multi-layer Perceptron $MLP_2$ for Single-cell composition table classification. Final loss is the weighted sum of binary cross entropy loss for single-cell table classification and row/column classification for material IDs. Weights are hyper-parameters.

%\subsubsection{Extracting Single-cell compositions}
%\label{sec:regex_extraction}


\textbf{Rule-based composition parser: }
For an SCC table, \sys\ must parse the full \emph{composition expression} written in a single cell in the row/column corresponding to each Material ID.  Such compositions are close to regular languages and can be parsed via regular expressions. Figure \ref{fig:comp_parser} shows the regular expression (simplified, for understandability) implemented in \sys. Here CMP denotes the matched composition, PATs are three main patterns for it, CSTs are sub-patterns, CPD is a compound, NUM is a number, OB and CB are, respectively, open and closed parentheses (or square brackets). W is zero or more whitespace characters, and SEP contains explicit separators like `-' or `+'. START and END are indicators to separate a regular expression from rest of the text.

The first pattern parses simple number-compound expressions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$. Here each of the two constituents will match with CST$_1$. The other two patterns handle \emph{nested} compositions, where simple expressions are mixed in a given ratio. The main difference between second and third pattern is in the placement of outer ratios -- after or before the simple composition, respectively. Example match for PAT$_2$ is (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and for PAT$_3$ is 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). 

To materialize these rules, \sys\ pre-labels compounds. For our dataset, we use a list-based extractor, though other chemical data extractors \cite{chemdataextractor_v1} may also be used.  After parsing, \sys\ normalizes all coefficients so that they sum to hundred. For nested expressions, the outer ratio and the inner ones are normalized separately and then multiplied.
For units, \sys\ searches for common unit keywords such as mol, mass, weight, and their abbreviations like wt.\%, and at.\%. The search is done iteratively with increasing distance from cell containing the composition. If not found in the table, then the caption is searched. If still not found, mole\% is used as default.

\textbf{Manual Features:} GNN$_1$ uses two hand-coded features. The first feature is set to true if that cell contains a composition that matches our rule-based composition parser. Each value, true or false, is embedded as $\overrightarrow{o}$.
The second feature named \emph{max frequency feature} adds the bias that material IDs are generally unique in a table. We compute $q_{i}^{r}$ and $q_{j}^{c}$, which denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$, respectively. If these numbers are on the lower side, then that row/column has more unique strings, which should increase the probability that it contains material IDs. The computed $q$ values are embedded in a vector as $\overrightarrow{q}$. The embedded feature $\overrightarrow{f_{ij}}$ for cell $(i,j)$ is initialized as $\overrightarrow{o_{ij}} \;||\;  (\overrightarrow{q_{ij}^r}+\overrightarrow{q_{ij}^c})$.


%We notice that single cell compositions are written in a form that can be matched and parsed using Regular Expressions (REs). We write different REs for compositions having elements and compounds. Below, we describe three REs for compounds: $pat1, pat2, $ and $pat3$. Similar REs can be written for elements, difference being that coefficients precede elements, whereas they succeed compounds. We first create a list of common elements and compounds ($comps$) which are required by the REs to parse compositions. $pat1$ matches compositions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$, $pat_2$ matches compositions like (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and $pat3$ matches compositions like 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). During parsing, we normalize the coefficients so that they sum to one.

%\[ comps = (Al\backslash(OH\backslash)3 | PbO2 | PbO | \dots) \]
%\[ num = (\backslash d*\backslash.\backslash d+| 0 | [1-9]\backslash d*) \]
%\[ var = (x | y | z | X) \]
%\[ enum = ((num \; var) | num | var) \]
%\[ exp = enum (\backslash s*[+\backslash-/]\backslash s*enum)* \]
%\[ expr = ((num\backslash s*\%)|exp|(\backslash(exp \backslash))) \]
%\[ sep = \backslash s*[-*:+,]?\backslash s* \]
%\[ start = (\string^|[\string^\backslash w-]) \]
%\[ end = ([\string^\backslash w-]|\$) \]

%\begin{enumerate}
%    \item $subpat1 = expr? \backslash s*comps$ \\
%    $pat1 = start(subpat1(sep \; subpat1)+)end$
    
%    \item $subpat2 = (subpat1(sep \; subpat1)*)$ \\
%    $subpat3 = ((subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash])\backslash s*expr)$ \\
%    $pat2 = start(subpat3(sep\; subpat3)+)end$
    
%    \item $subpat4 = (expr\backslash s*(subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash]))$ \\
%    $pat3 = start(subpat4(sep\; subpat4)+)end$
    
%\end{enumerate}

%We then use these six REs along with predicted row or column index containing material IDs to extract composition tuples from the predicted Single-cell composition tables. For units (mol or weight), we search keywords like mol, mass percent, weight percent, at.\%, wt.\% . We first search for units in table in increasing L1 distance from cell containing composition, and then look for these keywords in the table caption if not found in table.

\subsection{Multi-cell composition tables}
\label{sec:multi-cell}

If $T$ is predicted to not be an SCC table, \sys\ runs it through another GNN (GNN$_2$). The graph structure is very similar to $G_T$ from Section \ref{sec:gnn}, but with two major changes. 
%geared towards incorporating the caption information at prediction time.
First, a new \emph{caption node} is created with initial embedding as given by $LM$ processing the caption text.  
%\textcolor{red}{For this, the table node is replaced by a new \emph{caption node, }}
Edges are added from caption node to all row and column nodes. To propagate the information further to cells, edges are added from row/column nodes to corresponding cell nodes. The caption node especially helps in identifying non-composition (NC) tables. Second,
the max frequency feature from Section \ref{sec:single_cell_table} is also included in this GNN. 

We use tables in Figure \ref{fig:two_comp_tables_2} as our running examples. Notice that Figure \ref{fig:two_comp_tables_2}a is a complete-information table, whereas Figure \ref{fig:two_comp_tables_2}b is not, and can only be understood in the context of its caption, which describes the composition as  $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$. Here x, y are variables, which also need to be extracted and matched with the caption. \sys\ first decodes the row and column feature vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$, as computed by GNN$_2$, via an MLP$_3$ into four classes: composition, constituent, ID, and other (label IDs 1, 2, 3, 0, respectively). The figures illustrate this labeling for our running example. The cell at the intersection of composition row/column and constituent column/row  contains the percentage contribution of that constituent in that composition. 


%Having identified the Single-cell composition tables and extracting compositions from them, we now model the Multi-cell composition tables. We identified two prominent classes, all-info tables and partial-info tables, as shown in Figure \ref{fig:two_comp_tables_2}. In the text corresponding to table shown in Figure \ref{fig:partial_info_table_2}, we find $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$ which helps to decode the table.

\begin{figure}[t]
\begin{center}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/multi_cell_table_1_S0022309314000660.png}
        % \label{fig:multi_cell_comp_table_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/partial_info_table_2_S0022309305006903.png}
        % \label{fig:partial_info_table_2}
    \end{subfigure}
    % \vspace{-1ex}
    \caption{Multi-cell composition tables (a) Complete information \cite{fig_5a} (b) Partial information \cite{fig_5b}}
    \label{fig:two_comp_tables_2}
\end{center}
    \vspace{-0.35in}
\end{figure}

%For Multi-cell composition tables, we classify rows and columns of input table among four classes: \textbf{1 for Composition}, \textbf{2 for Constituent}, \textbf{3 for Material IDs} and \textbf{0 for Others}.
%Label 1 means that row/column specifies a composition. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, all except first two rows and all except first row are composition rows respectively. In Figure \ref{fig:nom_exp_table}, all columns except first are composition columns. Similarly, label 2 implies that row/column contains the percentage contribution of some constituent(s) for every composition column/row. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, first three columns and first two columns are constituent columns respectively. In Figure \ref{fig:nom_exp_table}, last seven rows except the middle one are constituent rows and second row has label 3 as it contains the Material IDs. All other rows and columns have label 0. Note that the cell at the intersection of composition row and constituent column or composition column and constituent row contains the percentage contribution of that constituent in that composition.

Further, to associate the identified percentage contribution with the corresponding constituent (like P$_2$O$_5$ in Figure \ref{fig:two_comp_tables_2}a) or variables x, y in Figure \ref{fig:two_comp_tables_2}b), we perform classification at the edge level. For ease of exposition, we describe our method in this Section \ref{sec:multi-cell} for the setting that the table has been predicted by GNN$_2$ to have row-wise orientation, i.e., rows are compositions and columns are constituents. A transposed computation is done in the reverse case. Since the constituent/variable will likely occur in the same column or row as the cell containing percentage contribution, our method computes an edge feature vector: for edge $e=(i,j)\rightarrow(i',j')$, s.t. $i=i' \vee j=j' $, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{i'j'}}$.
%\textcolor{red}{and for edge $e=(i,j)\rightarrow(i',j')$, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{ij'}}$}. 
It then takes all such edges $e$ from cell $(i,j)$, if row $i$ is labeled composition and column $j$ is labeled constituent. Each edge $e$ is classified through an MLP$_4$, and the edge with maximum logit value is picked to identify constituent/variable. This helps connect 36 to P$_2$O$_5$ and 0.8 to x in our running examples. %A transposed computation is done if rows are constituents and columns are compositions.

GNN$_2$ also helps in predicting NC tables. In case none of the rows/columns are predicted as 1 or 2, then the table is deemed as non-composition and discarded.

%we construct an edge from every table cell to all cells with the same row/column including itself. We then select the edge with maximum logit and use a simple RE to get the constituent/variable from the cell at the other end of selected edge. Some examples of valid edges in above figures are the ones which connect 90 to Sb$_2$O$_3$, 30 to PbCl$_2$, 0.3 to y, 0.8 to x, etc.

% \subsubsection{LM-Lin-Table baseline}
% \label{sec:lm_lin_table}
% Figure \ref{fig:lm_lin_table_baseline} depicts our LM-Lin-Table baseline model. Here, LM is a pre-trained Language Model. Here, we flatten the input table row-wise after replacing the empty table cells with special [EMPTY] token. Then, we tokenize this linear table using the LM tokenizer. It's possible to obtain more than one wordpiece for some table cells. Since, the length of tokenized linear table can be greater than 512, we truncate minimum possible rows from the end so that input length to LM becomes less than or equal to 512. Let the tokenized linear table be denoted by $[t_0, t_1, \dots, t_n]$, where $t_0 = [CLS]$, $t_n = [SEP]$, $n < 512$ and the number of rows after truncation be $R'$. We then pass $[t_0, t_1, \dots, t_n]$ through the LM to obtain contextual embeddings of every wordpiece $[\overrightarrow{z_0}, \dots, \overrightarrow{z_n}]$.

% \begin{figure}[!htb]
% \begin{center}
%     \centering
%     \includegraphics[scale=0.3]{multi_cell_baseline.png}
%     \caption{Schematic of the LM-Lin-Table baseline model}
%     \label{fig:lm_lin_table_baseline}
% \end{center}
% \end{figure}

% We take the contextual embedding of first word-piece of every table cell to be representative of it. Let $0 < k_{1,1} < k_{1,2} < \dots < k_{R',C} < n$ be the indices such that $k_{i,j}$ is the index of first wordpiece of cell $(i, j)$.
% To make the baseline model aware of different row and column indexes, we add randomly initialized row and column index embeddings, so that final cell embeddings become $[\overrightarrow{h_{k_{1,1}}}, \dots, \overrightarrow{h_{k_{R',C}}}]$, where $\overrightarrow{h_{k_{i,j}}} = \overrightarrow{z_{k_{i,j}}} + \overrightarrow{rid_{i}} + \overrightarrow{cid_{j}}$, $\overrightarrow{rid_{i}}$ and $\overrightarrow{cid_{j}}$ are the $i^{th}$ row and $j^{th}$ column index embeddings respectively. For brevity, we now denote $\overrightarrow{h_{k_{i,j}}}$ by $\overrightarrow{h_{i,j}}$.
% Row and column embeddings are computed by taking average of final cell embeddings of cells occurring in that row/column i.e. $\overrightarrow{r_i} = Mean(\overrightarrow{h_{i,1}}, \dots, \overrightarrow{h_{i,C}})$ and $\overrightarrow{c_j} = Mean(\overrightarrow{h_{1,j}}, \dots, \overrightarrow{h_{R',j}})$.
% Edge embeddings are computed by concatenating the final cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. Finally, all row and column embeddings are fed to a MLP to get probabilities of every row and column belonging to 4 classes as described earlier and edge embeddings are passed through another MLP to obtain logit score for every table edge. Loss function consists of row/column cross-entropy loss and edge binary cross-entropy loss.

%\subsubsection{GAT-Multi-cell-table}

%This model is mostly similar to the model as discussed in section \ref{sec:gat_single_cell_table}. Since, we do not need to do table-level classification in this case, we remove the $(0, 0)$ table node and its edges from the graph. Here too, the contextual row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$ are obtained with the help of $LM$ and $GNN$. Then, we feed them through a MLP with softmax activation at the end to get probabilities of every row and column belonging to four classes (composition, constituent, material ID and others). Edge embeddings are computed by concatenating the contextual cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. These edge embeddings are then passed through another MLP to obtain logit score for every table edge. Training loss consists of weighted row/column cross-entropy loss and edge binary cross-entropy loss.



\textbf{Partial information table predictor: }
%Till now, we have predicted the row \&column labels and also linked the extracted percentage contributions with the corresponding constituent/variable. If all row and column labels are predicted to be 0, then we classify that table as a non-composition table.
Next, \sys\ distinguishes between complete-information (CI) and partial-information (PI) MCC tables. It uses a logistic regression model with custom input features for this prediction task. 
%We describe this assuming the table orientation is predicted to be row-oriented by GNN$_2$ (i.e., rows are compositions, columns are constituents); analogous transposed computation will be done for the reverse case. 
Let $P$ and $Q$ be the sets of all row indices with label 1 (composition) and column indices with label 2 (constituent), respectively. Also, assume $n_{ij}$ is the number present in table cell $(i, j)$ or $0$ if no number is present.  To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely an MCC-PI, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is MCC-CI. Features F4 (and F5) computes the maximum (average) of the sum of all extracted compositions. The intuition of F4 and F5 is that the higher these feature values, higher the chance of the table being an MCC-CI. Formally, 

\[
\mathrm{F4}=(\max_{i \in P} \sum_{j \in Q}n_{ij}) ~~~~~~~~~~~~~
\mathrm{F5}=(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij}).
\]

%to extract the composition tuples as described in section \ref{sec:proposed_cls_tables}. For this, we build a Logistic Regression model with custom input features.
%Assume the table to be a row-oriented table as inferred from predicted row and column labels. Let $P$ and $Q$ be the sets of all row indexes with label 1 and column indexes with label 2 respectively. Also, assume $n_{ij}$ is the first number present in table cell $(i, j)$ or $0$ if no number is there. To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely a partial-information table, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is complete information. Features F4 (and F5) computes the maximum (average) of the sum of 

%\begin{enumerate}
%    \item \textit{Number of unique variables}: If we have some variables, then it is more likely for the table to belong to partial information table class.

%    \item \textit{Number of unique constituents}: If there are many constituents, then table is more likely to be an all information table.

%    \item \textit{Maximum sum among all extracted compositions} $(\max_{i \in P} \sum_{j \in Q}n_{ij})$: Greater this quantity, greater the chances of being in all-information table class.
    
%    \item \textit{Average sum across all extracted compositions} $(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij})$: Explanation similar to above feature.

%    \item \textit{Number of rows/columns with label 2}: If there are lesser number of rows/columns with label 2, then table is probably a partial information table.

%\end{enumerate}

\textbf{MCC table extractor: } For MCC-CI, MLP$_3$ and MLP$_4$ outputs are post-processed, and units are added (similar to SCC tables), to construct final extracted tuples. For MCC-PI, on the other hand, information in text needs to be combined with the MLP outputs for final extraction. The first step here is to search for the composition expression, which may be present in table caption, table footer, and if not there, in somewhere in the rest of the research paper. Here, \sys\ resorts to using our rule-based composition parser from Figure \ref{fig:comp_parser}, but with one key difference. Now, the composition may contain variables ($x$, $y$) and even mathematical expressions like $100-x$. So the regular grammar is enhanced to replace the non-terminal NUM with a non-terminal EXPR, which represents, numbers, variables, and simple mathematical expressions over them. An added constraint is that if there are variables in set $Q$, then those variables must be present in the matched composition expression. \sys\ completes the composition by substituting the variable values from every composition row into the matched composition. There may be other types of MCC-PI tables where only compounds are identified in tables, such as Figure \ref{fig:three comp_tables}b. For these, \sys\ first computes the constituent contributions in terms of variables from composition expression, and then equates it with the numbers present in rows/columns labeled 1 (composition). In our example, \sys\ matches x with the numbers 10, 20, 30, and 40, and the rest of the composition is extracted by processing the composition expression in the caption with these values of x. Units and material IDs are added to the tuples, similar to other tables.


%After identifying the partial information Multi-cell composition tables, we try to complete the composition by searching for REs in the table caption, table footer, and then sequentially in research paper text from top to bottom. In case of variables as in Figure \ref{fig:partial_info_table_2}, we search for REs containing precisely those variables and complete the composition by substituting the variable values from every composition row. If case of constituents as in Figure \ref{fig:partial_info_table_1}, we first compute the constituent contributions in terms of variables and then equate it with the numbers present in rows/columns having label 1. For example, in terms of variables, contribution of $CsCl$ is $x/100$ for table shown in Figure \ref{fig:partial_info_table_1}. Since $0 \leq x/100 \leq 1$, we divide the numbers in table by 100. And then solve for x by equating $x/100 = 40/100$ for last row, giving $x = 40$, which completes the composition as $\{(La_2S_3, 0.2), (Ga_2S_3, 0.4), (CsCl, 0.4)\}$. Then we prepend material IDs and append units to the tuples to complete the extraction.


\subsection{Loss functions \& constraint-aware training}
\label{sec:constraints}

\sys\ needs to train the two GNNs and the PI table predictor. Our data construction provides gold labels for each prediction task (discussed in next section), so we train these component-wise. The PI table predictor is trained on standard logistic regression loss. GNN$_1$ is trained on a weighted sum of binary cross entropy loss for SCC table classification and row/column classification for material IDs --  weight is a hyper-parameter. Similarly, GNN$_2$ loss function consists of sum of row/column cross-entropy loss and edge binary cross-entropy loss. 

GNN$_2$ has the more complex prediction problem, since it has to perform four-way labeling for each row and column. In initial experiments, we find that the model sometimes makes structural errors like labeling one row as constituent and another row as composition in the same table -- highly unlikely as per the semantics of composition tables. To encourage GNN$_2$ to make structurally consistent predictions, we express a set of constraints on the complete labelings, as follows. (1) A row and a column cannot both have compositions or constituents.  %(2) Compositions and constituents should be orthogonally predicted  
(2) Composition and material ID must be orthogonally predicted (i.e, if a row has a composition then ID must be predicted in some column, and vice versa). (3) Constituents and material IDs must never be orthogonally predicted (if rows have constituents then another row must have the ID). And, (4) material ID must occur at most once for the entire table. Limitation of space precludes complete mathematical exposition of all constraints (see App. ~\ref{app:constraint} for details). As an example, constraint (1) can be expressed as a hard constraint as:
\begin{center}
\(
r_i = l \Rightarrow c_j \neq l ~~~~\forall i\in\{1,\ldots, R\}, j\in \{1,\ldots,C\}, l\in\{1,2\}. 
\)
\end{center}
Here, $r_i$ and $c_j$ are predicted labels of row $i$ and column $j$. We wish to impose these structural constraints at training time, so that the model is trained to honor them. We follow prior work by Nandwani et al. \cite{yatin}, to first convert these hard constraints into a probabilistic statement. For example, constraint (1) gets expressed as:
\begin{center}
\(
P(r_i = l; \theta) + P(c_j = l; \theta) - 1 \leq 0\) \( \forall i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}.
\)
\end{center}
$\theta$ represents GNN$_2$'s parameters. Following same work, each such constraint gets converted to an auxiliary penalty term, which gets added in the loss function for constraint-aware training. The first constraint gets converted to:
\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l; \theta) + P(c_j = l; \theta) - 1) \]
This (and similar auxiliary losses for other constraints) get added to the GNN$_2$'s loss function for better training. $\lambda$ is a hyper-parameter. Note that we also use constraint (4) for GNN$_1$ training.

%We augmented our GAT based models with some features/constraints to improve the performance. These bells and whistles have been discussed in the following sub-sections.

%\subsubsection{Constraints}
%\label{sec:constraints}
%In the approach presented till now, it is possible for the model to predict some row as composition row and some column as composition column and similar is the case for constituents. But practically, this does not make sense. We formulate these constraints mathematically and modify our training procedure by adding a suitable term to the loss function.

%Let $r_i$ be the label assigned by the model to row $i$ and $c_j$ be the label assigned to column $j$. We can write the hard version of these constraints as $r_i = 1 \Rightarrow c_j \neq 1$ and $r_i = 2 \Rightarrow c_j \neq 2$, where $i \in \{1, \dots, R\}$ and $j \in \{1, \dots, C\}$. We rewrite these as
%$r_i \neq l \lor c_j \neq l$ for $l \in \{1, 2\}$. In a similar fashion, labels 1 \& 3 can't occur simultaneously in rows or columns, labels 2 and 3 can't occur orthogonal to each other, and label 3 can occur at most once for the entire table.
%We convert all these hard constraints to soft constraints as done by Yatin et al. \cite{yatin} to obtain:

%\begin{enumerate}
%    \item $P(r_i = l) + P(c_j = l) - 1 \leq 0\;$ for $i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}$
    
%    \item $P(r_{i_1} = 1) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $i_1, i_2 \in \{1, \dots R\}, \; i_1 \neq i_2$
    
%    \item $P(c_{j_1} = 1) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $j_1, j_2 \in \{1, \dots C\}, \; j_1 \neq j_2$
    
%    \item $P(r_i = l) + P(c_j = 5-l) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}, \; l \in \{2, 3\}$
    
%    \item $P(r_{i_1} = 3) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $1 \leq i_1 < i_2 \leq R$
    
%    \item $P(c_{j_1} = 3) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $1 \leq j_1 < j_2 \leq C$
    
%    \item $P(r_i = 3) + P(c_j = 3) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}$

%\end{enumerate}

%We now convert these soft constraints to penalty terms and add them to the loss function. For the first soft constraint, we add
%\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l) + P(c_j = l) - 1) \]
%to the loss function for all tables $T$ in the training dataset. Here, $\lambda$ is a hyper-parameter which controls the magnitude of penalty relative to the original training loss. We add similar penalty terms for other soft constraints.

%\subsubsection{Manual features}

%Here, we introduce some task-specific features which can potentially boost the performance.

%\begin{enumerate}
%    \item \textit{Max-frequency Feature}: This feature helps to incorporate the bias that material IDs are unique. Let $f_{i}^{(r)}$ and $f_{j}^{(c)}$ denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$ respectively. If these numbers are on the lower side, then that row/column has more probability of containing material IDs. For Figure \ref{fig:nom_exp_table}, $f_1^{(r)} = 6$, $f_2^{(r)} = 2$, and $f_3^{(r)} = 3$. This is because we copy the cell contents in case of merged cells. We also set $f_0^{(r)} = f_0^{(c)} = 0$. These numbers are then mapped to learnable embeddings $(\overrightarrow{q_m}'s)$ and concatenated with $\overrightarrow{x_{ij}}$. Hence, $\overrightarrow{z_{ij}} = (\overrightarrow{x_{ij}} + \overrightarrow{p_i}) + \overrightarrow{p_j}) \; || \; (\overrightarrow{q_{f_{i}^{(r)}}} + \overrightarrow{q_{f_{j}^{(c)}}})$. Here, we take $\overrightarrow{q_{m}} = \overrightarrow{q_m'}$ for all $m > m'$ and $m'$ is a hyper-parameter. Size of $\overrightarrow{q_m}'s$ is also a hyper-parameter.
    
%    \item \textit{Boolean Regex Feature}: We use this feature while classifying Single-cell composition tables. The feature is set to true for a table cell if that cell contains a composition that can be parsed using any of our regular expressions. We map true and false to different embeddings and concatenate them with $\overrightarrow{x_{ij}}'s$ to obtain new $\overrightarrow{z_{ij}}'s$.

%\end{enumerate}

%\subsubsection{Caption node}
%Sometimes, table captions can be useful to differentiate composition tables from non-composition tables. Therefore, we add a node in the graph corresponding to table caption for Multi-cell composition tables. We represent the caption node by $(0, 0)$ and add edges from caption node to all row and column nodes. To propagate the information further to table cells, edges are added from row and column nodes to corresponding table cell nodes.


==> sections_old/5_experiments.tex <==
% !TEX root = main.tex
\section{Experiments} 
\label{sec:experiments}


%\subsection{Dataset}
%\begin{wraptable}{R}{0.4\textwidth}
%\vspace{-0.15in}
%\centering
%\caption{\small Statistics of table types in all three splits}
%\begin{tabular}{lccc}
%    \toprule &
%    \multicolumn{3}{c}{ \textbf{Splits}}\\
%    \cmidrule(lr){2-4}
%    \textbf{Table Type} &  \textbf{Train} & \textbf{Dev} & \textbf{Test} \\
%    \midrule
%    SCC & 704 & 110 & 113 \\
%    MCC-CI & 626 & 132 & 132 \\
%    MCC-PI & 317 & 109 & 112 \\
%    NC & 2761 & 387 & 380 \\
%    \midrule
%    Total & 4408 & 738 & 737 \\
%    \bottomrule
%\end{tabular}
%\label{tab:dataset_stats}
%\vspace{-0.2in}
%\end{wraptable}

% \textbf{Dataset construction:} % moved to appendix
\textbf{Dataset details:} We match a manually-curated KB of materials and compositions with tables in the relevant papers, to automatically provide distantly-supervised labels for extraction (hand-annotated for dev/test sets). This results in 5,883 tables from 2536 publications, of which 2,355 express compositions, with 16,729 materials, and a total of 58,481 (material ID, constituent, composition percentage, unit) tuples. Dataset construction and details are provided in App.~\ref{app:dataset} and~\ref{app:dataset-details}.\\
\textbf{Baseline models: }
We implement \sys\ with $LM$ as \textsc{MatSciBERT} \cite{gupta_matscibert_2022}, and the GNNs as Graph Attention Networks \cite{velickovic2018graph}. We compare \sys\ with four non-GNN baseline models. Our first baseline is \textsc{TaPas} \cite{herzig-etal-2020-tapas}, a state-of-the-art table QA system, which flattens the table, adds row and column index embeddings, and passes as input to a language model. To use TaPas for our task, we use table caption as proxy for the input question. All the model parameters in this setting are initialized randomly. Our second baseline is \textsc{TaPas-Adapted}, with the goal of providing the benefit of \textsc{MatSciBERT} to  \textsc{TaPas} -- it initializes language model weights by \textsc{MatSciBERT}. For the input to remain consistent with \textsc{MatSciBERT}, we add row and column index embeddings to \textsc{MatSciBERT} \emph{output}, instead of input as in original \textsc{TaPas} model. The third baseline model is based on \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation. Similar to \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} uses \textsc{MatSciBERT} as the LM instead of \textsc{BERT}. Further details on the \textsc{TaPas} and \textsc{TaBERT} models are included in App.~\ref{app:baseline}.

%{$\bullet$ \bf \textsc{TaPas}:} This has the same architecture as proposed by Herzig et al. \cite{herzig-etal-2020-tapas} for Table-QA task. Here, row and column index embeddings are passed as input to $LM$. All the model parameters are initialized randomly. We use table caption as a proxy for the input question.\\
%{\bf $\bullet$ \textsc{TaPas-Adapted}:} Here, we initialize \textsc{TaPas} with $LM$ pre-trained weights for a fair comparison with \sys. Also, for the input to remain consistent with the original $LM$, we add row and column index embeddings to the $LM$ output and we do not include caption in the input. We term this modified model as \textsc{TaPas-Adapted}. 

%The input table is flattened row-wise and passed through these two baseline models. We provide the precise details in Appendix.

\begin{table*}[htb]
\centering
\scalebox{0.85}{
\begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} &  \textbf{CV} \\
    \midrule
    
    \textsc{TaPas} & 80.37 ($\pm$ 4.78) & 71.23 ($\pm$ 0.77) & 49.88 ($\pm$ 0.10) & 543.67 \\
    \textsc{TaPas-Adapted} & \textbf{89.65} ($\pm$ 0.46) & 70.91 ($\pm$ 3.79) & 57.88 ($\pm$ 2.73) & \textbf{490.33} \\
    \textsc{TaBERT} & 79.61 ($\pm$ 8.25) & 58.20 ($\pm$ 1.79) & 47.05 ($\pm$ 1.50) & 1729.67 \\
    \textsc{TaBERT-Adapted} & 85.07 ($\pm$ 6.28) & 59.31 ($\pm$ 0.67) & 50.10 ($\pm$ 2.86) & 1195.67 \\
    % \textsc{TaPas-Adapted} & 86.80 ($\pm$ 0.50) & 70.43 ($\pm$ 2.01) & 56.67 ($\pm$ 4.67) & 424.33 \\
    \textsc{v-}\sys & 77.38 ($\pm$ 12.21) & \textbf{76.52} ($\pm$ 2.37) & \textbf{64.71} ($\pm$ 3.45) & 626.33 \\
    \bottomrule
\end{tabular}
}
\caption{Performance of \textsc{v-}\sys{} vs baseline models on MCC-CI and NC table types.}
\label{tab:baselines}
\vspace{-0.10cm}
\end{table*}

\begin{table*}[htb]
\centering
%\vspace{-2ex}
\scalebox{0.85}{
\begin{tabular}{lccccc}
    \toprule
    \textbf{Model} & \textbf{TT Acc.} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
    \midrule
    
    \sys & 88.35 ($\pm$ 1.20) & 82.40 ($\pm$ 3.88) & \textbf{70.14} ($\pm$ 0.44) & \textbf{63.51} ($\pm$ 1.90) & 87.33 \\
    \midrule

\sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 80.80 ($\pm$ 3.24) & 68.60 ($\pm$ 1.26) & 62.53 ($\pm$ 1.89) & 120.11 \\
    \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 78.71 ($\pm$ 3.66) & 69.28 ($\pm$ 1.11) & 60.94 ($\pm$ 0.98) & 584.78 \\
    \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.23} ($\pm$ 0.51) & 67.51 ($\pm$ 1.36) & 63.50 ($\pm$ 2.49) & \textbf{19.11} \\
    \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 68.54 ($\pm$ 9.32) & 65.98 ($\pm$ 1.21) & 59.36 ($\pm$ 2.20) & 541 \\
    
    \bottomrule
\end{tabular}
}
\caption{Contribution of task specific features and constraints in \sys.}
\label{tab:ablations}
\vspace{-0.1in}
\end{table*}

\begin{table}[!htb]
% \vspace{-1.5cm}
\centering
\scalebox{0.75}{
\begin{tabular}{ccccc}
    \toprule
    \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} \\
    \midrule
    
    SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) \\
    
    MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) \\
    
    MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) \\

    \bottomrule
\end{tabular}
}
\caption{\sys{} performance on the table-types.}
\label{tab:perf_table_types}
\vspace{-0.25in}
\end{table}

%\subsection{Evaluation metrics}
\textbf{Evaluation metrics:} 
We compute several metrics in our evaluation. (1) \emph{Table-type (TT) prediction accuracy} -- it computes table-level accuracy on the 4-way table classification as NC, SCC, MCC-CI and MCC-PI. 
(2) \textit{ID F$_1$ score} computes F$_1$ score for Material ID extraction.  
(3) \textit{Tuple-level (TL) F$_1$ score} evaluates performance on the extraction of composition tuples. A gold is considered matching with a predicted 4-tuple if \emph{all} arguments match exactly. 
(4) \textit{Material-level (MatL) F$_1$ score} is the strongest metric. It evaluates whether all predicted information related to a material (including its ID, all constituents and their percentages) match exactly with the gold.
Finally, (5) \textit{constraint violations (CV)} counts the number of violations of hard constraints in the prediction. We consider all four types of constraints, as discussed in Section \ref{sec:constraints}. %\end{enumerate}

%Thus, TL precision means how many, out of all the tuples model predict, are correct. Similarly, TL recall means how many, out of all the gold tuples, were predicted by the model. TL F$_1$ score is the harmonic mean of TL precision and recall.\\
%$\bullet$\textit{Composition-level (CL) metrics}: This set of metrics evaluate model at the composition level. So, CL precision means out of all the compositions (set of tuples) model predict, how many of them were completely correct. Similarly, CL recall means out of all the gold compositions, how many were exactly predicted by the model. CL F$_1$ score is the harmonics mean of CL precision and CL recall.\\
    
\textbf{Implementation details: }
%In our experiments, we take the $LM$ as MatSciBERT \cite{gupta_matscibert_2022} which is a materials-science domain specific language model and we choose $GNN$ to be 
For Graph Attention Networks (GATs) \cite{velickovic2018graph}, we use the GAT implementation of Deep Graph Library \cite{dgl_citation_wang2019}. For LMs, \textsc{TaPas}, we use the implementation by Transformers library \cite{transformers_huggingface}. We use \textsc{TaBERT}'s source code from their github repository. We implement and train all models using PyTorch  \cite{pytorch_NEURIPS2019_9015}. We optimize the model parameters using Adam \cite{adam_opt_kingma} and a triangular learning rate \cite{triangle_lr}. We further use different learning rates for $LM$ and non-LM parameters (GNNs, MLPs) (App.~\ref{app:hyperparameter}). To deal with imbalanced labels, we scale loss for all labels by weights inversely proportional to their frequency in the training set. All experiments were run on a machine with one 32 GB V100 GPU. Each model is run with three seeds and the mean and std. deviation are reported. The code and data is available \href{https://anonymous.4open.science/r/DiSCoMaT-EEFB/}{here}.

%\vspace{-0.5cm}
\subsection{Results}
%\vspace{-0.2cm}
\emph{How does table linearization compare with a graph-based model for our task?} To answer this question,  we compare \sys{} with four models: {\sc TaPas}, \textsc{TaBERT}, and their adapted versions. \textsc{TaPas} and \textsc{TaBERT} do table level and row level linearizations respectively. Since the baselines do not have the benefit of regular expressions, features, and constraints, we implement a version of our model without these, which we call \textsc{v-}\sys. We do this comparison, trained and tested only on the subset of MCC-CI and NC tables, since other table types require regular expressions for processing. As shown in Table \ref{tab:baselines} \textsc{v-}\sys{} obtains 6-7 pt higher F$_1$ on TL and MatL scores, suggesting that a graph-based extractor is likely a better fit for our problem - this led to us choosing a GNN-based approach for \sys. 

%\textsc{TaPas} and \textsc{TaPas-Adapted} as shown in Table \ref{tab:baselines}. For simplicity, we train and evaluate all three models on MCC-CI and NC tables only. We refer to \sys{} without max-frequency feature, constraint loss, and caption node as Vanilla-\sys{} or in short \textsc{V-}\sys.

\emph{How does \sys{} model perform on the complete task?}
Table \ref{tab:ablations}, reports \sys{} performance on the full test set with all table types. 
%Here, we have 3 set of parameters for GNN$_1$ and 3 set of parameters for GNN$_2$ corresponding to 3 seeds. Hence, we report results averaged over 9 ordered pair of seeds.
Its ID and tuple F$_1$-scores are 82 and 70, respectively. Since these errors get multiplied, unsurprisingly, its material-level F$_1$-score is lower (63.5). Table \ref{tab:perf_table_types} reports \sys{} performance for different table types. In this experiment, we assume that table type is already known and run only the relevant part of \sys{} for extraction. We find that MCC-PI is the hardest table type, since it requires combining information from text and tables for accurate extraction. A larger standard deviation in ID F$_1$ for MCC-PI is attributed to the fact that material IDs occur relatively rarely for this table type -- the test set for MCC-PI consists of merely 20 material ID rows and columns.
\begin{wrapfigure}{r}{0.25\textwidth}
    \vspace{-0.1in}
    \centering
    \includegraphics[width=0.25\textwidth]{confusion_matrix.png}
    %\vspace{-1ex}
    \caption{Confusion matrix for all table types}
    \label{fig:confusion}
    \vspace{-0.2in}
\end{wrapfigure}
\emph{What is the incremental contribution of task-specific features and constraints?}
Table \ref{tab:ablations} also presents the ablation experiments. \sys{} scores much higher that \textsc{v-}\sys, which does not have these features and constraints. We also perform additional ablations removing one component at a time. Unsurprisingly constrained training helps with reducing constraint violations. Both constraints and features help with ID prediction, due to constraints (2), (3), (4) and max frequency feature. Removal of caption node significantly hurts performance on MCC-PI tables, as these tables require combining caption with table cells. All contribute to the tuple-level metric. 
\emph{What are the typical errors in \sys?} 
Confusion matrix in Figure \ref{fig:confusion} suggests that most table type errors are between MCC-PI and NC tables. This could be attributed to following reasons. (i) \sys{} has difficulty identifying rare compounds like Yb$_2$O$_3$, ErS$_{3/2}$, Co$_3$O$_4$ found in MCC-PI---these aren't present frequently in the training set. (ii) MCC-PI tables specify dopant percentages found in small quantities. %are also a source of error. %Generally the text contains a base composition (summing to 100), in which dopant is added. Finding the base composition in paper text corresponding to dopants mentioned in the table is non-trivial. Sometimes, instead of percentage contributions being expressed as variables, constituents are specified as variables. 
(iii) Completion of composition in MCC-PI tables require other tables from the same publication. (iv) Finally, MCC-PI composition may contain additional information such as properties that may bias the model to classify it as an NC table. Some corner cases are given in App.~\ref{app:corner}. %Yet another case is when caption mentions silicates/phosphates and hence remaining constituent is SiO$_2$/P$_2$O$_5$.
%\vspace{-0.1in}

%Table \ref{tab:perf_table_types} shows the performance of \sys{} (averaged over three seeds) on individual table types. In these experiments, we assume that table type is already known. For SCC, we use GNN$_1$ just for materials ID prediction and Rule-based composition parser to parse compositions from table cells. From CL F$_1$-score, we can observe that \sys performs best on SCC, then MCC-CI, and then MCC-PI. Large standard deviation in Material IDs F$_1$-Score for MCC-PI can be attributed to the fact that Material IDs occur relatively rarely for this table type. Test set for MCC-PI consists of merely 20 Material ID rows and columns.

% \begin{wraptable}{R}{0.6\textwidth}
% \vspace{-1.5cm}
% \centering
% \caption{Performance of \sys{} on different table types}
% \scalebox{0.75}{
% \begin{tabular}{ccccc}
%     \toprule
%     \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
%     \midrule
    
%     SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) & 0.67 \\
    
%     MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) & 59.33 \\
    
%     MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) & 26.67 \\

%     \bottomrule
% \end{tabular}
% }
% \label{tab:perf_table_types}
% % \vspace{-0.2cm}
% \end{wraptable}


==> sections_old/6_conclusions.tex <==
\section{Conclusions} 
\label{sec:conclusions}
\vspace{-0.15cm}
We define the novel task of extracting material compositions from tables in scientific articles. We harvest a dataset using distant supervision, combining information from a manually developed database of materials with tables in respective papers. We present a strong baseline system, \sys, a pipeline based on LM, GNNs, and task-specific regex, %, which is a pipeline of a material science language model, two graph neural networks along with task-specific regular expressions, features and constraints. Our experiments show 
that outperforms other architectures that linearizes the tables. We plan to extend it to extract material properties as well. \\
\textbf{Limitations and outlook:} \sys\ is a pipelined solution trained component-wise. This raises a research question: can we train one end-to-end trained ML model that not only analyzes a wide variety of table structures, but also combines understanding of regular expressions, extraction of chemical compounds and scientific units, text understanding and some mathematical processing. This defines a challenging ML research question, and one that can have direct impact to the scientific MatSci community.

==> sections_old/7_acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:checklist}

% This document has been adapted
% by Steven Bethard, Ryan Cotterell and Rui Yan
% from the instructions for earlier ACL and NAACL proceedings, including those for 
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan, 
% NAACL 2017 by Margaret Mitchell, 
% ACL 2012 by Maggie Li and Michael White, 
% ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
% ACL 2002 by Eugene Charniak and Dekang Lin, 
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections_old/7_checklist.tex <==
% !TEX root = main.tex
\section*{Checklist}
\label{sec:checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections_old_v2/0_abstract.tex <==
%Tables in scientific articles carry important information (often numeric), which must be adequately extracted for a comprehensive machine understanding of an article. Our paper studies information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction.  Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also develop \sys, a strong baseline for the task, which combines graph neural networks with several problem-specific regular expressions, features and constraints. Our experiments evaluate the contribution of each model component in the final performance. We release our code and data for further research.

A crucial component in the curation of KB for a scientific domain is information extraction from tables in the domain's published research articles. To facilitate research in this direction, we define a novel NLP task of extracting compositions of materials (e.g., glasses) from tables in material science papers. The task involves solving several challenges in concert, such as tables that mention compositions have highly varying structures;  text in captions and full paper needs to be incorporated along with data in tables; and regular languages for numbers,  chemical compounds, composition expressions must be integrated in the model. 
We release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present \sys, a strong baseline that combines multiple graph neural networks with several task-specific regular expressions, features, and constraints. We show that \sys{} outperforms recent table processing architectures by significant margins. 
%Our experiments also assess the value of additional modifications on the final performance of the model. 
We release our code and data for further research.

%Most of the work on table extraction assumes prior knowledge on the table structure and format---a scenario that may not hold true for tables from scientific literature. A generic framework that can mine information from tables is crucial for the development of knowledge bases in several engineering and scientific domains. To address this challenge, we take a holistic view on information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction. Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present a strong baseline for the task, \sys, which combines graph neural networks with several problem-specific regular expressions, features, and constraints. We show that \sys outperforms other existing models. Our experiments also evaluate how additional modifications can enhance the final performance of the model. We release our code and data for further research.

%-- progress on the task will hopefully lead to the construction of a large repository of materials (and subsequently their properties) known to mankind.

%Vast amount of Materials Science-specific information like compositions and properties is stored in tables, images and text of research publications. Since property extraction can only be performed after composition extraction, we focus on extracting compositions from tables.
% missing motivation to extract compositions from tables instead of text
%This paper is a first attempt to solve this problem and no annotated datasets are publicly available.
%First, we formally define a new problem to the ML community.
%Second, to motivate the problem, we perform extensive analysis of the ways in which compositions are reported and highlight various facets of the problem.
%Third, we share a dataset comprising of 4408 distantly supervised training tables, along with 738 and 737 manually annotated dev and test tables respectively.
%Fourth, we propose a strong baseline model based on Graph Attention Networks (GATs) \cite{velickovic2018graph} and MatSciBERT \cite{gupta_matscibert_2022} (pre-trained BERT-based Language Model).
% can mention results, bert based based baseline
%\footnote{Code and data are available at: \url{https://github.com/}.}
%\end{comment}

==> sections_old_v2/1_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\label{sec:intro}

Advanced knowledge of a science or engineering domain is typically found in domain-specific research papers. Information extraction (IE) from scientific articles develops ML methods to automatically extract this knowledge for curating large-scale domain-specific KBs (e.g., \cite{ernst-bmc15,hope-naacl21}). These KBs have a variety of uses: they lead to ease of information access by domain researchers \cite{tsatsaronis-bmc15,hamon-sw17}, provide data for developing domain-specific ML models \cite{nadkarni-akbc21}, and potentially help in accelerating scientific discoveries \cite{materials_project, challenges_21}. 

Significant research exists on IE from \emph{text} of research papers (see \cite{nasar-scientometrics18} for survey), but less attention is given to IE (often, numeric) from tables. Tables may report performance of algorithms on a dataset, quantitative results of clinical trials, or other important information. Of special interest to us are tables that mention the composition and properties of an entity. Such tables are ubiquitous in various fields such as food and nutrition (tables of food items with nutritional values) \cite{Cavalcanti2021DonkeyMA, Stokvis2021EvaluationOT}, fuels (constituents and calorific values) \cite{Kar2022EffectOF, Beliavskii2022EffectOF}, building construction (components and costs) \cite{Aggarwal2022ComponentRC}, materials (constituents and properties) \cite{keshri2022elucidating}, medicine (compounds with weights in drugs) \cite{kalegari2014chemical}, and more. 

% \textcolor{red}{In materials science (MatSci) articles, the details on synthesis and characterization are reported in the text~\cite{mysore-etal-2019-materials}, while material compositions are mostly reported in tables~\cite{jensen2019machine}}. 
In materials science (MatSci) articles, the details on synthesis and characterization are reported in the text~\cite{mysore-etal-2019-materials}, while material compositions are mostly reported in tables~\cite{jensen2019machine}.
A preliminary analysis of MatSci papers reveals that $\sim$85\%\footnote{estimated by randomly choosing 100 compositions from a MatSci database and checking where they are reported} of material compositions and their associated properties (e.g., density, stiffness) are reported in tables and not text. %\todo{M: I added "not text" -- can you check if this is still 85\%} 
Thus, IE from tables is essential for a comprehensive understanding of a given paper, and for increasing the coverage of resulting KBs. To this extent, we define a novel NLP task of extraction of materials (via IDs mentioned in paper), constituents, and their relative percentages. For instance, Fig.\ref{fig:three comp_tables}a should output four materials A1-A4, where ID A1 is associated with three constituents (MoO$_3$, Fe$_2$O$_3$, and P$_2$O$_5$) and their respective percentages, 5, 38, and 57. 

% \begin{figure}[t]
% \begin{center}
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{multi_cell_comp_table_1_S0022309303003624.png}
%         \label{fig:multi_cell_comp_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{\scriptsize Glass compositions in the paper: $20La_2S_3-(80 - x)Ga_2S_3-xCsCl$.}
%         \includegraphics[width=\textwidth]{partial_info_table_1_S0022309399000617.png}
%         \label{fig:partial_info_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{single_cell_S0022459614003995.png}
%         \label{fig:single_cell_comp_table}
%     \end{subfigure}
%     \vspace{-0.3cm}
%     \caption{\small Examples of composition tables (a) Multi-cell complete-info composition table (b) Multi-cell partial-info composition table (c) Single-cell composition table }
%     \label{fig:three comp_tables}
%     \vspace{-0.6cm}
% \end{center}
% \end{figure}

\begin{figure*}[t]
\begin{center}
    \centering
    \includegraphics[width=\textwidth]{figure_1.png}
    \caption{Examples of composition tables (a) Multi-cell complete-info \cite{fig_1a_mcc_all} (b) Multi-cell partial-info {with caption on top} \cite{fig_1b_mcc_pi} (c) Single-cell \cite{fig_1c_scc}}
    \label{fig:three comp_tables}
    \vspace{-0.6cm}
\end{center}
\end{figure*}

A model for this task necessitates solving several challenges. First, compositions in MatSci paper are expressed in widely varying table styles. Two main types are \emph{multi-cell compositions} (MCC), where a material composition is presented in multiple cells %and constituents are on two axes %\todo{T: constituents are not always on the same axes. M: how will you describe differently. T: all constituents and their contribution are in table} 
%with each cell representing the percentage 
(Fig.~\ref{fig:three comp_tables}a), and \emph{single-cell compositions} (SCC), where the full composition is mentioned in a single cell as an expression (Fig.~\ref{fig:three comp_tables}c). Second, tables may have incomplete information, which requires reading caption or paper text for complete understanding (Fig.~\ref{fig:three comp_tables}b). Third, there is a need to integrate regular expression processing (such as for chemical compounds, numbers, units and composition expression in SCC tables) within the IE model. 
Fourth, there can be four units for specifying the percentage -- mol\%, mol fraction, wt.\% or wt. fraction, requiring normalization. Finally, IE can benefit from constraint processing, e.g., percentages should sum to hundred. See Appendix ~\ref{sec:problem} for further discussion on challenges. %Interestingly, some researchers write percentages such that they add to numbers less than or more than 100, and expect the reader to re-normalize. 
% All these and more make the problem of extracting material compositions from scientific tables a challenging problem. 
While many of these issues have been investigated separately (e.g., numerical IE \cite{madaan-aaai16}, unit extraction \cite{sarawagi14}, chemical compound identification \cite{weston2019named}, NLP for tables \cite{jensen2019machine,swain2016chemdataextractor}), solving all these in concert creates a challenging testbed for the NLP community. 

Here, we harvest a distantly supervised training dataset of 4,408 tables and 38,799 composition-constituent tuples by aligning a MatSci database with tables in papers. We also label 1,475 tables manually for dev and test sets. We build a baseline system \sys, which uses a pipeline of a domain-specific language model \cite{gupta_matscibert_2022}, and two graph neural networks (GNNs), along with several hand-coded features and constraints. We evaluate our system on accuracy metrics for various subtasks, including material ID prediction, tuple-level predictions, and material-level complete predictions. We find that \sys's GNN architecture obtains $\sim$15 point increase in accuracy numbers, compared to table processors \cite{herzig-etal-2020-tapas, yin-etal-2020-tabert}, which linearize the table for IE. %by a language model. 
Subsequent analysis reveals common sources of \sys\ errors, which will inform future research. We release all our data and code for further research on this challenging task.

% pleas use these short forms in the paper
%\begin{table}
 %   \centering
  %  \begin{tabular}{ll} 
   %     \toprule
    %    Table Type & Meaning \\
     %   \midrule
      %  SCC table & Single-cell composition table \\
       % MCC-CI table & Multi-cell composition complete-info table \\
       % MCC-PI table & Multi-cell composition partial-info table \\
       % NC table & Non-composition table \\
    %    \bottomrule
    %\end{tabular}
%\end{table}

% Motivation to CL Community: IE tasks have either been studied from text, or from tables with well-defined/known structures. Our task is challenging for NLP because (1) tables that mention compositions have highly varying structures; (2) text in captions and full paper needs to be incorporated along with data in tables for IE; (3) processing is needed for regular languages: numbers, units, chemical compounds, compositions expressions; (4) there are additional math constraints (e.g., percentages summing to 100). While many of these issues have been investigated separately (e.g., NLP papers on numerical IE, unit extractors, chemical compound identification, NLP for tables, etc.), solving all these challenges in concert creates a challenging testbed for the NLP community.
% Task is too specific: Extracting information from scientific articles is a broad theme of vast importance. We posit that the specific task considered by us will have ramifications for similar tasks in many other disciplines, such as food and nutrition (tables of foods with nutritional values) [1,2], fuels (constituents and calorific values) [3,4], building construction (costs of components) [5,6], medicines (compounds with weights), and more. Please see these references for the broad relevance of our work. The approach is built on the notion that there are two main styles of writing compositions – one in single cells as a long pattern, and other in multiple cells of the table. Similarly, some constituents may be implied (or mentioned in caption/text) and hence not needed in tables. These two notions are generic and should apply in other domains too. The specific lists of compounds, or units are specific and will need to be reworked for a new domain – but those are minor aspects of the solution.
% Material Science focus: It is indeed true that our paper has the strongest linkage to material science. But, similar focused CL papers have been published earlier, e.g., a paper on material science at EMNLP [7], a paper on chemical compounds at EMNLP [8], financial NER at ACL [9] and more. We expect our method to be adaptable to other similar tasks – the domain-specific features and engineering are relatively small parts of the paper.


==> sections_old_v2/2_related_work.tex <==
% !TEX root = main.tex
\section{Related work} 
\label{sec:related_work}
%Information extraction (IE) is instrumental for knowledge base creation. 
%While most of the earlier works on information extraction (IE) focusses on rule-based approaches \cite{chiticariu-etal-2013-rule}, large datasets, computational efficiency, and success of neural models lead to machine learning-based IE systems\cite{chiticariu-etal-2013-rule}.
\vspace{-0.075in}
Recent works have developed neural models for various NLP tasks based on tabular data, \textit{viz}, tabular natural language inference \cite{tnli_orihuela2021natural, xinfotabs}, QA over one or a corpus of tables \cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr, chemmengath-emnlp21}, table orientation classification\cite{deeptable_habibi2020,nishida2017understanding}, and relation extraction from tables \cite{relation_ex_tables_2013, neurel_relex_2}. Several recent papers study QA models---they all linearize a table and pass it to pre-trained language model. For example, 
\textsc{TaPas} \cite{herzig-etal-2020-tapas} does this for Wikipedia tables to answers natural language questions by selecting table cells and aggregation operators. \textsc{TaBERT} \cite{yin-etal-2020-tabert} and RCI \cite{feifei_row_col_interact} also use similar ideas alongside some architectural modifications to handle rows and columns better. \textsc{TABBIE} \cite{tabbie} consists of two transformers that encode rows and columns independently, whereas \textsc{TaPEx} uses encoder-decoder architecture using BART. TABBIE and \textsc{TaPEx} also introduce pre-training over tables to learn table representations better. Similar to our work, tables have also been modeled as graphs for sequential question answering over tables \cite{muller_acq_2019}. However, all these works generally assume a fixed and known structure of tables with the same orientation, with the top row being the header row in all cases -- an assumption violated in our setting. 
%uses a different pre-training objective and model architecture to jointly learn NL sentence and table representations. Row and column intersection (RCI) model \cite{feifei_row_col_interact} predicts the probability of finding the answer to a given question in each row and column of a table independently, without any pre-training on tables. \textsc{TaPEx} \cite{tapex} uses a BART encoder-decoder architecture, pre-trained via synthetic executable programs to mimic the behaviour of SQL execution engine. \textsc{TABBIE} \cite{tabbie} consists of two transformers that encode rows and columns independently and is pre-trained using the corrupt-cell objective. 
%TABBIE performs better than other models on table-based tasks such as column type prediction. 
%Similar to our work, tables have also been modeled as graphs for sequential question answering over tables \cite{muller_acq_2019}. However, all these works generally assume a fixed and known structure of tables with the same orientation, with the top row being the header row in all cases -- an assumption violated in our setting. 
%The table orientation and header row are assumed to be fixed for this problem. 
\\
{\bf Orientation and semantic structure classification:} %of tables has also been attempted using neural models.
DeepTable \cite{deeptable_habibi2020} is a permutation-invariant neural model, which classifies tables into three orientations, while TabNet \cite{nishida2017understanding} uses RNNs and CNNs in a hybrid fashion to classify web tables into five different types of orientations. \textsc{InfoTabS} \cite{infotabs} studies natural language inference on tabular data via linearization and language models, which has been extended to the multilingual setting \cite{xinfotabs}, and has been combined with knowledge graphs \cite{transkblstm}. Some earlier works also focused on annotating column types, entity ID cells, and pair of columns with binary relations, based on rule-based and other ML approaches, given a catalog~\cite{sunita_iitb}.%consisting of types, entities and relations .
%. Here, concatenated premise-hypothesis pair is sent through language models to classify whether the premise (info-box) entails, contradicts, or is unrelated to a given hypothesis. 
%However, these info-boxes are special type of tables containing two columns: first containing keys and other containing values. 
%This has been extended to the multilingual setting \cite{xinfotabs}, and has been combined with knowledge graphs \cite{transkblstm}. 
%Extending this, Minhas et al. \cite{xinfotabs} released a multilingual TNLI dataset comprising of info-boxes from ten different languages.  Further, TransKBLSTM model was proposed by Varun et al. \cite{transkblstm} to augment TNLI models with knowledge graphs. 

%There has also been work on annotating column types, cells with entity IDs, pair of columns with binary relations, etc given a catalog consisting of types, entities and relations \cite{sunita_iitb}. But again in this work, they take simple tables with fixed header and no merged rows or columns. 

%But their graph structure is different than ours as the table orientation and header row is fixed for their dataset.

%Distant Supervision, proposed by Mintz et al. \cite{mintz-etal-2009-distant}, is an approach to create a noisy dataset and does not require labelled data. This method is generally used to annotate any given sentence with the relations it might express. In our work, we use a similar approach where we use the Interglad database to annotate our training set.

%{\bf NLP for materials literature:} After the success of BERT \cite{devlin2018bert}, numerous domain-specific language models have been released for  public-use. For MatSci domain, researchers have contributed language models like MatSciBERT \cite{gupta_matscibert_2022}, MatBERT \cite{matbert_2022}, and BatteryBERT \cite{batterybert_2022}. MatBERT \cite{matbert_2022} highlights the advantages of materials domain-specific pre-training on the NER task. BatteryBERT  exhibits superior performance on battery related downstream tasks. MatSciBERT  yields state of the art performance on downstream tasks of abstract classification, NER, and relation classification, and we use it in our work. Wang et al. \cite{wang_automated_2022} recently develop a rule-based NER and relation extraction to create a pipeline for extracting superalloy data from text and tables. There also exists a table extraction tool that takes input HTML or XML of MatSci research papers, and uses regular expression based parser for extracting compositions, scientific units, and related information \cite{mit_table_parser}. However, the regexs used in these works are highly specific and will require significant modifications for different classes of materials.  Despite the availability of MatSci language models, deep neural models have not been explored for IE from materials tables -- the focus of this work.


% Information extraction (IE) is instrumental for knowledge base creation. The transition from rule based IE systems to machine learning IE systems became possible due to availability of large datasets and computational efficiency\cite{chiticariu-etal-2013-rule}. IE from text and tabular data has witnessed tools like WOE\cite{wu-weld-2010-open}, ReVerb\cite{ReVerb2011}, OLLIE\cite{mausam-etal-2012-open}, TaPaS\cite{herzig-etal-2020-tapas}, TaBERT \cite{yin-etal-2020-tabert}, and TabNet\cite{tabnet_Arik_Pfister_2021} to name a few. Specifically, neural models capable of semantically parsing tabular information are jointly pre-trained over natural language queries and structured and semi-structured tables\cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr}. 
% Information extraction from MS literature is an emerging field because accurately creating, maintaining, and updating material compositions and property databases is a humanly difficult task. Researchers have developed specialised tools for extracting information like extracting inorganic material synthesis routes using word embedding, named entity recognition a\cite{kim_we_ner_cvae, kim_virtual_2017}, and generating database of Curie and Néel temperatures by using a combination of text parsing, table parsing, relation extraction on XMLs and HTMLs of relevant scientific documents\cite{court_auto-generated_2018}, and rule based NER and relation extraction for creating superalloys database\cite{wang_automated_2022}.

% For IE from MS tables, researchers have developed a table extraction tool which takes input of HTML or XML of material science research papers, and uses regex based parser for extracting compositions, scientific units, and related information\cite{mit_table_parser}. This tool was used to extract data related to zeolites\cite{mit_table_parser}, cementitious materials\cite{mit_cement_uvegi}, and aluminum alloys\cite{elsa_aluminium}. ChemDataExtractor is another tool which is capable of extracting complete chemical compositions, but, only from the full information tables present in research papers\cite{chemdataextractor_v1,chemdataextractor_v2}. However, these existing tools are quite specific and can not understand the different structures of MS tables posing special challenges in information extraction as discussed in section 2.1. 

% Recently, researchers have developed materials science language models like MatSciBERT\cite{gupta_matscibert_2022}, MatBERT\cite{matbert_2022}, and BatteryBERT\cite{batterybert_2022}. MatSciBERT\cite{gupta_matscibert_2022} yielded state of the art performance on downstream tasks of abstract classification, named entity recognition, and relation classification, MatBERT\cite{matbert_2022} authors achieved state of the art results on NER tasks, and BatteryBERT\cite{batterybert_2022} was used to enhance battery materials database by LM based question answering downstream task.


==> sections_old_v2/3_dataset_construction.tex <==
% !TEX root = main.tex
\section{Dataset construction}
\label{sec:dataset_construction}
We match a MatSci DB of materials and compositions with tables from published papers, to automatically provide distantly-supervised labels for extraction (hand-annotated for dev \& test sets). This results in 5,883 tables from 2536 publications, of which 2,355 express compositions, with 16,729 materials, and a total of 58,481 (material ID, constituent, composition percentage, unit) tuples.

Now, we create a train set with table-level annotation (NC, SCC, MCC-PI, MCC-CI), row/column-level annotation (ID, composition, constituent, other), and edge level annotation. We also create dev/test sets with these and final tuple-level ground truth. For training set, we first use a commercial DB \cite{interglad} of glass compositions with the respective references. Then, we extract all tables from the 2,536 references in the DB using textmining API. We use table parser \cite{mit_table_parser} for raw XML tables and captions.  We keep 1,880 papers for train set, and rest are split in dev and test (Table \ref{tab:dataset_stats_2}).

The DB does not contain information about the location of a given composition in the paper -- in text, images, graphs, or tables. If present in a table, it can appear in any column or row. Since we do not know the exact location of a composition, we use distantly supervised train set construction \cite{mintz-etal-2009-distant}. First, we simply match the chemical compounds and percentages (or equivalent fractions) mentioned in the DB with the text in a table from the associated paper. If all composition percentages are found and in multiple cells of the table, it is marked as MCC-CI. However, due to several problems (see Section~\ref{sec:problem}), it misses many composition tables. To increase the coverage, we additionally use our rule-based composition parser, but restricted to only those compounds (CPD non-terminal in Figure \ref{fig:comp_parser}) that appear in the DB for this paper. This is important supervision, and leads to a high quality annotation of composition expressions in these papers. If this matching happens: (i) in a cell, the table is deemed as SCC, (ii) on caption/paper text that has a variable (or compound) found in the table, it is marked as MCC-PI. In case of no matching, the table is marked as NC. This automatic annotation is post-processed into row, column and edge labels.

One further challenge is that material IDs mentioned in papers are not provided in the DB. So, we manually annotate material IDs for all the identified composition tables in the training set. This leads to a train set of 11,207 materials with 38,799 tuples from 4,408 tables. Since train set is distantly supervised and can have noise, a MatSci expert manually annotated the dev and test tables with row/column/edge labels, units, tuples, compositions, and table type, resulting in over 2,500 materials and over 9,500 tuples per set. Further statistics are discussed in ~\ref{app:dataset-details}.


==> sections_old_v2/4_model.tex <==
% !TEX root = main.tex
\section{\sys\ architecture} 
\label{sec:model}
To address automated extraction of material compositions from tables, we present an ML formulation of the problem.  Formally, given a table $T$, its caption, and the complete text of publication in which $T$ occurs, we aim to extract compositions expressed in $T$, in the form $\{(id, c_k^{id}, p_k^{id}, u_k^{id} )\}_{k=1}^{K^{id}}$. Here, $id$ represents the material ID, as defined in the paper. Material IDs are defined by MatSci researchers to succinctly refer to that composition in text and other tables. $c_k^{id}$ is a constituent element or compound present in the material, $K^{id}$ is the total number of constituents in the material, $p_k^{id} > 0$ denotes the percentage contribution of $c_k^{id}$ in its composition, and $u_k^{id}$ is the unit of $p_k^{id}$ (either mole\% or weight\%). For instance, the desired output tuples corresponding to ID A1 from Figure \ref{fig:three comp_tables}a are (A1, MoO$_3$, 5, mol\%), (A1, Fe$_2$O$_3$, 38, mol\%), (A1, P$_2$O$_5$, 57, mol\%).

% \begin{wrapfigure}{l}{0.55\textwidth}
%     \vspace{-3ex}
%     \centering
%     \includegraphics[width=0.55\textwidth, height=4cm]{flowchart.png}
%     \caption{The design of \sys}
%     \label{fig:comp_table_cls}
%     \vspace{-1ex}
% \end{wrapfigure}
\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.45\textwidth, height=3cm]{flowchart.png}
    \caption{The design of \sys}
    \label{fig:comp_table_cls}
    \vspace{-1ex}
\end{figure}

Figure \ref{fig:comp_table_cls} illustrates the basic pipeline for extraction in \sys. We find that the simplest task is to identify whether the table $T$ is an SCC table, owing to a distinctive presence of multiple numbers, and compounds in single cells. \sys{} first runs a GNN-based SCC predictor, which classifies $T$ as an SCC table or not. For SCC table, it uses a standalone rule-based composition parser. For the other category, \sys{} runs a second GNN (GNN$_2$), and labels rows and columns of $T$ as compositions, material IDs, constituents, and others. If no constituents or composition predictions are found, then $T$ is deemed to be a non-composition (NC) table. Else, it is an MCC table, for which \sys{} predicts whether it has all information in $T$ or some information is missing (partial-information predictor). If it is complete information table, then GNN$_2$'s predictions are post-processed into compositions. If not, the caption and text of paper are also processed, along with GNN$_2$'s predictions leading to final composition extraction. We note that our system ignores statistically infrequent corner cases, such as single-cell partial information tables -- we discuss this further in our error analysis. We now describe each of these components, one by one.

%We propose to classify all MS Tables as shown in Figure \ref{fig:comp_table_cls}. At the first level, we classify tables as Single-cell composition tables and Multi-cell composition tables \& Non-composition tables. Both, Single-cell and Multi-cell composition tables are further classified as to whether complete information is present inside tables to extract compositions, or only partial compositions reside inside tables. We also depict an example of each type of table in Figure \ref{fig:comp_table_cls}. Single-cell partial information tables occur very rarely in our dataset, hence we do not consider this class in the remaining paper.
\subsection{GNNs for table processing}
\label{sec:gnn}
At the core of \sys\ are two GNNs that learn representations for each cell, row, column and the whole table. Let table $T$ has $R$ rows, $C$ columns, and text at $(i,j)^{th}$ cell be $t_{ij}$, where $1\leq i\leq R$, and $1\leq j\leq C$. We construct a directed graph 
$G_T = (V_T, E_T)$, where $V_T$ has a node for each cell $(i,j)$, one additional node for each row and column, denoted by $(i,0)$ and $(0,j)$, respectively, and one node for the whole table represented by $(0,0)$. There are bidirectional edges between two nodes of the same row or column. All cell nodes have directed edges to the table node and also their corresponding row and column nodes. 
%We initialize the embeddings $\overrightarrow{x_{ij}}$ for each node $(i,j)$ as follows. 
The table, row and column embeddings are randomly-initialized with a common vector, which gets trained during learning. A node $(i,j)$'s embedding $\overrightarrow{x_{ij}}$ is initialized by running a language model $LM$ over $t_{ij}$.

As constructed, $G_T$ is permutation-invariant, i.e., if we permute rows or columns, we get the same graph and embeddings. However, initial rows/columns can be semantically different, since they often represent headings for the subsequent list. For instance, material IDs are generally mentioned in first one or two rows/columns of the table. So, we additionally define \emph{index embeddings} $\overrightarrow{p_{i}}$ to represent a row/column numbered $i$. We use the same index embeddings for rows and columns so that our model stays transpose-invariant. We also observe that while first few indices are different, the semantics is generally uniform for indices higher than 3. %\textcolor{red}{This is because, after the headers (or material IDs) in the first two rows/columns, the following indices have either different constituents or compositions (for example, rows 4-5 in Figure \ref{fig:three comp_tables}b and \ref{fig:three comp_tables}c)}. 
Accordingly, to allow \sys\ to handle large tables, we simply use $\overrightarrow{p_{i}}=\overrightarrow{p_{3}}~ \forall i > 3$. 
Finally, any manually-defined features added to each node are embedded as $\overrightarrow{f}$ and concatenated to the cell embeddings. Combining all ideas, a cell embedding is initialized as: 
\vspace{-1ex}
%\begin{equation}
\[
\overrightarrow{x_{ij}} =  \overrightarrow{f_{ij}} \;||\; \left( LM_{CLS}(\langle CLS ~ t_{ij} ~ SEP \rangle) \!+\! \overrightarrow{p_{i}} \!+\! \overrightarrow{p_{j}} \right) \] 
%\[(1\leq i \leq R, 1 \leq j \leq C). \]
%\end{equation}
Here, $1\leq i \leq R, 1 \leq j \leq C$. $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token after running a $LM$ over the sentence inside $\langle\rangle$. Message passing is run on the graph $G_T$ using a GNN, which computes a learned feature vector $\overrightarrow{h}$ for every node: \[\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN\left(\{\overrightarrow{x_{ij}}\}_{i,j=(0,0)}^{(R,C)}\right).\]

\subsection{Single-cell composition tables}
\label{sec:single_cell_table}
In its pipeline, \sys\ first classifies whether $T$ is an SCC table. 
For that, it runs a GNN (named GNN$_1$) on $T$ with two manually defined features (see below). 
It then implements a Multi-layer Perceptron MLP$_1$ over the table-level feature vector $\overrightarrow{h_{00}}$  to make the prediction. Additionally, GNN$_1$ also feeds row and column vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$ through another MLP (MLP$_2$) to predict whether they contain material IDs  or not. If $T$ is predicted as an SCC table, then one with the highest MLP$_2$ probability is deemed as material ID row/column (provided probability > $\alpha$, where $\alpha$ is a hyper-parameter tuned on dev set), and its contents are extracted as potential material IDs. If all row and column probabilities are less than $\alpha$, then table is predicted to not have Material IDs, as in Figure \ref{fig:three comp_tables}c.

% \begin{wrapfigure}{r}{0.46\textwidth}
%   \vspace{-2ex}
%     \centering
% \FramedBox{3cm}{6.2cm}
% {CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
% PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
% ~\\
% CST$_1$ = NUM? W CPD\\
% CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
% CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
% CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
% }
% \caption{Regexes in composition parser}
%     \label{fig:comp_parser}
%     \vspace{-2ex}
% \end{wrapfigure}
% \begin{figure}[hbt]
%     \centering
% \FramedBox{2.5cm}{5.3cm}
% {\small{CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
% PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
% ~\\
% CST$_1$ = NUM? W CPD\\
% CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
% CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
% CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
% }}
% \caption{Regexes in composition parser}
%     \label{fig:comp_parser}
%     \vspace{-2ex}
% \end{figure}

\textbf{Rule-based composition parser: }
For an SCC table, \sys\ must parse the full \emph{composition expression} written in a single cell in the row/column corresponding to each Material ID.  
\begin{wrapfigure}{l}{0.3\textwidth}
    \vspace{-0.1in}
    % \centering
    % \includegraphics[width=0.25\textwidth]{confusion_matrix.png}
    % %\vspace{-1ex}
    % \caption{Confusion matrix for all table types}
    % \label{fig:confusion}
    % \vspace{-0.2in}
    \centering
    \FramedBox{2.5cm}{5.3cm}
    {\small{CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
    PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
    ~\\
    CST$_1$ = NUM? W CPD\\
    CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
    CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
    CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
    }}
    \caption{Regexes in parser}
        \label{fig:comp_parser}
        \vspace{-2ex}
\end{wrapfigure}
Such compositions are close to regular languages and can be parsed via regular expressions. Figure \ref{fig:comp_parser} shows the regular expression (simplified, for understandability) implemented in \sys. Here CMP denotes the matched composition, PATs are three main patterns for it, CSTs are sub-patterns, CPD is a compound, NUM is a number, OB and CB are, respectively, open and closed parentheses (or square brackets). W is zero or more whitespace characters, and SEP contains explicit separators like `-' or `+'. START and END are indicators to separate a regular expression from rest of the text.

%Single-cell composition tables or others (Multi-cell and Non-composition tables). Then, we use Regular Expressions to extract compositions (set of tuples) from the predicted Single-cell composition tables.

% \subsubsection{RegEx baseline model}
% \label{sub_sec:regex}
% First, we use create a simple Regular Expression based model (RegEx) to identify Single-cell composition tables. We notice that single cell compositions are written in a form that can be matched and parsed using regular expressions (REs). We write different REs for compositions having elements and compounds. This is because in general coefficients succeed compounds and precede elements. After error analysis, we added some more types of RE which can parse compositions involving multiplication of coefficients like $(Ge_{0.25}Ga_{0.10}S_{0.65})_{0.9}-Br_{0.1}$ and $(50-x)Bi_2O_3 * (50-x)B_2O_3 * 2x(AgI-AgBr)$. In total, we write six different types of REs. These REs also handle the case when percentage contribution of compounds is an arithmetic expression having multiplication and division operators. The compounds may be separated by various special characters like $*, -, :, +$ or space or may not be separated. We also created a list of common elements and compounds which are required by the REs in order to parse compositions. RegEx Model predicts a table to be Single-cell composition table if any of the table cell matches with any of the six REs.


%\subsubsection{Classifying Single-cell composition tables vs Others}
%\label{sec:gat_single_cell_table}

%We use a Graph Neural Networks ($GNN$) to predict whether a table is Single-cell composition table or not. We represent table as a graph, where each table cell is a graph node. Formally, let $T$ be the table, $R$ and $C$ be the number of rows and columns in $T$. We represent the table graph by $G_T = (V_T, E_T)$. Here, $V_T = \{(i, j) \; | \; 0 \leq i \leq R, 0 \leq j \leq C\}$ is the set of all nodes/vertices in $G_T$. Note that these also include row nodes of the form $(i, 0)$, column nodes of the form $(0, j)$, and table node $(0, 0)$. We include the row and column nodes to identify the row or column containing material IDs and table node to perform classification at the table level. 
%We connect two table cells by an edge if they share same row or same column. All the table cells also have edges directed to the table node and their corresponding row and column nodes. Hence the set of edges is
%\[ E_T = \{((i_1, j_1), (i_2, j_2)) \; | \; i_1 = i_2 \;or\; j_1 = j_2, \; 1 \leq i_1, i_2 \leq R, 1 \leq j_1, j_2 \leq C\} \; \cup \; \]
%\[ \{((i, j), (i, 0)) \; | \; 1 \leq i \leq R, 0 \leq j \leq C\} \; \cup \; \{((i, j), (0, j)) \; | \; 0 \leq i \leq R, 1 \leq j \leq C\} \; \cup \; \]
%\[ \{((i, j), (0, 0)) \; | \; 1 \leq i \leq R, 1 \leq j \leq C\} \]

%Let $t_{ij}$ and $\overrightarrow{x_{ij}}$ be the text and initial node features for table cell $(i, j)$ respectively. Using a pre-trained Language Model ($LM$) as the text encoder, we get
%\[ \overrightarrow{x_{ij}} = LM_{CLS}(CLS \;||\; t_{ij} \;||\; SEP) \; \forall \; 1 \leq i \leq R, 1 \leq j \leq C\]
%where $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token, which is representative of $t_{ij}$. Embeddings of row nodes, column nodes and table node are initialized with a random vector, which gets learned during training.
%It can be observed from the examples of composition tables presented till now that generally material IDs occur in the initial part of table. To make the model aware of this, we augment our model with row/column index embeddings.
%\[ \overrightarrow{z_{ij}} = \overrightarrow{x_{ij}} + \overrightarrow{p_{i}} + \overrightarrow{p_{j}} \]
%Here, $\overrightarrow{p_{i}}$ is randomly initialized embedding for row $i$ and similarly $\overrightarrow{p_{j}}$ is the embedding for column $j$ having the same size as that of $\overrightarrow{x_{ij}}'s$. We use the same index embeddings for row and column so that our model stays transpose-invariant. To handle the large tables and because of relatively small size of our dataset, we take $\overrightarrow{p_{3}} = \overrightarrow{p_{i}}$ for all $i > 3$.
%Then, $\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN(\{\overrightarrow{z_{ij}}\}_{i,j=(0,0)}^{(R,C)})$ are the output node features in the context of complete table.
%We then feed row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$, to a Multi-layer Perceptron $MLP_1$ to predict whether each row and column contains material IDs or not. If more than one row/column are predicted to have material IDs, then we select the one with highest probability. Finally, we pass $\overrightarrow{h_{00}}$ through another Multi-layer Perceptron $MLP_2$ for Single-cell composition table classification. Final loss is the weighted sum of binary cross entropy loss for single-cell table classification and row/column classification for material IDs. Weights are hyper-parameters.

%\subsubsection{Extracting Single-cell compositions}
%\label{sec:regex_extraction}



The first pattern parses simple number-compound expressions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$. Here each of the two constituents will match with CST$_1$. The other two patterns handle \emph{nested} compositions, where simple expressions are mixed in a given ratio. The main difference between second and third pattern is in the placement of outer ratios -- after or before the simple composition, respectively. Example match for PAT$_2$ is (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and for PAT$_3$ is 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). 

To materialize these rules, \sys\ pre-labels compounds. For our dataset, we use a list-based extractor, though other chemical data extractors \cite{chemdataextractor_v1} may also be used.  After parsing, \sys\ normalizes all coefficients so that they sum to hundred. For nested expressions, the outer ratio and the inner ones are normalized separately and then multiplied.
For units, \sys\ searches for common unit keywords such as mol, mass, weight, and their abbreviations like wt.\%, and at.\%. The search is done iteratively with increasing distance from cell containing the composition. If not found in the table, then the caption is searched. If still not found, mole\% is used as default.

\textbf{Manual Features:} GNN$_1$ uses two hand-coded features. The first feature is set to true if that cell contains a composition that matches our rule-based composition parser. Each value, true or false, is embedded as $\overrightarrow{o}$.
The second feature named \emph{max frequency feature} adds the bias that material IDs are generally unique in a table. We compute $q_{i}^{r}$ and $q_{j}^{c}$, which denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$, respectively. If these numbers are on the lower side, then that row/column has more unique strings, which should increase the probability that it contains material IDs. The computed $q$ values are embedded in a vector as $\overrightarrow{q}$. The embedded feature $\overrightarrow{f_{ij}}$ for cell $(i,j)$ is initialized as $\overrightarrow{o_{ij}} \;||\;  (\overrightarrow{q_{ij}^r}+\overrightarrow{q_{ij}^c})$.


%We notice that single cell compositions are written in a form that can be matched and parsed using Regular Expressions (REs). We write different REs for compositions having elements and compounds. Below, we describe three REs for compounds: $pat1, pat2, $ and $pat3$. Similar REs can be written for elements, difference being that coefficients precede elements, whereas they succeed compounds. We first create a list of common elements and compounds ($comps$) which are required by the REs to parse compositions. $pat1$ matches compositions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$, $pat_2$ matches compositions like (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and $pat3$ matches compositions like 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). During parsing, we normalize the coefficients so that they sum to one.

%\[ comps = (Al\backslash(OH\backslash)3 | PbO2 | PbO | \dots) \]
%\[ num = (\backslash d*\backslash.\backslash d+| 0 | [1-9]\backslash d*) \]
%\[ var = (x | y | z | X) \]
%\[ enum = ((num \; var) | num | var) \]
%\[ exp = enum (\backslash s*[+\backslash-/]\backslash s*enum)* \]
%\[ expr = ((num\backslash s*\%)|exp|(\backslash(exp \backslash))) \]
%\[ sep = \backslash s*[-*:+,]?\backslash s* \]
%\[ start = (\string^|[\string^\backslash w-]) \]
%\[ end = ([\string^\backslash w-]|\$) \]

%\begin{enumerate}
%    \item $subpat1 = expr? \backslash s*comps$ \\
%    $pat1 = start(subpat1(sep \; subpat1)+)end$
    
%    \item $subpat2 = (subpat1(sep \; subpat1)*)$ \\
%    $subpat3 = ((subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash])\backslash s*expr)$ \\
%    $pat2 = start(subpat3(sep\; subpat3)+)end$
    
%    \item $subpat4 = (expr\backslash s*(subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash]))$ \\
%    $pat3 = start(subpat4(sep\; subpat4)+)end$
    
%\end{enumerate}

%We then use these six REs along with predicted row or column index containing material IDs to extract composition tuples from the predicted Single-cell composition tables. For units (mol or weight), we search keywords like mol, mass percent, weight percent, at.\%, wt.\% . We first search for units in table in increasing L1 distance from cell containing composition, and then look for these keywords in the table caption if not found in table.

\subsection{Multi-cell composition tables}
\label{sec:multi-cell}

If $T$ is predicted to not be an SCC table, \sys\ runs it through another GNN (GNN$_2$). The graph structure is very similar to $G_T$ from Section \ref{sec:gnn}, but with two major changes. 
%geared towards incorporating the caption information at prediction time.
First, a new \emph{caption node} is created with initial embedding as given by $LM$ processing the caption text.  
%\textcolor{red}{For this, the table node is replaced by a new \emph{caption node, }}
Edges are added from caption node to all row and column nodes. To propagate the information further to cells, edges are added from row/column nodes to corresponding cell nodes. The caption node especially helps in identifying non-composition (NC) tables. Second,
the max frequency feature from Section \ref{sec:single_cell_table} is also included in this GNN. 

We use tables in Figure \ref{fig:two_comp_tables_2} as our running examples. While Figure \ref{fig:two_comp_tables_2}a is a complete-information table, Figure \ref{fig:two_comp_tables_2}b is not, and can only be understood in the context of its caption, which describes the composition as  $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$. Here x, y are variables, which also need to be extracted and matched with the caption. \sys\ first decodes the row and column feature vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$, as computed by GNN$_2$, via an MLP$_3$ into four classes: composition, constituent, ID, and other (label IDs 1, 2, 3, 0, respectively). The figures illustrate this labeling for our running example. The cell at the intersection of composition row/column and constituent column/row represents the percentage contribution of that constituent in that composition. 
%Having identified the Single-cell composition tables and extracting compositions from them, we now model the Multi-cell composition tables. We identified two prominent classes, all-info tables and partial-info tables, as shown in Figure \ref{fig:two_comp_tables_2}. In the text corresponding to table shown in Figure \ref{fig:partial_info_table_2}, we find $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$ which helps to decode the table.

\begin{figure}[t]
\begin{center}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/multi_cell_table_1_S0022309314000660.png}
        % \label{fig:multi_cell_comp_table_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/partial_info_table_2_S0022309305006903.png}
        % \label{fig:partial_info_table_2}
    \end{subfigure}
    % \vspace{-1ex}
    \caption{Multi-cell composition tables (a) Complete information \cite{fig_5a} (b) Partial information \cite{fig_5b}}
    \label{fig:two_comp_tables_2}
\end{center}
    \vspace{-4ex}
\end{figure}
%For Multi-cell composition tables, we classify rows and columns of input table among four classes: \textbf{1 for Composition}, \textbf{2 for Constituent}, \textbf{3 for Material IDs} and \textbf{0 for Others}.
%Label 1 means that row/column specifies a composition. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, all except first two rows and all except first row are composition rows respectively. In Figure \ref{fig:nom_exp_table}, all columns except first are composition columns. Similarly, label 2 implies that row/column contains the percentage contribution of some constituent(s) for every composition column/row. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, first three columns and first two columns are constituent columns respectively. In Figure \ref{fig:nom_exp_table}, last seven rows except the middle one are constituent rows and second row has label 3 as it contains the Material IDs. All other rows and columns have label 0. Note that the cell at the intersection of composition row and constituent column or composition column and constituent row contains the percentage contribution of that constituent in that composition.

Further, to associate the identified percentage contribution with the corresponding constituent (like P$_2$O$_5$ in Figure \ref{fig:two_comp_tables_2}a) or variables x, y in Figure \ref{fig:two_comp_tables_2}b), we perform classification at the edge level. For ease of exposition, we describe our method in this Section \ref{sec:multi-cell} for the setting that the table has been predicted by GNN$_2$ to have row-wise orientation, i.e., rows are compositions and columns are constituents. A transposed computation is done in the reverse case. Since the constituent/variable will likely occur in the same column or row as the cell containing percentage contribution, our method computes an edge feature vector: for edge $e=(i,j)\rightarrow(i',j')$, s.t. $i=i' \vee j=j' $, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{i'j'}}$.
%\textcolor{red}{and for edge $e=(i,j)\rightarrow(i',j')$, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{ij'}}$}. 
It then takes all such edges $e$ from cell $(i,j)$, if row $i$ is labeled composition and column $j$ is labeled constituent. Each edge $e$ is classified through an MLP$_4$, and the edge with maximum logit value is picked to identify constituent/variable. This helps connect 36 to P$_2$O$_5$ and 0.8 to x in our running examples. %A transposed computation is done if rows are constituents and columns are compositions.
GNN$_2$ also helps in predicting NC tables. In case none of the rows/columns are predicted as 1 or 2, then the table is deemed as NC and discarded.

%we construct an edge from every table cell to all cells with the same row/column including itself. We then select the edge with maximum logit and use a simple RE to get the constituent/variable from the cell at the other end of selected edge. Some examples of valid edges in above figures are the ones which connect 90 to Sb$_2$O$_3$, 30 to PbCl$_2$, 0.3 to y, 0.8 to x, etc.

% \subsubsection{LM-Lin-Table baseline}
% \label{sec:lm_lin_table}
% Figure \ref{fig:lm_lin_table_baseline} depicts our LM-Lin-Table baseline model. Here, LM is a pre-trained Language Model. Here, we flatten the input table row-wise after replacing the empty table cells with special [EMPTY] token. Then, we tokenize this linear table using the LM tokenizer. It's possible to obtain more than one wordpiece for some table cells. Since, the length of tokenized linear table can be greater than 512, we truncate minimum possible rows from the end so that input length to LM becomes less than or equal to 512. Let the tokenized linear table be denoted by $[t_0, t_1, \dots, t_n]$, where $t_0 = [CLS]$, $t_n = [SEP]$, $n < 512$ and the number of rows after truncation be $R'$. We then pass $[t_0, t_1, \dots, t_n]$ through the LM to obtain contextual embeddings of every wordpiece $[\overrightarrow{z_0}, \dots, \overrightarrow{z_n}]$.

% \begin{figure}[!htb]
% \begin{center}
%     \centering
%     \includegraphics[scale=0.3]{multi_cell_baseline.png}
%     \caption{Schematic of the LM-Lin-Table baseline model}
%     \label{fig:lm_lin_table_baseline}
% \end{center}
% \end{figure}

% We take the contextual embedding of first word-piece of every table cell to be representative of it. Let $0 < k_{1,1} < k_{1,2} < \dots < k_{R',C} < n$ be the indices such that $k_{i,j}$ is the index of first wordpiece of cell $(i, j)$.
% To make the baseline model aware of different row and column indexes, we add randomly initialized row and column index embeddings, so that final cell embeddings become $[\overrightarrow{h_{k_{1,1}}}, \dots, \overrightarrow{h_{k_{R',C}}}]$, where $\overrightarrow{h_{k_{i,j}}} = \overrightarrow{z_{k_{i,j}}} + \overrightarrow{rid_{i}} + \overrightarrow{cid_{j}}$, $\overrightarrow{rid_{i}}$ and $\overrightarrow{cid_{j}}$ are the $i^{th}$ row and $j^{th}$ column index embeddings respectively. For brevity, we now denote $\overrightarrow{h_{k_{i,j}}}$ by $\overrightarrow{h_{i,j}}$.
% Row and column embeddings are computed by taking average of final cell embeddings of cells occurring in that row/column i.e. $\overrightarrow{r_i} = Mean(\overrightarrow{h_{i,1}}, \dots, \overrightarrow{h_{i,C}})$ and $\overrightarrow{c_j} = Mean(\overrightarrow{h_{1,j}}, \dots, \overrightarrow{h_{R',j}})$.
% Edge embeddings are computed by concatenating the final cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. Finally, all row and column embeddings are fed to a MLP to get probabilities of every row and column belonging to 4 classes as described earlier and edge embeddings are passed through another MLP to obtain logit score for every table edge. Loss function consists of row/column cross-entropy loss and edge binary cross-entropy loss.

%\subsubsection{GAT-Multi-cell-table}

%This model is mostly similar to the model as discussed in section \ref{sec:gat_single_cell_table}. Since, we do not need to do table-level classification in this case, we remove the $(0, 0)$ table node and its edges from the graph. Here too, the contextual row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$ are obtained with the help of $LM$ and $GNN$. Then, we feed them through a MLP with softmax activation at the end to get probabilities of every row and column belonging to four classes (composition, constituent, material ID and others). Edge embeddings are computed by concatenating the contextual cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. These edge embeddings are then passed through another MLP to obtain logit score for every table edge. Training loss consists of weighted row/column cross-entropy loss and edge binary cross-entropy loss.



\textbf{Partial information table predictor:}
%Till now, we have predicted the row \&column labels and also linked the extracted percentage contributions with the corresponding constituent/variable. If all row and column labels are predicted to be 0, then we classify that table as a non-composition table.
Next, \sys\ distinguishes between complete-information (CI) and partial-information (PI) MCC tables. It uses a logistic regression model with custom input features for this prediction task. 
%We describe this assuming the table orientation is predicted to be row-oriented by GNN$_2$ (i.e., rows are compositions, columns are constituents); analogous transposed computation will be done for the reverse case. 
Let $P$ and $Q$ be the sets of all row indices with label 1 (composition) and column indices with label 2 (constituent), respectively. Also, assume $n_{ij}$ is the number present in table cell $(i, j)$ or $0$ if no number is present.  To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely an MCC-PI, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is MCC-CI. Features F4 (and F5) computes the maximum (average) of the sum of all extracted compositions. The intuition of F4 and F5 is that the higher these feature values, higher the chance of the table being an MCC-CI. Formally, 

\[
\mathrm{F4}=(\max_{i \in P} \sum_{j \in Q}n_{ij}) ~~~~~~~~~~~~~
\mathrm{F5}=(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij}).
\]

%to extract the composition tuples as described in section \ref{sec:proposed_cls_tables}. For this, we build a Logistic Regression model with custom input features.
%Assume the table to be a row-oriented table as inferred from predicted row and column labels. Let $P$ and $Q$ be the sets of all row indexes with label 1 and column indexes with label 2 respectively. Also, assume $n_{ij}$ is the first number present in table cell $(i, j)$ or $0$ if no number is there. To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely a partial-information table, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is complete information. Features F4 (and F5) computes the maximum (average) of the sum of 

%\begin{enumerate}
%    \item \textit{Number of unique variables}: If we have some variables, then it is more likely for the table to belong to partial information table class.

%    \item \textit{Number of unique constituents}: If there are many constituents, then table is more likely to be an all information table.

%    \item \textit{Maximum sum among all extracted compositions} $(\max_{i \in P} \sum_{j \in Q}n_{ij})$: Greater this quantity, greater the chances of being in all-information table class.
    
%    \item \textit{Average sum across all extracted compositions} $(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij})$: Explanation similar to above feature.

%    \item \textit{Number of rows/columns with label 2}: If there are lesser number of rows/columns with label 2, then table is probably a partial information table.

%\end{enumerate}

\textbf{MCC table extractor:} For MCC-CI, MLP$_3$ and MLP$_4$ outputs are post-processed, and units are added (similar to SCC tables), to construct final extracted tuples. For MCC-PI, on the other hand, information in text needs to be combined with the MLP outputs for final extraction. The first step here is to search for the composition expression, which may be present in table caption, table footer, and if not there, in somewhere in the rest of the research paper. Here, \sys\ resorts to using our rule-based composition parser from Figure \ref{fig:comp_parser}, but with one key difference. Now, the composition may contain variables ($x$, $y$) and even mathematical expressions like $100-x$. So the regular grammar is enhanced to replace the non-terminal NUM with a non-terminal EXPR, which represents, numbers, variables, and simple mathematical expressions over them. An added constraint is that if there are variables in set $Q$, then those variables must be present in the matched composition expression. \sys\ completes the composition by substituting the variable values from every composition row into the matched composition. There may be other types of MCC-PI tables where only compounds are identified in tables, such as Figure \ref{fig:three comp_tables}b. For these, \sys\ first computes the constituent contributions in terms of variables from composition expression, and then equates it with the numbers present in rows/columns labeled 1 (composition). In our example, \sys\ matches x with the numbers 10, 20, 30, and 40, and the rest of the composition is extracted by processing the composition expression in the caption with these values of x. Units and material IDs are added to the tuples, similar to other tables.


%After identifying the partial information Multi-cell composition tables, we try to complete the composition by searching for REs in the table caption, table footer, and then sequentially in research paper text from top to bottom. In case of variables as in Figure \ref{fig:partial_info_table_2}, we search for REs containing precisely those variables and complete the composition by substituting the variable values from every composition row. If case of constituents as in Figure \ref{fig:partial_info_table_1}, we first compute the constituent contributions in terms of variables and then equate it with the numbers present in rows/columns having label 1. For example, in terms of variables, contribution of $CsCl$ is $x/100$ for table shown in Figure \ref{fig:partial_info_table_1}. Since $0 \leq x/100 \leq 1$, we divide the numbers in table by 100. And then solve for x by equating $x/100 = 40/100$ for last row, giving $x = 40$, which completes the composition as $\{(La_2S_3, 0.2), (Ga_2S_3, 0.4), (CsCl, 0.4)\}$. Then we prepend material IDs and append units to the tuples to complete the extraction.


\subsection{Constraint-aware loss functions}
\label{sec:constraints}

\sys\ needs to train the two GNNs and the PI table predictor. Our data construction provides gold labels for each prediction task (discussed in next section), so we train these component-wise. The PI table predictor is trained on standard logistic regression loss. GNN$_1$ is trained on a weighted sum of binary cross entropy loss for SCC table classification and row/column classification for material IDs --  weight is a hyper-parameter. Similarly, GNN$_2$ loss function consists of sum of row/column cross-entropy and edge binary cross-entropy losses. 

GNN$_2$ has the more complex prediction problem, since it has to perform four-way labeling for each row and column. In initial experiments, we find that the model sometimes makes structural errors like labeling one row as constituent and another row as composition in the same table -- highly unlikely as per the semantics of composition tables. To encourage GNN$_2$ to make structurally consistent predictions, we express a set of constraints on the complete labelings, as follows. (1) A row and a column cannot both have compositions or constituents.  %(2) Compositions and constituents should be orthogonally predicted  
(2) Composition and material ID must be orthogonally predicted (i.e, if a row has a composition then ID must be predicted in some column, and vice versa). (3) Constituents and material IDs must never be orthogonally predicted (if rows have constituents then another row must have the ID). And, (4) material ID must occur at most once for the entire table. 
%Limitation of space precludes complete mathematical exposition of all constraints (see App. ~\ref{app:constraint} for details). 
As an example, constraint (1) can be expressed as a hard constraint as:
\begin{center}
\(
r_i = l \Rightarrow c_j \neq l ~~~~\forall i\in\{1,\ldots, R\}, j\in \{1,\ldots,C\}, l\in\{1,2\}. 
\)
\end{center}
Here, $r_i$ and $c_j$ are predicted labels of row $i$ and column $j$. We wish to impose these structural constraints at training time, so that the model is trained to honor them. We follow prior work by Nandwani et al. \cite{yatin}, to first convert these hard constraints into a probabilistic statement. For example, constraint (1) gets expressed as:
\begin{center}
\(
P(r_i = l; \theta) + P(c_j = l; \theta) - 1 \leq 0\) \( \forall i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}.
\)
\end{center}
$\theta$ represents GNN$_2$'s parameters. Following same work, each such constraint gets converted to an auxiliary penalty term, which gets added in the loss function for constraint-aware training. The first constraint gets converted to:
\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l; \theta) + P(c_j = l; \theta) - 1) \]
This and similar auxiliary losses for other constraints (App.~\ref{app:constraint}) get added to the GNN$_2$'s loss function for better training. $\lambda$ is a hyper-parameter. We also use constraint (4) for GNN$_1$ training.

%We augmented our GAT based models with some features/constraints to improve the performance. These bells and whistles have been discussed in the following sub-sections.

%\subsubsection{Constraints}
%\label{sec:constraints}
%In the approach presented till now, it is possible for the model to predict some row as composition row and some column as composition column and similar is the case for constituents. But practically, this does not make sense. We formulate these constraints mathematically and modify our training procedure by adding a suitable term to the loss function.

%Let $r_i$ be the label assigned by the model to row $i$ and $c_j$ be the label assigned to column $j$. We can write the hard version of these constraints as $r_i = 1 \Rightarrow c_j \neq 1$ and $r_i = 2 \Rightarrow c_j \neq 2$, where $i \in \{1, \dots, R\}$ and $j \in \{1, \dots, C\}$. We rewrite these as
%$r_i \neq l \lor c_j \neq l$ for $l \in \{1, 2\}$. In a similar fashion, labels 1 \& 3 can't occur simultaneously in rows or columns, labels 2 and 3 can't occur orthogonal to each other, and label 3 can occur at most once for the entire table.
%We convert all these hard constraints to soft constraints as done by Yatin et al. \cite{yatin} to obtain:

%\begin{enumerate}
%    \item $P(r_i = l) + P(c_j = l) - 1 \leq 0\;$ for $i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}$
    
%    \item $P(r_{i_1} = 1) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $i_1, i_2 \in \{1, \dots R\}, \; i_1 \neq i_2$
    
%    \item $P(c_{j_1} = 1) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $j_1, j_2 \in \{1, \dots C\}, \; j_1 \neq j_2$
    
%    \item $P(r_i = l) + P(c_j = 5-l) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}, \; l \in \{2, 3\}$
    
%    \item $P(r_{i_1} = 3) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $1 \leq i_1 < i_2 \leq R$
    
%    \item $P(c_{j_1} = 3) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $1 \leq j_1 < j_2 \leq C$
    
%    \item $P(r_i = 3) + P(c_j = 3) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}$

%\end{enumerate}

%We now convert these soft constraints to penalty terms and add them to the loss function. For the first soft constraint, we add
%\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l) + P(c_j = l) - 1) \]
%to the loss function for all tables $T$ in the training dataset. Here, $\lambda$ is a hyper-parameter which controls the magnitude of penalty relative to the original training loss. We add similar penalty terms for other soft constraints.

%\subsubsection{Manual features}

%Here, we introduce some task-specific features which can potentially boost the performance.

%\begin{enumerate}
%    \item \textit{Max-frequency Feature}: This feature helps to incorporate the bias that material IDs are unique. Let $f_{i}^{(r)}$ and $f_{j}^{(c)}$ denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$ respectively. If these numbers are on the lower side, then that row/column has more probability of containing material IDs. For Figure \ref{fig:nom_exp_table}, $f_1^{(r)} = 6$, $f_2^{(r)} = 2$, and $f_3^{(r)} = 3$. This is because we copy the cell contents in case of merged cells. We also set $f_0^{(r)} = f_0^{(c)} = 0$. These numbers are then mapped to learnable embeddings $(\overrightarrow{q_m}'s)$ and concatenated with $\overrightarrow{x_{ij}}$. Hence, $\overrightarrow{z_{ij}} = (\overrightarrow{x_{ij}} + \overrightarrow{p_i}) + \overrightarrow{p_j}) \; || \; (\overrightarrow{q_{f_{i}^{(r)}}} + \overrightarrow{q_{f_{j}^{(c)}}})$. Here, we take $\overrightarrow{q_{m}} = \overrightarrow{q_m'}$ for all $m > m'$ and $m'$ is a hyper-parameter. Size of $\overrightarrow{q_m}'s$ is also a hyper-parameter.
    
%    \item \textit{Boolean Regex Feature}: We use this feature while classifying Single-cell composition tables. The feature is set to true for a table cell if that cell contains a composition that can be parsed using any of our regular expressions. We map true and false to different embeddings and concatenate them with $\overrightarrow{x_{ij}}'s$ to obtain new $\overrightarrow{z_{ij}}'s$.

%\end{enumerate}

%\subsubsection{Caption node}
%Sometimes, table captions can be useful to differentiate composition tables from non-composition tables. Therefore, we add a node in the graph corresponding to table caption for Multi-cell composition tables. We represent the caption node by $(0, 0)$ and add edges from caption node to all row and column nodes. To propagate the information further to table cells, edges are added from row and column nodes to corresponding table cell nodes.


==> sections_old_v2/5_experiments.tex <==
% !TEX root = main.tex
\section{Experiments} 
\label{sec:experiments}
%\subsection{Dataset}
%\begin{wraptable}{R}{0.4\textwidth}
%\vspace{-0.15in}
%\centering
%\caption{\small Statistics of table types in all three splits}
%\begin{tabular}{lccc}
%    \toprule &
%    \multicolumn{3}{c}{ \textbf{Splits}}\\
%    \cmidrule(lr){2-4}
%    \textbf{Table Type} &  \textbf{Train} & \textbf{Dev} & \textbf{Test} \\
%    \midrule
%    SCC & 704 & 110 & 113 \\
%    MCC-CI & 626 & 132 & 132 \\
%    MCC-PI & 317 & 109 & 112 \\
%    NC & 2761 & 387 & 380 \\
%    \midrule
%    Total & 4408 & 738 & 737 \\
%    \bottomrule
%\end{tabular}
%\label{tab:dataset_stats}
%\vspace{-0.2in}
%\end{wraptable}
% \textbf{Dataset construction:} % moved to appendix
% \textbf{Dataset details:} We match a manually-curated KB of materials and compositions with tables in the relevant papers, to automatically provide distantly-supervised labels for extraction (hand-annotated for dev/test sets). This results in 5,883 tables from 2536 publications, of which 2,355 express compositions, with 16,729 materials, and a total of 58,481 (material ID, constituent, composition percentage, unit) tuples.\\

\textbf{Baseline models: }
% We implement \sys\ with $LM$ as \textsc{MatSciBERT} \cite{gupta_matscibert_2022}, and the GNNs as Graph Attention Networks \cite{velickovic2018graph}. We compare \sys\ with six non-GNN baseline models. Our first baseline is \textsc{TaPas} \cite{herzig-etal-2020-tapas}, a state-of-the-art table QA system, which flattens the table, adds row and column index embeddings, and passes as input to a language model. To use TaPas for our task, we use table caption as proxy for the input question. All the model parameters in this setting are initialized randomly. Our second baseline is \textsc{TaPas-Adapted}, with the goal of providing the benefit of \textsc{MatSciBERT} to  \textsc{TaPas} -- it initializes language model weights by \textsc{MatSciBERT}. For the input to remain consistent with \textsc{MatSciBERT}, we add row and column index embeddings to \textsc{MatSciBERT} \emph{output}, instead of input as in original \textsc{TaPas} model. The third baseline model is \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation. Similar to \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} uses \textsc{MatSciBERT} as the LM instead of \textsc{BERT}. 
% \textcolor{red}{We use TABBIE as our fifth baseline model, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. It's architecture mainly consists of two transformers that independently encode information across rows and columns and their representations are pooled after each layer for getting the overall table information. Likewise, \textsc{TABBIE-ADAPTED} uses \textsc{MatSciBERT} as the LM}. 
% Further details on baselines in App.~\ref{app:baseline}.
We implement \sys\ with $LM$ as \textsc{MatSciBERT} \cite{gupta_matscibert_2022}, and the GNNs as Graph Attention Networks \cite{velickovic2018graph}. We compare \sys\ with six non-GNN baseline models. Our first baseline is \textsc{TaPas} \cite{herzig-etal-2020-tapas}, a state-of-the-art table QA system, which flattens the table, adds row and column index embeddings, and passes as input to a language model. To use TaPas for our task, we use table caption as proxy for the input question. All the model parameters in this setting are initialized randomly. 
Next, we use \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation.
Finally, we use \textsc{TABBIE}, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. 
% It's architecture consists of two transformers that independently encode information across rows and columns after which representations are pooled at each layer.
Additionally, we replace the LM of all models with \textsc{MatSciBERT} to provide domain specific embeddings to obtain the respective \textsc{Adapted} versions. Further details on baselines in App.~\ref{app:baseline}.
% \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} and \textsc{TABBIE-Adapted} with the goal of providing the benefit of \textsc{MatSciBERT} to  \textsc{TaPas} -- it initializes language model weights by \textsc{MatSciBERT}. For the input to remain consistent with \textsc{MatSciBERT}, we add row and column index embeddings to \textsc{MatSciBERT} \emph{output}, instead of input as in original \textsc{TaPas} model. 
% The third baseline model is \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation. Similar to \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} uses \textsc{MatSciBERT} as the LM instead of \textsc{BERT}. 
% \textcolor{red}{We use TABBIE as our fifth baseline model, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. It's architecture mainly consists of two transformers that independently encode information across rows and columns and their representations are pooled after each layer for getting the overall table information. Likewise, \textsc{TABBIE-ADAPTED} uses \textsc{MatSciBERT} as the LM}. 
% Further details on baselines in App.~\ref{app:baseline}.



%{$\bullet$ \bf \textsc{TaPas}:} This has the same architecture as proposed by Herzig et al. \cite{herzig-etal-2020-tapas} for Table-QA task. Here, row and column index embeddings are passed as input to $LM$. All the model parameters are initialized randomly. We use table caption as a proxy for the input question.\\
%{\bf $\bullet$ \textsc{TaPas-Adapted}:} Here, we initialize \textsc{TaPas} with $LM$ pre-trained weights for a fair comparison with \sys. Also, for the input to remain consistent with the original $LM$, we add row and column index embeddings to the $LM$ output and we do not include caption in the input. We term this modified model as \textsc{TaPas-Adapted}. 

%The input table is flattened row-wise and passed through these two baseline models. We provide the precise details in Appendix.

\begin{table*}[htb]
\centering
\scalebox{0.85}{
\begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} &  \textbf{CV} \\
    \midrule
    
    \textsc{TaPas} & 80.37 ($\pm$ 4.78) & 71.23 ($\pm$ 0.77) & 49.88 ($\pm$ 0.10) & 543.67 \\
    \textsc{TaPas-Adapted} & \textbf{89.65} ($\pm$ 0.46) & 70.91 ($\pm$ 3.79) & 57.88 ($\pm$ 2.73) & 490.33 \\
    \textsc{TaBERT} & 79.61 ($\pm$ 8.25) & 58.20 ($\pm$ 1.79) & 47.05 ($\pm$ 1.50) & 1729.67 \\
    \textsc{TaBERT-Adapted} & 85.07 ($\pm$ 6.28) & 59.31 ($\pm$ 0.67) & 50.10 ($\pm$ 2.86) & 1195.67 \\
    \textsc{TABBIE} & 80.99 ($\pm$ 2.41) & 50.90 ($\pm$ 3.34) & 47.03 ($\pm$ 2.14) & \textbf{388.00} \\
    \textsc{TABBIE-Adapted} & 80.18 ($\pm$ 5.38) & 53.20 ($\pm$ 5.57) & 48.89 ($\pm$ 2.73) & 728.67 \\
    % \textsc{TaPas-Adapted} & 86.80 ($\pm$ 0.50) & 70.43 ($\pm$ 2.01) & 56.67 ($\pm$ 4.67) & 424.33 \\
    \textsc{v-}\sys & 77.38 ($\pm$ 12.21) & \textbf{76.52} ($\pm$ 2.37) & \textbf{64.71} ($\pm$ 3.45) & 626.33 \\
    \bottomrule
\end{tabular}
}
\caption{Performance of \textsc{v-}\sys{} vs baseline models on MCC-CI and NC table types. Refer to Evaluation metrics (Section 5) for detailed  definitions of these metrics.}
\label{tab:baselines}
\vspace{-0.10cm}
\end{table*}

% \begin{table*}[htb]
% \centering
% %\vspace{-2ex}
% \scalebox{0.85}{
% \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Model} & \textbf{TT Acc.} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
%     \midrule
    
%     \sys & 88.35 ($\pm$ 1.20) & 82.40 ($\pm$ 3.88) & \textbf{70.14} ($\pm$ 0.44) & \textbf{63.51} ($\pm$ 1.90) & 87.33 \\
%     \midrule

% \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 80.80 ($\pm$ 3.24) & 68.60 ($\pm$ 1.26) & 62.53 ($\pm$ 1.89) & 120.11 \\
%     \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 78.71 ($\pm$ 3.66) & 69.28 ($\pm$ 1.11) & 60.94 ($\pm$ 0.98) & 584.78 \\
%     \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.23} ($\pm$ 0.51) & 67.51 ($\pm$ 1.36) & 63.50 ($\pm$ 2.49) & \textbf{19.11} \\
%     \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 68.54 ($\pm$ 9.32) & 65.98 ($\pm$ 1.21) & 59.36 ($\pm$ 2.20) & 541 \\
    
%     \bottomrule
% \end{tabular}
% }
% \caption{Contribution of task specific features and constraints in \sys.}
% \label{tab:ablations}
% \vspace{-0.1in}
% \end{table*}
\begin{table*}[htb]
\centering
%\vspace{-2ex}
\scalebox{0.85}{
\begin{tabular}{lccccc}
    \toprule
    \textbf{Model} & \textbf{TT Acc.} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
    \midrule
    
    % \sys & 88.35 ($\pm$ 1.20) & 82.40 ($\pm$ 3.88) & \textbf{70.14} ($\pm$ 0.44) & \textbf{63.51} ($\pm$ 1.90) & 87.33 \\
    \sys & 88.35 ($\pm$ 1.20) & 84.57 ($\pm$ 2.16) & \textbf{70.04} ($\pm$ 0.69) & \textbf{63.53} ($\pm$ 1.45) & 75.22 \\
    \midrule

    % \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 80.80 ($\pm$ 3.24) & 68.60 ($\pm$ 1.26) & 62.53 ($\pm$ 1.89) & 120.11 \\
    \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 84.15 ($\pm$ 1.61) & 68.31 ($\pm$ 1.45) & 62.47 ($\pm$ 1.98) & 83.11 \\
    % \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 78.71 ($\pm$ 3.66) & 69.28 ($\pm$ 1.11) & 60.94 ($\pm$ 0.98) & 584.78 \\
    \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 84.07 ($\pm$ 0.83) & 69.68 ($\pm$ 1.21) & 61.44 ($\pm$ 1.00) & 434.44 \\
    % \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.23} ($\pm$ 0.51) & 67.51 ($\pm$ 1.36) & 63.50 ($\pm$ 2.49) & \textbf{19.11} \\
    \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.76} ($\pm$ 0.68) & 66.82 ($\pm$ 1.90) & 62.68 ($\pm$ 3.33) & \textbf{17.89} \\
    % \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 68.54 ($\pm$ 9.32) & 65.98 ($\pm$ 1.21) & 59.36 ($\pm$ 2.20) & 541 \\
    \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 76.61 ($\pm$ 6.16) & 66.15 ($\pm$ 2.00) & 59.52 ($\pm$ 3.33) & 380.11 \\
    
    \bottomrule
\end{tabular}
}
\caption{Contribution of task specific features and constraints in \sys. Refer to Evaluation metrics (Section 5) for detailed  definitions of these metrics.}
\label{tab:ablations}
\vspace{-0.1in}
\end{table*}

\begin{table}[!htb]
% \vspace{-1.5cm}
\centering
\scalebox{0.75}{
\begin{tabular}{ccccc}
    \toprule
    \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} \\
    \midrule
    
    SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) \\
    
    MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) \\
    
    MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) \\

    \bottomrule
\end{tabular}
}
\caption{\sys{} performance on the table-types.}
\label{tab:perf_table_types}
\vspace{-0.25in}
\end{table}

%\subsection{Evaluation metrics}
\textbf{Evaluation metrics:} 
We compute several metrics in our evaluation. (1) \emph{Table-type (TT) prediction accuracy} -- it computes table-level accuracy on the 4-way table classification as NC, SCC, MCC-CI and MCC-PI. 
(2) \textit{ID F$_1$ score} computes F$_1$ score for Material ID extraction.  
(3) \textit{Tuple-level (TL) F$_1$ score} evaluates performance on the extraction of composition tuples. A gold is considered matching with a predicted 4-tuple if \emph{all} arguments match exactly. 
(4) \textit{Material-level (MatL) F$_1$ score} is the strongest metric. It evaluates whether all predicted information related to a material (including its ID, all constituents and their percentages) match exactly with the gold.
Finally, (5) \textit{constraint violations (CV)} counts the number of violations of hard constraints in the prediction. We consider all four types of constraints, as discussed in Section \ref{sec:constraints}. %\end{enumerate}
%Thus, TL precision means how many, out of all the tuples model predict, are correct. Similarly, TL recall means how many, out of all the gold tuples, were predicted by the model. TL F$_1$ score is the harmonic mean of TL precision and recall.\\
%$\bullet$\textit{Composition-level (CL) metrics}: This set of metrics evaluate model at the composition level. So, CL precision means out of all the compositions (set of tuples) model predict, how many of them were completely correct. Similarly, CL recall means out of all the gold compositions, how many were exactly predicted by the model. CL F$_1$ score is the harmonics mean of CL precision and CL recall.\\  
% \textbf{Implementation details: }
% %In our experiments, we take the $LM$ as MatSciBERT \cite{gupta_matscibert_2022} which is a materials-science domain specific language model and we choose $GNN$ to be 
% For Graph Attention Networks (GATs) \cite{velickovic2018graph}, we use the GAT implementation of Deep Graph Library \cite{dgl_citation_wang2019}. For LMs, \textsc{TaPas}, we use the implementation by Transformers library \cite{transformers_huggingface}. We use \textsc{TaBERT}'s source code from their github repository. We implement and train all models using PyTorch  \cite{pytorch_NEURIPS2019_9015}. We optimize the model parameters using Adam \cite{adam_opt_kingma} and a triangular learning rate \cite{triangle_lr}. We further use different learning rates for $LM$ and non-LM parameters (GNNs, MLPs) (App.~\ref{app:hyperparameter}). To deal with imbalanced labels, we scale loss for all labels by weights inversely proportional to their frequency in the training set. All experiments were run on a machine with one 32 GB V100 GPU. Each model is run with three seeds and the mean and std. deviation are reported. 
Implementation details are mentioned in App.~\ref{app:implementation}. The code and data is available \href{https://anonymous.4open.science/r/DiSCoMaT-EEFB/}{here}.
\vspace{-1ex}
%\vspace{-0.5cm}
\subsection{Results}
%\vspace{-0.2cm}
\emph{How does table linearization compare with a graph-based model for our task?} To answer this question,  we compare \sys{} with four models that use linearization: {\sc TaPas}, \textsc{TaBERT}, and their adapted versions. \textsc{TaPas} and \textsc{TaBERT} do table level and row level linearizations respectively. Since the baselines do not have the benefit of regular expressions, features, and constraints, we implement a version of our model without these, which we call \textsc{v-}\sys. We do this comparison, trained and tested only on the subset of MCC-CI and NC tables, since other table types require regular expressions for processing. As shown in Table \ref{tab:baselines} \textsc{v-}\sys{} obtains 6-7 pt higher F$_1$ on TL and MatL scores, suggesting that a graph-based extractor is likely a better fit for our problem - this led to us choosing a GNN-based approach for \sys. 

%\textsc{TaPas} and \textsc{TaPas-Adapted} as shown in Table \ref{tab:baselines}. For simplicity, we train and evaluate all three models on MCC-CI and NC tables only. We refer to \sys{} without max-frequency feature, constraint loss, and caption node as Vanilla-\sys{} or in short \textsc{V-}\sys.

\emph{How does \sys{} perform on the complete task?}
Table \ref{tab:ablations}, reports \sys{} performance on the full test set with all table types. 
%Here, we have 3 set of parameters for GNN$_1$ and 3 set of parameters for GNN$_2$ corresponding to 3 seeds. Hence, we report results averaged over 9 ordered pair of seeds.
Its ID and tuple F$_1$-scores are 82 and 70, respectively. Since these errors get multiplied, unsurprisingly, its material-level F$_1$-score is lower (63.5). Table \ref{tab:perf_table_types} reports \sys{} performance for different table types. In this experiment, we assume that table type is already known and run only the relevant part of \sys{} for extraction. We find that MCC-PI is the hardest table type, since it requires combining information from text and tables for accurate extraction. A larger standard deviation in ID F$_1$ for MCC-PI is attributed to the fact that material IDs occur relatively rarely for this table type -- the test set for MCC-PI consists of merely 20 material ID rows and columns.

\emph{What is the incremental contribution of task-specific features and constraints?}
Table \ref{tab:ablations} also presents the ablation experiments. \sys{} scores much higher that \textsc{v-}\sys, which does not have these features and constraints. We also perform additional ablations removing one component at a time. Unsurprisingly constrained training helps with reducing constraint violations. Both constraints and features help with ID prediction, due to constraints (2), (3), (4) and max frequency feature. Removal of caption node significantly hurts performance on MCC-PI tables, as these tables require combining caption with table cells. All contribute to the tuple-level metric. 

\emph{What are the typical errors in \sys?} 
Confusion matrix in Figure \ref{fig:confusion} suggests that most table type errors are between MCC-PI and NC tables. This could be attributed to following reasons. (i) \sys{} has difficulty identifying rare compounds like Yb$_2$O$_3$, ErS$_{3/2}$, Co$_3$O$_4$ found in MCC-PI---these aren't present frequently in the training set. (ii) MCC-PI tables specify dopant percentages found in small quantities. %are also a source of error. %Generally the text contains a base composition (summing to 100), in which dopant is added. Finding the base composition in paper text corresponding to dopants mentioned in the table is non-trivial. Sometimes, instead of percentage contributions being expressed as variables, constituents are specified as variables. 
(iii) Completion of composition in MCC-PI tables may require other tables from the same paper. (iv) Finally, MCC-PI composition may contain additional information such as properties that may bias the model to classify it as  NC. Some corner cases are given in App.~\ref{app:corner}. %Yet another case is when caption mentions silicates/phosphates and hence remaining constituent is SiO$_2$/P$_2$O$_5$.
%\vspace{-0.1in}
\begin{wrapfigure}{r}{0.25\textwidth}
    \vspace{-0.1in}
    \centering
    \includegraphics[width=0.25\textwidth]{confusion_matrix.png}
    \vspace{-0.15in}
    \caption{Confusion matrix for all table types}
    \label{fig:confusion}
    \vspace{-0.30in}
\end{wrapfigure}
%Table \ref{tab:perf_table_types} shows the performance of \sys{} (averaged over three seeds) on individual table types. In these experiments, we assume that table type is already known. For SCC, we use GNN$_1$ just for materials ID prediction and Rule-based composition parser to parse compositions from table cells. From CL F$_1$-score, we can observe that \sys performs best on SCC, then MCC-CI, and then MCC-PI. Large standard deviation in Material IDs F$_1$-Score for MCC-PI can be attributed to the fact that Material IDs occur relatively rarely for this table type. Test set for MCC-PI consists of merely 20 Material ID rows and columns.

% \begin{wraptable}{R}{0.6\textwidth}
% \vspace{-1.5cm}
% \centering
% \caption{Performance of \sys{} on different table types}
% \scalebox{0.75}{
% \begin{tabular}{ccccc}
%     \toprule
%     \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
%     \midrule
    
%     SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) & 0.67 \\
    
%     MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) & 59.33 \\
    
%     MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) & 26.67 \\

%     \bottomrule
% \end{tabular}
% }
% \label{tab:perf_table_types}
% % \vspace{-0.2cm}
% \end{wraptable}


==> sections_old_v2/6_conclusions.tex <==
\vspace{-0.25cm}
\section{Conclusions} 
\label{sec:conclusions}
\vspace{-0.15cm}
We define the novel task of extracting material compositions from tables in scientific papers. We harvest a dataset using distant supervision, combining information from a MatSci DB with tables in respective papers. We present a strong baseline system, \sys, a pipeline based on LM, GNNs, and task-specific regex, %, which is a pipeline of a material science language model, two graph neural networks along with task-specific regular expressions, features and constraints. Our experiments show 
that outperforms other architectures that linearizes the tables. We plan to extend it to extract material properties as well. \\
\textbf{Limitations and outlook:} \sys\ is a pipelined solution trained component-wise. This raises a research question: can we train one end-to-end trained ML model that not only analyzes a wide variety of table structures, but also combines understanding of regular expressions, extraction of chemical compounds and scientific units, text understanding and some mathematical processing. This defines a challenging ML research question, and one that can have direct impact to the scientific MatSci community. \\
Indeed, automating parts of scientific discovery through such NLP-based approaches has the potential of biases and errors. Note that wrong and biased results can lead to erroneous information about materials. To a great extent this issue is addressed as we rely only on published literature. The issue could be further addresses by considering larger datasets covering wider range of materials.

==> sections_old_v2/7_acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:checklist}

% This document has been adapted
% by Steven Bethard, Ryan Cotterell and Rui Yan
% from the instructions for earlier ACL and NAACL proceedings, including those for 
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan, 
% NAACL 2017 by Margaret Mitchell, 
% ACL 2012 by Maggie Li and Michael White, 
% ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
% ACL 2002 by Eugene Charniak and Dekang Lin, 
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections_old_v2/7_checklist.tex <==
% !TEX root = main.tex
\section*{Checklist}
\label{sec:checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> sections_old_v3/0_abstract.tex <==
%Tables in scientific articles carry important information (often numeric), which must be adequately extracted for a comprehensive machine understanding of an article. Our paper studies information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction.  Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also develop \sys, a strong baseline for the task, which combines graph neural networks with several problem-specific regular expressions, features and constraints. Our experiments evaluate the contribution of each model component in the final performance. We release our code and data for further research.

A crucial component in the curation of KB for a scientific domain is information extraction from tables in the domain's published research articles. To facilitate research in this direction, we define a novel NLP task of extracting compositions of materials (e.g., glasses) from tables in material science papers. The task involves solving several challenges in concert, such as tables that mention compositions have highly varying structures;  text in captions and full paper needs to be incorporated along with data in tables; and regular languages for numbers,  chemical compounds, composition expressions must be integrated in the model. 
We release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present \sys, a strong baseline that combines multiple graph neural networks with several task-specific regular expressions, features, and constraints. We show that \sys{} outperforms recent table processing architectures by significant margins. 
%Our experiments also assess the value of additional modifications on the final performance of the model. 
We release our code and data for further research.

%Most of the work on table extraction assumes prior knowledge on the table structure and format---a scenario that may not hold true for tables from scientific literature. A generic framework that can mine information from tables is crucial for the development of knowledge bases in several engineering and scientific domains. To address this challenge, we take a holistic view on information extraction from scientific tables in the context of extracting compositions of materials (e.g., glasses, alloys). We first observe that material science researchers organize similar composition information in a wide variety of table styles, necessitating an intelligent model for table understanding and composition extraction. Consequently, we define this novel task as a challenge for the ML community, and release a training dataset comprising 4,408 distantly supervised tables, along with 1,475 manually annotated dev and test tables. We also present a strong baseline for the task, \sys, which combines graph neural networks with several problem-specific regular expressions, features, and constraints. We show that \sys outperforms other existing models. Our experiments also evaluate how additional modifications can enhance the final performance of the model. We release our code and data for further research.

%-- progress on the task will hopefully lead to the construction of a large repository of materials (and subsequently their properties) known to mankind.

%Vast amount of Materials Science-specific information like compositions and properties is stored in tables, images and text of research publications. Since property extraction can only be performed after composition extraction, we focus on extracting compositions from tables.
% missing motivation to extract compositions from tables instead of text
%This paper is a first attempt to solve this problem and no annotated datasets are publicly available.
%First, we formally define a new problem to the ML community.
%Second, to motivate the problem, we perform extensive analysis of the ways in which compositions are reported and highlight various facets of the problem.
%Third, we share a dataset comprising of 4408 distantly supervised training tables, along with 738 and 737 manually annotated dev and test tables respectively.
%Fourth, we propose a strong baseline model based on Graph Attention Networks (GATs) \cite{velickovic2018graph} and MatSciBERT \cite{gupta_matscibert_2022} (pre-trained BERT-based Language Model).
% can mention results, bert based based baseline
%\footnote{Code and data are available at: \url{https://github.com/}.}
%\end{comment}

==> sections_old_v3/1_introduction.tex <==
% !TEX root = main.tex
\section{Introduction}
\label{sec:intro}

Advanced knowledge of a science or engineering domain is typically found in domain-specific research papers. Information extraction (IE) from scientific articles develops ML methods to automatically extract this knowledge for curating large-scale domain-specific KBs (e.g., \cite{ernst-bmc15,hope-naacl21}). These KBs have a variety of uses: they lead to ease of information access by domain researchers \cite{tsatsaronis-bmc15,hamon-sw17}, provide data for developing domain-specific ML models \cite{nadkarni-akbc21}, and potentially help in accelerating scientific discoveries \cite{materials_project, challenges_21}. 

Significant research exists on IE from \emph{text} of research papers (see \cite{nasar-scientometrics18} for survey), but less attention is given to IE (often, numeric) from tables. Tables may report performance of algorithms on a dataset, quantitative results of clinical trials, or other important information. Of special interest to us are tables that mention the composition and properties of an entity. Such tables are ubiquitous in various fields such as food and nutrition (tables of food items with nutritional values) \cite{Cavalcanti2021DonkeyMA, Stokvis2021EvaluationOT}, fuels (constituents and calorific values) \cite{Kar2022EffectOF, Beliavskii2022EffectOF}, building construction (components and costs) \cite{Aggarwal2022ComponentRC}, materials (constituents and properties) \cite{keshri2022elucidating}, medicine (compounds with weights in drugs) \cite{kalegari2014chemical}, and more. 

% \textcolor{red}{In materials science (MatSci) articles, the details on synthesis and characterization are reported in the text~\cite{mysore-etal-2019-materials}, while material compositions are mostly reported in tables~\cite{jensen2019machine}}. 
In materials science (MatSci) articles, the details on synthesis and characterization are reported in the text~\cite{mysore-etal-2019-materials}, while material compositions are mostly reported in tables~\cite{jensen2019machine}.
A preliminary analysis of MatSci papers reveals that $\sim$85\%\footnote{estimated by randomly choosing 100 compositions from a MatSci database and checking where they are reported} of material compositions and their associated properties (e.g., density, stiffness) are reported in tables and not text. %\todo{M: I added "not text" -- can you check if this is still 85\%} 
Thus, IE from tables is essential for a comprehensive understanding of a given paper, and for increasing the coverage of resulting KBs. To this extent, we define a novel NLP task of extraction of materials (via IDs mentioned in paper), constituents, and their relative percentages. For instance, Fig.\ref{fig:three comp_tables}a should output four materials A1-A4, where ID A1 is associated with three constituents (MoO$_3$, Fe$_2$O$_3$, and P$_2$O$_5$) and their respective percentages, 5, 38, and 57. 

% \begin{figure}[t]
% \begin{center}
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{multi_cell_comp_table_1_S0022309303003624.png}
%         \label{fig:multi_cell_comp_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{\scriptsize Glass compositions in the paper: $20La_2S_3-(80 - x)Ga_2S_3-xCsCl$.}
%         \includegraphics[width=\textwidth]{partial_info_table_1_S0022309399000617.png}
%         \label{fig:partial_info_table_1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \caption{}
%         \includegraphics[width=\textwidth]{single_cell_S0022459614003995.png}
%         \label{fig:single_cell_comp_table}
%     \end{subfigure}
%     \vspace{-0.3cm}
%     \caption{\small Examples of composition tables (a) Multi-cell complete-info composition table (b) Multi-cell partial-info composition table (c) Single-cell composition table }
%     \label{fig:three comp_tables}
%     \vspace{-0.6cm}
% \end{center}
% \end{figure}

\begin{figure*}[t]
\begin{center}
    \centering
    \includegraphics[width=\textwidth]{figure_1.png}
    \caption{Examples of composition tables (a) Multi-cell complete-info \cite{fig_1a_mcc_all} (b) Multi-cell partial-info {with caption on top} \cite{fig_1b_mcc_pi} (c) Single-cell \cite{fig_1c_scc}}
    \label{fig:three comp_tables}
    \vspace{-0.6cm}
\end{center}
\end{figure*}

A model for this task necessitates solving several challenges. First, compositions in MatSci papers are expressed in widely varying table styles. Two main types are \emph{multi-cell compositions} (MCC), where a material composition is presented in multiple cells %and constituents are on two axes %\todo{T: constituents are not always on the same axes. M: how will you describe differently. T: all constituents and their contribution are in table} 
%with each cell representing the percentage 
(Fig.~\ref{fig:three comp_tables}a), and \emph{single-cell compositions} (SCC), where the full composition is mentioned in a single cell as an expression (Fig.~\ref{fig:three comp_tables}c). Second, tables may have incomplete information, which requires reading caption or paper text for complete understanding (Fig.~\ref{fig:three comp_tables}b). Third, there is a need to integrate regular expression processing (such as for chemical compounds, numbers, units and composition expression in SCC tables) within the IE model. 
Fourth, there can be four units for specifying the percentage -- mol\%, mol fraction, wt.\% or wt. fraction, requiring normalization. Finally, IE can benefit from constraint processing, e.g., percentages should sum to hundred. See Appendix ~\ref{sec:problem} for further discussion on challenges. %Interestingly, some researchers write percentages such that they add to numbers less than or more than 100, and expect the reader to re-normalize. 
% All these and more make the problem of extracting material compositions from scientific tables a challenging problem. 
While many of these issues have been investigated separately (e.g., numerical IE \cite{madaan-aaai16}, unit extraction \cite{sarawagi14}, chemical compound identification \cite{weston2019named}, NLP for tables \cite{jensen2019machine,swain2016chemdataextractor}), solving all these in concert creates a challenging testbed for the NLP community. 

Here, we harvest a distantly supervised training dataset of 4,408 tables and 38,799 composition-constituent tuples by aligning a MatSci database with tables in papers. We also label 1,475 tables manually for dev and test sets. We build a baseline system \sys, which uses a pipeline of a domain-specific language model \cite{gupta_matscibert_2022}, and two graph neural networks (GNNs), along with several hand-coded features and constraints. We evaluate our system on accuracy metrics for various subtasks, including material ID prediction, tuple-level predictions, and material-level complete predictions. We find that \sys's GNN architecture obtains $\sim$15 point increase in accuracy numbers, compared to table processors \cite{herzig-etal-2020-tapas, yin-etal-2020-tabert}, which linearize the table for IE. %by a language model. 
Subsequent analysis reveals common sources of \sys\ errors, which will inform future research. We release all our data and code for further research on this challenging task.

% pleas use these short forms in the paper
%\begin{table}
 %   \centering
  %  \begin{tabular}{ll} 
   %     \toprule
    %    Table Type & Meaning \\
     %   \midrule
      %  SCC table & Single-cell composition table \\
       % MCC-CI table & Multi-cell composition complete-info table \\
       % MCC-PI table & Multi-cell composition partial-info table \\
       % NC table & Non-composition table \\
    %    \bottomrule
    %\end{tabular}
%\end{table}

% Motivation to CL Community: IE tasks have either been studied from text, or from tables with well-defined/known structures. Our task is challenging for NLP because (1) tables that mention compositions have highly varying structures; (2) text in captions and full paper needs to be incorporated along with data in tables for IE; (3) processing is needed for regular languages: numbers, units, chemical compounds, compositions expressions; (4) there are additional math constraints (e.g., percentages summing to 100). While many of these issues have been investigated separately (e.g., NLP papers on numerical IE, unit extractors, chemical compound identification, NLP for tables, etc.), solving all these challenges in concert creates a challenging testbed for the NLP community.
% Task is too specific: Extracting information from scientific articles is a broad theme of vast importance. We posit that the specific task considered by us will have ramifications for similar tasks in many other disciplines, such as food and nutrition (tables of foods with nutritional values) [1,2], fuels (constituents and calorific values) [3,4], building construction (costs of components) [5,6], medicines (compounds with weights), and more. Please see these references for the broad relevance of our work. The approach is built on the notion that there are two main styles of writing compositions – one in single cells as a long pattern, and other in multiple cells of the table. Similarly, some constituents may be implied (or mentioned in caption/text) and hence not needed in tables. These two notions are generic and should apply in other domains too. The specific lists of compounds, or units are specific and will need to be reworked for a new domain – but those are minor aspects of the solution.
% Material Science focus: It is indeed true that our paper has the strongest linkage to material science. But, similar focused CL papers have been published earlier, e.g., a paper on material science at EMNLP [7], a paper on chemical compounds at EMNLP [8], financial NER at ACL [9] and more. We expect our method to be adaptable to other similar tasks – the domain-specific features and engineering are relatively small parts of the paper.


==> sections_old_v3/2_related_work.tex <==
% !TEX root = main.tex
\section{Related work} 
\label{sec:related_work}
%Information extraction (IE) is instrumental for knowledge base creation. 
%While most of the earlier works on information extraction (IE) focusses on rule-based approaches \cite{chiticariu-etal-2013-rule}, large datasets, computational efficiency, and success of neural models lead to machine learning-based IE systems\cite{chiticariu-etal-2013-rule}.
\vspace{-0.075in}
Recent works have developed neural models for various NLP tasks based on tabular data, \textit{viz}, tabular natural language inference \cite{tnli_orihuela2021natural, xinfotabs}, QA over one or a corpus of tables \cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr, chemmengath-emnlp21}, table orientation classification\cite{deeptable_habibi2020,nishida2017understanding}, and relation extraction from tables \cite{relation_ex_tables_2013, neurel_relex_2}. Several recent papers study QA models---they all linearize a table and pass it to pre-trained language model. For example, 
\textsc{TaPas} \cite{herzig-etal-2020-tapas} does this for Wikipedia tables to answers natural language questions by selecting table cells and aggregation operators. \textsc{TaBERT} \cite{yin-etal-2020-tabert} and RCI \cite{feifei_row_col_interact} also use similar ideas alongside some architectural modifications to handle rows and columns better. \textsc{TABBIE} \cite{tabbie} consists of two transformers that encode rows and columns independently, whereas \textsc{TaPEx} uses encoder-decoder architecture using BART. TABBIE and \textsc{TaPEx} also introduce pre-training over tables to learn table representations better. Similar to our work, tables have also been modeled as graphs for sequential question answering over tables \cite{muller_acq_2019}. However, all these works generally assume a fixed and known structure of tables with the same orientation, with the top row being the header row in all cases -- an assumption violated in our setting. 
%uses a different pre-training objective and model architecture to jointly learn NL sentence and table representations. Row and column intersection (RCI) model \cite{feifei_row_col_interact} predicts the probability of finding the answer to a given question in each row and column of a table independently, without any pre-training on tables. \textsc{TaPEx} \cite{tapex} uses a BART encoder-decoder architecture, pre-trained via synthetic executable programs to mimic the behaviour of SQL execution engine. \textsc{TABBIE} \cite{tabbie} consists of two transformers that encode rows and columns independently and is pre-trained using the corrupt-cell objective. 
%TABBIE performs better than other models on table-based tasks such as column type prediction. 
%Similar to our work, tables have also been modeled as graphs for sequential question answering over tables \cite{muller_acq_2019}. However, all these works generally assume a fixed and known structure of tables with the same orientation, with the top row being the header row in all cases -- an assumption violated in our setting. 
%The table orientation and header row are assumed to be fixed for this problem. 
\\
{\bf Orientation and semantic structure classification:} %of tables has also been attempted using neural models.
DeepTable \cite{deeptable_habibi2020} is a permutation-invariant neural model, which classifies tables into three orientations, while TabNet \cite{nishida2017understanding} uses RNNs and CNNs in a hybrid fashion to classify web tables into five different types of orientations. \textsc{InfoTabS} \cite{infotabs} studies natural language inference on tabular data via linearization and language models, which has been extended to the multilingual setting \cite{xinfotabs}, and has been combined with knowledge graphs \cite{transkblstm}. Some earlier works also focused on annotating column types, entity ID cells, and pair of columns with binary relations, based on rule-based and other ML approaches, given a catalog~\cite{sunita_iitb}.%consisting of types, entities and relations .
%. Here, concatenated premise-hypothesis pair is sent through language models to classify whether the premise (info-box) entails, contradicts, or is unrelated to a given hypothesis. 
%However, these info-boxes are special type of tables containing two columns: first containing keys and other containing values. 
%This has been extended to the multilingual setting \cite{xinfotabs}, and has been combined with knowledge graphs \cite{transkblstm}. 
%Extending this, Minhas et al. \cite{xinfotabs} released a multilingual TNLI dataset comprising of info-boxes from ten different languages.  Further, TransKBLSTM model was proposed by Varun et al. \cite{transkblstm} to augment TNLI models with knowledge graphs. 

%There has also been work on annotating column types, cells with entity IDs, pair of columns with binary relations, etc given a catalog consisting of types, entities and relations \cite{sunita_iitb}. But again in this work, they take simple tables with fixed header and no merged rows or columns. 

%But their graph structure is different than ours as the table orientation and header row is fixed for their dataset.

%Distant Supervision, proposed by Mintz et al. \cite{mintz-etal-2009-distant}, is an approach to create a noisy dataset and does not require labelled data. This method is generally used to annotate any given sentence with the relations it might express. In our work, we use a similar approach where we use the Interglad database to annotate our training set.

%{\bf NLP for materials literature:} After the success of BERT \cite{devlin2018bert}, numerous domain-specific language models have been released for  public-use. For MatSci domain, researchers have contributed language models like MatSciBERT \cite{gupta_matscibert_2022}, MatBERT \cite{matbert_2022}, and BatteryBERT \cite{batterybert_2022}. MatBERT \cite{matbert_2022} highlights the advantages of materials domain-specific pre-training on the NER task. BatteryBERT  exhibits superior performance on battery related downstream tasks. MatSciBERT  yields state of the art performance on downstream tasks of abstract classification, NER, and relation classification, and we use it in our work. Wang et al. \cite{wang_automated_2022} recently develop a rule-based NER and relation extraction to create a pipeline for extracting superalloy data from text and tables. There also exists a table extraction tool that takes input HTML or XML of MatSci research papers, and uses regular expression based parser for extracting compositions, scientific units, and related information \cite{mit_table_parser}. However, the regexs used in these works are highly specific and will require significant modifications for different classes of materials.  Despite the availability of MatSci language models, deep neural models have not been explored for IE from materials tables -- the focus of this work.


% Information extraction (IE) is instrumental for knowledge base creation. The transition from rule based IE systems to machine learning IE systems became possible due to availability of large datasets and computational efficiency\cite{chiticariu-etal-2013-rule}. IE from text and tabular data has witnessed tools like WOE\cite{wu-weld-2010-open}, ReVerb\cite{ReVerb2011}, OLLIE\cite{mausam-etal-2012-open}, TaPaS\cite{herzig-etal-2020-tapas}, TaBERT \cite{yin-etal-2020-tabert}, and TabNet\cite{tabnet_Arik_Pfister_2021} to name a few. Specifically, neural models capable of semantically parsing tabular information are jointly pre-trained over natural language queries and structured and semi-structured tables\cite{herzig-etal-2020-tapas, yin-etal-2020-tabert, tabnet_Arik_Pfister_2021, feifei_row_col_interact, pan-etal-2021-cltr}. 
% Information extraction from MS literature is an emerging field because accurately creating, maintaining, and updating material compositions and property databases is a humanly difficult task. Researchers have developed specialised tools for extracting information like extracting inorganic material synthesis routes using word embedding, named entity recognition a\cite{kim_we_ner_cvae, kim_virtual_2017}, and generating database of Curie and Néel temperatures by using a combination of text parsing, table parsing, relation extraction on XMLs and HTMLs of relevant scientific documents\cite{court_auto-generated_2018}, and rule based NER and relation extraction for creating superalloys database\cite{wang_automated_2022}.

% For IE from MS tables, researchers have developed a table extraction tool which takes input of HTML or XML of material science research papers, and uses regex based parser for extracting compositions, scientific units, and related information\cite{mit_table_parser}. This tool was used to extract data related to zeolites\cite{mit_table_parser}, cementitious materials\cite{mit_cement_uvegi}, and aluminum alloys\cite{elsa_aluminium}. ChemDataExtractor is another tool which is capable of extracting complete chemical compositions, but, only from the full information tables present in research papers\cite{chemdataextractor_v1,chemdataextractor_v2}. However, these existing tools are quite specific and can not understand the different structures of MS tables posing special challenges in information extraction as discussed in section 2.1. 

% Recently, researchers have developed materials science language models like MatSciBERT\cite{gupta_matscibert_2022}, MatBERT\cite{matbert_2022}, and BatteryBERT\cite{batterybert_2022}. MatSciBERT\cite{gupta_matscibert_2022} yielded state of the art performance on downstream tasks of abstract classification, named entity recognition, and relation classification, MatBERT\cite{matbert_2022} authors achieved state of the art results on NER tasks, and BatteryBERT\cite{batterybert_2022} was used to enhance battery materials database by LM based question answering downstream task.


==> sections_old_v3/3_dataset_construction.tex <==
% !TEX root = main.tex
\section{Dataset construction}
\label{sec:dataset_construction}
We match a MatSci DB of materials and compositions with tables from published papers, to automatically provide distantly-supervised labels for extraction (hand-annotated for dev \& test sets). This results in 5,883 tables from 2536 publications, of which 2,355 express compositions, with 16,729 materials, and a total of 58,481 (material ID, constituent, composition percentage, unit) tuples.

Now, we create a train set with table-level annotation (NC, SCC, MCC-PI, MCC-CI), row/column-level annotation (ID, composition, constituent, other), and edge level annotation. We also create dev/test sets with these and final tuple-level ground truth. For training set, we first use a commercial DB \cite{interglad} of glass compositions with the respective references. Then, we extract all tables from the 2,536 references in the DB using textmining API. We use table parser \cite{mit_table_parser} for raw XML tables and captions.  We keep 1,880 papers for train set, and rest are split in dev and test (Table \ref{tab:dataset_stats_2}).

The DB does not contain information about the location of a given composition in the paper -- in text, images, graphs, or tables. If present in a table, it can appear in any column or row. Since we do not know the exact location of a composition, we use distantly supervised train set construction \cite{mintz-etal-2009-distant}. First, we simply match the chemical compounds and percentages (or equivalent fractions) mentioned in the DB with the text in a table from the associated paper. If all composition percentages are found and in multiple cells of the table, it is marked as MCC-CI. However, due to several problems (see Section~\ref{sec:problem}), it misses many composition tables. To increase the coverage, we additionally use our rule-based composition parser, but restricted to only those compounds (CPD non-terminal in Figure \ref{fig:comp_parser}) that appear in the DB for this paper. This is important supervision, and leads to a high quality annotation of composition expressions in these papers. If this matching happens: (i) in a cell, the table is deemed as SCC, (ii) on caption/paper text that has a variable (or compound) found in the table, it is marked as MCC-PI. In case of no matching, the table is marked as NC. This automatic annotation is post-processed into row, column and edge labels.

One further challenge is that material IDs mentioned in papers are not provided in the DB. So, we manually annotate material IDs for all the identified composition tables in the training set. This leads to a train set of 11,207 materials with 38,799 tuples from 4,408 tables. Since train set is distantly supervised and can have noise, a MatSci expert manually annotated the dev and test tables with row/column/edge labels, units, tuples, compositions, and table type, resulting in over 2,500 materials and over 9,500 tuples per set. Further statistics are discussed in ~\ref{app:dataset-details}.


==> sections_old_v3/4_model.tex <==
% !TEX root = main.tex
\section{\sys\ architecture} 
\label{sec:model}
To address automated extraction of material compositions from tables, we present an ML formulation of the problem.  Formally, given a table $T$, its caption, and the complete text of publication in which $T$ occurs, we aim to extract compositions expressed in $T$, in the form $\{(id, c_k^{id}, p_k^{id}, u_k^{id} )\}_{k=1}^{K^{id}}$. Here, $id$ represents the material ID, as defined in the paper. Material IDs are defined by MatSci researchers to succinctly refer to that composition in text and other tables. $c_k^{id}$ is a constituent element or compound present in the material, $K^{id}$ is the total number of constituents in the material, $p_k^{id} > 0$ denotes the percentage contribution of $c_k^{id}$ in its composition, and $u_k^{id}$ is the unit of $p_k^{id}$ (either mole\% or weight\%). For instance, the desired output tuples corresponding to ID A1 from Figure \ref{fig:three comp_tables}a are (A1, MoO$_3$, 5, mol\%), (A1, Fe$_2$O$_3$, 38, mol\%), (A1, P$_2$O$_5$, 57, mol\%).

% \begin{wrapfigure}{l}{0.55\textwidth}
%     \vspace{-3ex}
%     \centering
%     \includegraphics[width=0.55\textwidth, height=4cm]{flowchart.png}
%     \caption{The design of \sys}
%     \label{fig:comp_table_cls}
%     \vspace{-1ex}
% \end{wrapfigure}
\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.45\textwidth, height=3cm]{flowchart.png}
    \caption{The design of \sys}
    \label{fig:comp_table_cls}
    \vspace{-1ex}
\end{figure}

Figure \ref{fig:comp_table_cls} illustrates the basic pipeline for extraction in \sys. We find that the simplest task is to identify whether the table $T$ is an SCC table, owing to a distinctive presence of multiple numbers, and compounds in single cells. \sys{} first runs a GNN-based SCC predictor, which classifies $T$ as an SCC table or not. For SCC table, it uses a standalone rule-based composition parser. For the other category, \sys{} runs a second GNN (GNN$_2$), and labels rows and columns of $T$ as compositions, material IDs, constituents, and others. If no constituents or composition predictions are found, then $T$ is deemed to be a non-composition (NC) table. Else, it is an MCC table, for which \sys{} predicts whether it has all information in $T$ or some information is missing (partial-information predictor). If it is complete information table, then GNN$_2$'s predictions are post-processed into compositions. If not, the caption and text of paper are also processed, along with GNN$_2$'s predictions leading to final composition extraction. We note that our system ignores statistically infrequent corner cases, such as single-cell partial information tables -- we discuss this further in our error analysis. We now describe each of these components, one by one.

%We propose to classify all MS Tables as shown in Figure \ref{fig:comp_table_cls}. At the first level, we classify tables as Single-cell composition tables and Multi-cell composition tables \& Non-composition tables. Both, Single-cell and Multi-cell composition tables are further classified as to whether complete information is present inside tables to extract compositions, or only partial compositions reside inside tables. We also depict an example of each type of table in Figure \ref{fig:comp_table_cls}. Single-cell partial information tables occur very rarely in our dataset, hence we do not consider this class in the remaining paper.
\subsection{GNNs for table processing}
\label{sec:gnn}
At the core of \sys\ are two GNNs that learn representations for each cell, row, column and the whole table. Let table $T$ has $R$ rows, $C$ columns, and text at $(i,j)^{th}$ cell be $t_{ij}$, where $1\leq i\leq R$, and $1\leq j\leq C$. We construct a directed graph 
$G_T = (V_T, E_T)$, where $V_T$ has a node for each cell $(i,j)$, one additional node for each row and column, denoted by $(i,0)$ and $(0,j)$, respectively, and one node for the whole table represented by $(0,0)$. There are bidirectional edges between two nodes of the same row or column. All cell nodes have directed edges to the table node and also their corresponding row and column nodes. 
%We initialize the embeddings $\overrightarrow{x_{ij}}$ for each node $(i,j)$ as follows. 
The table, row and column embeddings are randomly-initialized with a common vector, which gets trained during learning. A node $(i,j)$'s embedding $\overrightarrow{x_{ij}}$ is initialized by running a language model $LM$ over $t_{ij}$.

As constructed, $G_T$ is permutation-invariant, i.e., if we permute rows or columns, we get the same graph and embeddings. However, initial rows/columns can be semantically different, since they often represent headings for the subsequent list. For instance, material IDs are generally mentioned in first one or two rows/columns of the table. So, we additionally define \emph{index embeddings} $\overrightarrow{p_{i}}$ to represent a row/column numbered $i$. We use the same index embeddings for rows and columns so that our model stays transpose-invariant. We also observe that while first few indices are different, the semantics is generally uniform for indices higher than 3. %\textcolor{red}{This is because, after the headers (or material IDs) in the first two rows/columns, the following indices have either different constituents or compositions (for example, rows 4-5 in Figure \ref{fig:three comp_tables}b and \ref{fig:three comp_tables}c)}. 
Accordingly, to allow \sys\ to handle large tables, we simply use $\overrightarrow{p_{i}}=\overrightarrow{p_{3}}~ \forall i > 3$. 
Finally, any manually-defined features added to each node are embedded as $\overrightarrow{f}$ and concatenated to the cell embeddings. Combining all ideas, a cell embedding is initialized as: 
\vspace{-1ex}
%\begin{equation}
\[
\overrightarrow{x_{ij}} =  \overrightarrow{f_{ij}} \;||\; \left( LM_{CLS}(\langle CLS ~ t_{ij} ~ SEP \rangle) \!+\! \overrightarrow{p_{i}} \!+\! \overrightarrow{p_{j}} \right) \] 
%\[(1\leq i \leq R, 1 \leq j \leq C). \]
%\end{equation}
Here, $1\leq i \leq R, 1 \leq j \leq C$. $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token after running a $LM$ over the sentence inside $\langle\rangle$. Message passing is run on the graph $G_T$ using a GNN, which computes a learned feature vector $\overrightarrow{h}$ for every node: \[\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN\left(\{\overrightarrow{x_{ij}}\}_{i,j=(0,0)}^{(R,C)}\right).\]

\subsection{Single-cell composition tables}
\label{sec:single_cell_table}
In its pipeline, \sys\ first classifies whether $T$ is an SCC table. 
For that, it runs a GNN (named GNN$_1$) on $T$ with two manually defined features (see below). 
It then implements a Multi-layer Perceptron MLP$_1$ over the table-level feature vector $\overrightarrow{h_{00}}$  to make the prediction. Additionally, GNN$_1$ also feeds row and column vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$ through another MLP (MLP$_2$) to predict whether they contain material IDs  or not. If $T$ is predicted as an SCC table, then one with the highest MLP$_2$ probability is deemed as material ID row/column (provided probability > $\alpha$, where $\alpha$ is a hyper-parameter tuned on dev set), and its contents are extracted as potential material IDs. If all row and column probabilities are less than $\alpha$, then table is predicted to not have Material IDs, as in Figure \ref{fig:three comp_tables}c.

% \begin{wrapfigure}{r}{0.46\textwidth}
%   \vspace{-2ex}
%     \centering
% \FramedBox{3cm}{6.2cm}
% {CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
% PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
% ~\\
% CST$_1$ = NUM? W CPD\\
% CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
% CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
% CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
% }
% \caption{Regexes in composition parser}
%     \label{fig:comp_parser}
%     \vspace{-2ex}
% \end{wrapfigure}
% \begin{figure}[hbt]
%     \centering
% \FramedBox{2.5cm}{5.3cm}
% {\small{CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
% PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
% ~\\
% CST$_1$ = NUM? W CPD\\
% CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
% CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
% CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
% }}
% \caption{Regexes in composition parser}
%     \label{fig:comp_parser}
%     \vspace{-2ex}
% \end{figure}

\textbf{Rule-based composition parser: }
For an SCC table, \sys\ must parse the full \emph{composition expression} written in a single cell in the row/column corresponding to each Material ID.  
\begin{wrapfigure}{l}{0.3\textwidth}
    \vspace{-0.1in}
    % \centering
    % \includegraphics[width=0.25\textwidth]{confusion_matrix.png}
    % %\vspace{-1ex}
    % \caption{Confusion matrix for all table types}
    % \label{fig:confusion}
    % \vspace{-0.2in}
    \centering
    \FramedBox{2.5cm}{5.3cm}
    {\small{CMP = PAT$_1$ | PAT$_2$ | PAT$_3$\\
    PAT$_i$ = START CST$_i$ (SEP CST$_i$)$^+$ END \\
    ~\\
    CST$_1$ = NUM? W CPD\\
    CST$_t$ = CST$_1$ (SEP CST$_1$)$^*$ \\
    CST$_2$ = (CST$_t$ | OB CST$_t$ CB) W NUM  \\
    CST$_3$ = NUM W (CST$_t$ | OB CST$_t$ CB)
    }}
    \caption{Regexes in parser}
        \label{fig:comp_parser}
        \vspace{-2ex}
\end{wrapfigure}
Such compositions are close to regular languages and can be parsed via regular expressions. Figure \ref{fig:comp_parser} shows the regular expression (simplified, for understandability) implemented in \sys. Here CMP denotes the matched composition, PATs are three main patterns for it, CSTs are sub-patterns, CPD is a compound, NUM is a number, OB and CB are, respectively, open and closed parentheses (or square brackets). W is zero or more whitespace characters, and SEP contains explicit separators like `-' or `+'. START and END are indicators to separate a regular expression from rest of the text.

%Single-cell composition tables or others (Multi-cell and Non-composition tables). Then, we use Regular Expressions to extract compositions (set of tuples) from the predicted Single-cell composition tables.

% \subsubsection{RegEx baseline model}
% \label{sub_sec:regex}
% First, we use create a simple Regular Expression based model (RegEx) to identify Single-cell composition tables. We notice that single cell compositions are written in a form that can be matched and parsed using regular expressions (REs). We write different REs for compositions having elements and compounds. This is because in general coefficients succeed compounds and precede elements. After error analysis, we added some more types of RE which can parse compositions involving multiplication of coefficients like $(Ge_{0.25}Ga_{0.10}S_{0.65})_{0.9}-Br_{0.1}$ and $(50-x)Bi_2O_3 * (50-x)B_2O_3 * 2x(AgI-AgBr)$. In total, we write six different types of REs. These REs also handle the case when percentage contribution of compounds is an arithmetic expression having multiplication and division operators. The compounds may be separated by various special characters like $*, -, :, +$ or space or may not be separated. We also created a list of common elements and compounds which are required by the REs in order to parse compositions. RegEx Model predicts a table to be Single-cell composition table if any of the table cell matches with any of the six REs.


%\subsubsection{Classifying Single-cell composition tables vs Others}
%\label{sec:gat_single_cell_table}

%We use a Graph Neural Networks ($GNN$) to predict whether a table is Single-cell composition table or not. We represent table as a graph, where each table cell is a graph node. Formally, let $T$ be the table, $R$ and $C$ be the number of rows and columns in $T$. We represent the table graph by $G_T = (V_T, E_T)$. Here, $V_T = \{(i, j) \; | \; 0 \leq i \leq R, 0 \leq j \leq C\}$ is the set of all nodes/vertices in $G_T$. Note that these also include row nodes of the form $(i, 0)$, column nodes of the form $(0, j)$, and table node $(0, 0)$. We include the row and column nodes to identify the row or column containing material IDs and table node to perform classification at the table level. 
%We connect two table cells by an edge if they share same row or same column. All the table cells also have edges directed to the table node and their corresponding row and column nodes. Hence the set of edges is
%\[ E_T = \{((i_1, j_1), (i_2, j_2)) \; | \; i_1 = i_2 \;or\; j_1 = j_2, \; 1 \leq i_1, i_2 \leq R, 1 \leq j_1, j_2 \leq C\} \; \cup \; \]
%\[ \{((i, j), (i, 0)) \; | \; 1 \leq i \leq R, 0 \leq j \leq C\} \; \cup \; \{((i, j), (0, j)) \; | \; 0 \leq i \leq R, 1 \leq j \leq C\} \; \cup \; \]
%\[ \{((i, j), (0, 0)) \; | \; 1 \leq i \leq R, 1 \leq j \leq C\} \]

%Let $t_{ij}$ and $\overrightarrow{x_{ij}}$ be the text and initial node features for table cell $(i, j)$ respectively. Using a pre-trained Language Model ($LM$) as the text encoder, we get
%\[ \overrightarrow{x_{ij}} = LM_{CLS}(CLS \;||\; t_{ij} \;||\; SEP) \; \forall \; 1 \leq i \leq R, 1 \leq j \leq C\]
%where $||$ is the concat operation and $LM_{CLS}$ gives the contextual embedding of the $CLS$ token, which is representative of $t_{ij}$. Embeddings of row nodes, column nodes and table node are initialized with a random vector, which gets learned during training.
%It can be observed from the examples of composition tables presented till now that generally material IDs occur in the initial part of table. To make the model aware of this, we augment our model with row/column index embeddings.
%\[ \overrightarrow{z_{ij}} = \overrightarrow{x_{ij}} + \overrightarrow{p_{i}} + \overrightarrow{p_{j}} \]
%Here, $\overrightarrow{p_{i}}$ is randomly initialized embedding for row $i$ and similarly $\overrightarrow{p_{j}}$ is the embedding for column $j$ having the same size as that of $\overrightarrow{x_{ij}}'s$. We use the same index embeddings for row and column so that our model stays transpose-invariant. To handle the large tables and because of relatively small size of our dataset, we take $\overrightarrow{p_{3}} = \overrightarrow{p_{i}}$ for all $i > 3$.
%Then, $\{\overrightarrow{h_{ij}}\}_{i,j=(0,0)}^{(R,C)} = GNN(\{\overrightarrow{z_{ij}}\}_{i,j=(0,0)}^{(R,C)})$ are the output node features in the context of complete table.
%We then feed row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$, to a Multi-layer Perceptron $MLP_1$ to predict whether each row and column contains material IDs or not. If more than one row/column are predicted to have material IDs, then we select the one with highest probability. Finally, we pass $\overrightarrow{h_{00}}$ through another Multi-layer Perceptron $MLP_2$ for Single-cell composition table classification. Final loss is the weighted sum of binary cross entropy loss for single-cell table classification and row/column classification for material IDs. Weights are hyper-parameters.

%\subsubsection{Extracting Single-cell compositions}
%\label{sec:regex_extraction}



The first pattern parses simple number-compound expressions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$. Here each of the two constituents will match with CST$_1$. The other two patterns handle \emph{nested} compositions, where simple expressions are mixed in a given ratio. The main difference between second and third pattern is in the placement of outer ratios -- after or before the simple composition, respectively. Example match for PAT$_2$ is (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and for PAT$_3$ is 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). 

To materialize these rules, \sys\ pre-labels compounds. For our dataset, we use a list-based extractor, though other chemical data extractors \cite{chemdataextractor_v1} may also be used.  After parsing, \sys\ normalizes all coefficients so that they sum to hundred. For nested expressions, the outer ratio and the inner ones are normalized separately and then multiplied.
For units, \sys\ searches for common unit keywords such as mol, mass, weight, and their abbreviations like wt.\%, and at.\%. The search is done iteratively with increasing distance from cell containing the composition. If not found in the table, then the caption is searched. If still not found, mole\% is used as default.

\textbf{Manual Features:} GNN$_1$ uses two hand-coded features. The first feature is set to true if that cell contains a composition that matches our rule-based composition parser. Each value, true or false, is embedded as $\overrightarrow{o}$.
The second feature named \emph{max frequency feature} adds the bias that material IDs are generally unique in a table. We compute $q_{i}^{r}$ and $q_{j}^{c}$, which denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$, respectively. If these numbers are on the lower side, then that row/column has more unique strings, which should increase the probability that it contains material IDs. The computed $q$ values are embedded in a vector as $\overrightarrow{q}$. The embedded feature $\overrightarrow{f_{ij}}$ for cell $(i,j)$ is initialized as $\overrightarrow{o_{ij}} \;||\;  (\overrightarrow{q_{ij}^r}+\overrightarrow{q_{ij}^c})$.


%We notice that single cell compositions are written in a form that can be matched and parsed using Regular Expressions (REs). We write different REs for compositions having elements and compounds. Below, we describe three REs for compounds: $pat1, pat2, $ and $pat3$. Similar REs can be written for elements, difference being that coefficients precede elements, whereas they succeed compounds. We first create a list of common elements and compounds ($comps$) which are required by the REs to parse compositions. $pat1$ matches compositions like 40Bi$_2$O$_3$ * 60B$_2$O$_3$, $pat_2$ matches compositions like (40Bi$_2$O$_3$+60B$_2$O$_3$)30 - (AgI+AgCl)70, and $pat3$ matches compositions like 40Bi$_2$O$_3$,40B$_2$O$_3$,20(AgI:2AgCl). During parsing, we normalize the coefficients so that they sum to one.

%\[ comps = (Al\backslash(OH\backslash)3 | PbO2 | PbO | \dots) \]
%\[ num = (\backslash d*\backslash.\backslash d+| 0 | [1-9]\backslash d*) \]
%\[ var = (x | y | z | X) \]
%\[ enum = ((num \; var) | num | var) \]
%\[ exp = enum (\backslash s*[+\backslash-/]\backslash s*enum)* \]
%\[ expr = ((num\backslash s*\%)|exp|(\backslash(exp \backslash))) \]
%\[ sep = \backslash s*[-*:+,]?\backslash s* \]
%\[ start = (\string^|[\string^\backslash w-]) \]
%\[ end = ([\string^\backslash w-]|\$) \]

%\begin{enumerate}
%    \item $subpat1 = expr? \backslash s*comps$ \\
%    $pat1 = start(subpat1(sep \; subpat1)+)end$
    
%    \item $subpat2 = (subpat1(sep \; subpat1)*)$ \\
%    $subpat3 = ((subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash])\backslash s*expr)$ \\
%    $pat2 = start(subpat3(sep\; subpat3)+)end$
    
%    \item $subpat4 = (expr\backslash s*(subpat2|\backslash(\backslash s*subpat2\backslash s*\backslash)|\backslash[\backslash s*subpat2\backslash s*\backslash]))$ \\
%    $pat3 = start(subpat4(sep\; subpat4)+)end$
    
%\end{enumerate}

%We then use these six REs along with predicted row or column index containing material IDs to extract composition tuples from the predicted Single-cell composition tables. For units (mol or weight), we search keywords like mol, mass percent, weight percent, at.\%, wt.\% . We first search for units in table in increasing L1 distance from cell containing composition, and then look for these keywords in the table caption if not found in table.

\subsection{Multi-cell composition tables}
\label{sec:multi-cell}

If $T$ is predicted to not be an SCC table, \sys\ runs it through another GNN (GNN$_2$). The graph structure is very similar to $G_T$ from Section \ref{sec:gnn}, but with two major changes. 
%geared towards incorporating the caption information at prediction time.
First, a new \emph{caption node} is created with initial embedding as given by $LM$ processing the caption text.  
%\textcolor{red}{For this, the table node is replaced by a new \emph{caption node, }}
Edges are added from caption node to all row and column nodes. To propagate the information further to cells, edges are added from row/column nodes to corresponding cell nodes. The caption node especially helps in identifying non-composition (NC) tables. Second,
the max frequency feature from Section \ref{sec:single_cell_table} is also included in this GNN. 

We use tables in Figure \ref{fig:two_comp_tables_2} as our running examples. While Figure \ref{fig:two_comp_tables_2}a is a complete-information table, Figure \ref{fig:two_comp_tables_2}b is not, and can only be understood in the context of its caption, which describes the composition as  $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$. Here x, y are variables, which also need to be extracted and matched with the caption. \sys\ first decodes the row and column feature vectors $\overrightarrow{h_{i0}}$ and $\overrightarrow{h_{0j}}$, as computed by GNN$_2$, via an MLP$_3$ into four classes: composition, constituent, ID, and other (label IDs 1, 2, 3, 0, respectively). The figures illustrate this labeling for our running example. The cell at the intersection of composition row/column and constituent column/row represents the percentage contribution of that constituent in that composition. 
%Having identified the Single-cell composition tables and extracting compositions from them, we now model the Multi-cell composition tables. We identified two prominent classes, all-info tables and partial-info tables, as shown in Figure \ref{fig:two_comp_tables_2}. In the text corresponding to table shown in Figure \ref{fig:partial_info_table_2}, we find $[(Na_2O)_x(Rb_2O)_{1-x}]_y(B_2O_3)_{1-y}$ which helps to decode the table.

\begin{figure}[t]
\begin{center}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/multi_cell_table_1_S0022309314000660.png}
        % \label{fig:multi_cell_comp_table_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=2.8cm]{figures/partial_info_table_2_S0022309305006903.png}
        % \label{fig:partial_info_table_2}
    \end{subfigure}
    % \vspace{-1ex}
    \caption{Multi-cell composition tables (a) Complete information \cite{fig_5a} (b) Partial information \cite{fig_5b}}
    \label{fig:two_comp_tables_2}
\end{center}
    \vspace{-4ex}
\end{figure}
%For Multi-cell composition tables, we classify rows and columns of input table among four classes: \textbf{1 for Composition}, \textbf{2 for Constituent}, \textbf{3 for Material IDs} and \textbf{0 for Others}.
%Label 1 means that row/column specifies a composition. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, all except first two rows and all except first row are composition rows respectively. In Figure \ref{fig:nom_exp_table}, all columns except first are composition columns. Similarly, label 2 implies that row/column contains the percentage contribution of some constituent(s) for every composition column/row. For example, in Figure \ref{fig:multi_cell_comp_table_2} and \ref{fig:partial_info_table_2}, first three columns and first two columns are constituent columns respectively. In Figure \ref{fig:nom_exp_table}, last seven rows except the middle one are constituent rows and second row has label 3 as it contains the Material IDs. All other rows and columns have label 0. Note that the cell at the intersection of composition row and constituent column or composition column and constituent row contains the percentage contribution of that constituent in that composition.

Further, to associate the identified percentage contribution with the corresponding constituent (like P$_2$O$_5$ in Figure \ref{fig:two_comp_tables_2}a) or variables x, y in Figure \ref{fig:two_comp_tables_2}b), we perform classification at the edge level. For ease of exposition, we describe our method in this Section \ref{sec:multi-cell} for the setting that the table has been predicted by GNN$_2$ to have row-wise orientation, i.e., rows are compositions and columns are constituents. A transposed computation is done in the reverse case. Since the constituent/variable will likely occur in the same column or row as the cell containing percentage contribution, our method computes an edge feature vector: for edge $e=(i,j)\rightarrow(i',j')$, s.t. $i=i' \vee j=j' $, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{i'j'}}$.
%\textcolor{red}{and for edge $e=(i,j)\rightarrow(i',j')$, the feature vector $\overrightarrow{h_e}= \overrightarrow{h_{ij}} \;||\; \overrightarrow{h_{ij'}}$}. 
It then takes all such edges $e$ from cell $(i,j)$, if row $i$ is labeled composition and column $j$ is labeled constituent. Each edge $e$ is classified through an MLP$_4$, and the edge with maximum logit value is picked to identify constituent/variable. This helps connect 36 to P$_2$O$_5$ and 0.8 to x in our running examples. %A transposed computation is done if rows are constituents and columns are compositions.
GNN$_2$ also helps in predicting NC tables. In case none of the rows/columns are predicted as 1 or 2, then the table is deemed as NC and discarded.

%we construct an edge from every table cell to all cells with the same row/column including itself. We then select the edge with maximum logit and use a simple RE to get the constituent/variable from the cell at the other end of selected edge. Some examples of valid edges in above figures are the ones which connect 90 to Sb$_2$O$_3$, 30 to PbCl$_2$, 0.3 to y, 0.8 to x, etc.

% \subsubsection{LM-Lin-Table baseline}
% \label{sec:lm_lin_table}
% Figure \ref{fig:lm_lin_table_baseline} depicts our LM-Lin-Table baseline model. Here, LM is a pre-trained Language Model. Here, we flatten the input table row-wise after replacing the empty table cells with special [EMPTY] token. Then, we tokenize this linear table using the LM tokenizer. It's possible to obtain more than one wordpiece for some table cells. Since, the length of tokenized linear table can be greater than 512, we truncate minimum possible rows from the end so that input length to LM becomes less than or equal to 512. Let the tokenized linear table be denoted by $[t_0, t_1, \dots, t_n]$, where $t_0 = [CLS]$, $t_n = [SEP]$, $n < 512$ and the number of rows after truncation be $R'$. We then pass $[t_0, t_1, \dots, t_n]$ through the LM to obtain contextual embeddings of every wordpiece $[\overrightarrow{z_0}, \dots, \overrightarrow{z_n}]$.

% \begin{figure}[!htb]
% \begin{center}
%     \centering
%     \includegraphics[scale=0.3]{multi_cell_baseline.png}
%     \caption{Schematic of the LM-Lin-Table baseline model}
%     \label{fig:lm_lin_table_baseline}
% \end{center}
% \end{figure}

% We take the contextual embedding of first word-piece of every table cell to be representative of it. Let $0 < k_{1,1} < k_{1,2} < \dots < k_{R',C} < n$ be the indices such that $k_{i,j}$ is the index of first wordpiece of cell $(i, j)$.
% To make the baseline model aware of different row and column indexes, we add randomly initialized row and column index embeddings, so that final cell embeddings become $[\overrightarrow{h_{k_{1,1}}}, \dots, \overrightarrow{h_{k_{R',C}}}]$, where $\overrightarrow{h_{k_{i,j}}} = \overrightarrow{z_{k_{i,j}}} + \overrightarrow{rid_{i}} + \overrightarrow{cid_{j}}$, $\overrightarrow{rid_{i}}$ and $\overrightarrow{cid_{j}}$ are the $i^{th}$ row and $j^{th}$ column index embeddings respectively. For brevity, we now denote $\overrightarrow{h_{k_{i,j}}}$ by $\overrightarrow{h_{i,j}}$.
% Row and column embeddings are computed by taking average of final cell embeddings of cells occurring in that row/column i.e. $\overrightarrow{r_i} = Mean(\overrightarrow{h_{i,1}}, \dots, \overrightarrow{h_{i,C}})$ and $\overrightarrow{c_j} = Mean(\overrightarrow{h_{1,j}}, \dots, \overrightarrow{h_{R',j}})$.
% Edge embeddings are computed by concatenating the final cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. Finally, all row and column embeddings are fed to a MLP to get probabilities of every row and column belonging to 4 classes as described earlier and edge embeddings are passed through another MLP to obtain logit score for every table edge. Loss function consists of row/column cross-entropy loss and edge binary cross-entropy loss.

%\subsubsection{GAT-Multi-cell-table}

%This model is mostly similar to the model as discussed in section \ref{sec:gat_single_cell_table}. Since, we do not need to do table-level classification in this case, we remove the $(0, 0)$ table node and its edges from the graph. Here too, the contextual row embeddings $\overrightarrow{h_{i0}}$ and column embeddings $\overrightarrow{h_{0j}}$, where $1 \leq i \leq R$ and $1 \leq j \leq C$ are obtained with the help of $LM$ and $GNN$. Then, we feed them through a MLP with softmax activation at the end to get probabilities of every row and column belonging to four classes (composition, constituent, material ID and others). Edge embeddings are computed by concatenating the contextual cell embeddings of source and destination cells i.e. $\overrightarrow{e_{uv}} = \overrightarrow{h_u} \;||\; \overrightarrow{h_v}$, where $u$ and $v$ are two table cells having same row/column. These edge embeddings are then passed through another MLP to obtain logit score for every table edge. Training loss consists of weighted row/column cross-entropy loss and edge binary cross-entropy loss.



\textbf{Partial information table predictor:}
%Till now, we have predicted the row \&column labels and also linked the extracted percentage contributions with the corresponding constituent/variable. If all row and column labels are predicted to be 0, then we classify that table as a non-composition table.
Next, \sys\ distinguishes between complete-information (CI) and partial-information (PI) MCC tables. It uses a logistic regression model with custom input features for this prediction task. 
%We describe this assuming the table orientation is predicted to be row-oriented by GNN$_2$ (i.e., rows are compositions, columns are constituents); analogous transposed computation will be done for the reverse case. 
Let $P$ and $Q$ be the sets of all row indices with label 1 (composition) and column indices with label 2 (constituent), respectively. Also, assume $n_{ij}$ is the number present in table cell $(i, j)$ or $0$ if no number is present.  To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely an MCC-PI, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is MCC-CI. Features F4 (and F5) computes the maximum (average) of the sum of all extracted compositions. The intuition of F4 and F5 is that the higher these feature values, higher the chance of the table being an MCC-CI. Formally, 

\[
\mathrm{F4}=(\max_{i \in P} \sum_{j \in Q}n_{ij}) ~~~~~~~~~~~~~
\mathrm{F5}=(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij}).
\]

%to extract the composition tuples as described in section \ref{sec:proposed_cls_tables}. For this, we build a Logistic Regression model with custom input features.
%Assume the table to be a row-oriented table as inferred from predicted row and column labels. Let $P$ and $Q$ be the sets of all row indexes with label 1 and column indexes with label 2 respectively. Also, assume $n_{ij}$ is the first number present in table cell $(i, j)$ or $0$ if no number is there. To create the features, we first extract all the constituents (compounds) and variables predicted by MLP$_4$. We now construct five table-level features (F1-F5). F1 and F2 count the number of unique variables and chemical compounds extracted by MLP$_4$. The intuition is that F1 is high, then it is more likely a partial-information table, and vice-versa if F2 is high. F3 computes the number of rows and columns labeled as 2 (constituent) by MLP$_3$. The more the value of F3, the more likely it is that the table is complete information. Features F4 (and F5) computes the maximum (average) of the sum of 

%\begin{enumerate}
%    \item \textit{Number of unique variables}: If we have some variables, then it is more likely for the table to belong to partial information table class.

%    \item \textit{Number of unique constituents}: If there are many constituents, then table is more likely to be an all information table.

%    \item \textit{Maximum sum among all extracted compositions} $(\max_{i \in P} \sum_{j \in Q}n_{ij})$: Greater this quantity, greater the chances of being in all-information table class.
    
%    \item \textit{Average sum across all extracted compositions} $(\frac{1}{|P|} \sum_{i \in P} \sum_{j \in Q}n_{ij})$: Explanation similar to above feature.

%    \item \textit{Number of rows/columns with label 2}: If there are lesser number of rows/columns with label 2, then table is probably a partial information table.

%\end{enumerate}

\textbf{MCC table extractor:} For MCC-CI, MLP$_3$ and MLP$_4$ outputs are post-processed, and units are added (similar to SCC tables), to construct final extracted tuples. For MCC-PI, on the other hand, information in text needs to be combined with the MLP outputs for final extraction. The first step here is to search for the composition expression, which may be present in table caption, table footer, and if not there, in somewhere in the rest of the research paper. Here, \sys\ resorts to using our rule-based composition parser from Figure \ref{fig:comp_parser}, but with one key difference. Now, the composition may contain variables ($x$, $y$) and even mathematical expressions like $100-x$. So the regular grammar is enhanced to replace the non-terminal NUM with a non-terminal EXPR, which represents, numbers, variables, and simple mathematical expressions over them. An added constraint is that if there are variables in set $Q$, then those variables must be present in the matched composition expression. \sys\ completes the composition by substituting the variable values from every composition row into the matched composition. There may be other types of MCC-PI tables where only compounds are identified in tables, such as Figure \ref{fig:three comp_tables}b. For these, \sys\ first computes the constituent contributions in terms of variables from composition expression, and then equates it with the numbers present in rows/columns labeled 1 (composition). In our example, \sys\ matches x with the numbers 10, 20, 30, and 40, and the rest of the composition is extracted by processing the composition expression in the caption with these values of x. Units and material IDs are added to the tuples, similar to other tables.


%After identifying the partial information Multi-cell composition tables, we try to complete the composition by searching for REs in the table caption, table footer, and then sequentially in research paper text from top to bottom. In case of variables as in Figure \ref{fig:partial_info_table_2}, we search for REs containing precisely those variables and complete the composition by substituting the variable values from every composition row. If case of constituents as in Figure \ref{fig:partial_info_table_1}, we first compute the constituent contributions in terms of variables and then equate it with the numbers present in rows/columns having label 1. For example, in terms of variables, contribution of $CsCl$ is $x/100$ for table shown in Figure \ref{fig:partial_info_table_1}. Since $0 \leq x/100 \leq 1$, we divide the numbers in table by 100. And then solve for x by equating $x/100 = 40/100$ for last row, giving $x = 40$, which completes the composition as $\{(La_2S_3, 0.2), (Ga_2S_3, 0.4), (CsCl, 0.4)\}$. Then we prepend material IDs and append units to the tuples to complete the extraction.


\subsection{Constraint-aware loss functions}
\label{sec:constraints}

\sys\ needs to train the two GNNs and the PI table predictor. Our data construction provides gold labels for each prediction task (discussed in next section), so we train these component-wise. The PI table predictor is trained on standard logistic regression loss. GNN$_1$ is trained on a weighted sum of binary cross entropy loss for SCC table classification and row/column classification for material IDs --  weight is a hyper-parameter. Similarly, GNN$_2$ loss function consists of sum of row/column cross-entropy and edge binary cross-entropy losses. 

GNN$_2$ has the more complex prediction problem, since it has to perform four-way labeling for each row and column. In initial experiments, we find that the model sometimes makes structural errors like labeling one row as constituent and another row as composition in the same table -- highly unlikely as per the semantics of composition tables. To encourage GNN$_2$ to make structurally consistent predictions, we express a set of constraints on the complete labelings, as follows. (1) A row and a column cannot both have compositions or constituents.  %(2) Compositions and constituents should be orthogonally predicted  
(2) Composition and material ID must be orthogonally predicted (i.e, if a row has a composition then ID must be predicted in some column, and vice versa). (3) Constituents and material IDs must never be orthogonally predicted (if rows have constituents then another row must have the ID). And, (4) material ID must occur at most once for the entire table. 
%Limitation of space precludes complete mathematical exposition of all constraints (see App. ~\ref{app:constraint} for details). 
As an example, constraint (1) can be expressed as a hard constraint as:
\begin{center}
\(
r_i = l \Rightarrow c_j \neq l ~~~~\forall i\in\{1,\ldots, R\}, j\in \{1,\ldots,C\}, l\in\{1,2\}. 
\)
\end{center}
Here, $r_i$ and $c_j$ are predicted labels of row $i$ and column $j$. We wish to impose these structural constraints at training time, so that the model is trained to honor them. We follow prior work by Nandwani et al. \cite{yatin}, to first convert these hard constraints into a probabilistic statement. For example, constraint (1) gets expressed as:
\begin{center}
\(
P(r_i = l; \theta) + P(c_j = l; \theta) - 1 \leq 0\) \( \forall i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}.
\)
\end{center}
$\theta$ represents GNN$_2$'s parameters. Following same work, each such constraint gets converted to an auxiliary penalty term, which gets added in the loss function for constraint-aware training. The first constraint gets converted to:
\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l; \theta) + P(c_j = l; \theta) - 1) \]
This and similar auxiliary losses for other constraints (App.~\ref{app:constraint}) get added to the GNN$_2$'s loss function for better training. $\lambda$ is a hyper-parameter. We also use constraint (4) for GNN$_1$ training.

%We augmented our GAT based models with some features/constraints to improve the performance. These bells and whistles have been discussed in the following sub-sections.

%\subsubsection{Constraints}
%\label{sec:constraints}
%In the approach presented till now, it is possible for the model to predict some row as composition row and some column as composition column and similar is the case for constituents. But practically, this does not make sense. We formulate these constraints mathematically and modify our training procedure by adding a suitable term to the loss function.

%Let $r_i$ be the label assigned by the model to row $i$ and $c_j$ be the label assigned to column $j$. We can write the hard version of these constraints as $r_i = 1 \Rightarrow c_j \neq 1$ and $r_i = 2 \Rightarrow c_j \neq 2$, where $i \in \{1, \dots, R\}$ and $j \in \{1, \dots, C\}$. We rewrite these as
%$r_i \neq l \lor c_j \neq l$ for $l \in \{1, 2\}$. In a similar fashion, labels 1 \& 3 can't occur simultaneously in rows or columns, labels 2 and 3 can't occur orthogonal to each other, and label 3 can occur at most once for the entire table.
%We convert all these hard constraints to soft constraints as done by Yatin et al. \cite{yatin} to obtain:

%\begin{enumerate}
%    \item $P(r_i = l) + P(c_j = l) - 1 \leq 0\;$ for $i \in \{1, \dots, R\}, \; j \in \{1, \dots, C\}, \; l \in \{1, 2\}$
    
%    \item $P(r_{i_1} = 1) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $i_1, i_2 \in \{1, \dots R\}, \; i_1 \neq i_2$
    
%    \item $P(c_{j_1} = 1) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $j_1, j_2 \in \{1, \dots C\}, \; j_1 \neq j_2$
    
%    \item $P(r_i = l) + P(c_j = 5-l) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}, \; l \in \{2, 3\}$
    
%    \item $P(r_{i_1} = 3) + P(r_{i_2} = 3) - 1 \leq 0\;$ for $1 \leq i_1 < i_2 \leq R$
    
%    \item $P(c_{j_1} = 3) + P(c_{j_2} = 3) - 1 \leq 0\;$ for $1 \leq j_1 < j_2 \leq C$
    
%    \item $P(r_i = 3) + P(c_j = 3) - 1 \leq 0\;$ for $i \in \{1, \dots R\}, \; j \in \{1, \dots C\}$

%\end{enumerate}

%We now convert these soft constraints to penalty terms and add them to the loss function. For the first soft constraint, we add
%\[ \lambda \sum_{i=1}^R \sum_{j=1}^C \sum_{l=1}^2 max(0, P(r_i = l) + P(c_j = l) - 1) \]
%to the loss function for all tables $T$ in the training dataset. Here, $\lambda$ is a hyper-parameter which controls the magnitude of penalty relative to the original training loss. We add similar penalty terms for other soft constraints.

%\subsubsection{Manual features}

%Here, we introduce some task-specific features which can potentially boost the performance.

%\begin{enumerate}
%    \item \textit{Max-frequency Feature}: This feature helps to incorporate the bias that material IDs are unique. Let $f_{i}^{(r)}$ and $f_{j}^{(c)}$ denote the maximum frequency of any non-empty string occurring in the cells of row $i$ and column $j$ respectively. If these numbers are on the lower side, then that row/column has more probability of containing material IDs. For Figure \ref{fig:nom_exp_table}, $f_1^{(r)} = 6$, $f_2^{(r)} = 2$, and $f_3^{(r)} = 3$. This is because we copy the cell contents in case of merged cells. We also set $f_0^{(r)} = f_0^{(c)} = 0$. These numbers are then mapped to learnable embeddings $(\overrightarrow{q_m}'s)$ and concatenated with $\overrightarrow{x_{ij}}$. Hence, $\overrightarrow{z_{ij}} = (\overrightarrow{x_{ij}} + \overrightarrow{p_i}) + \overrightarrow{p_j}) \; || \; (\overrightarrow{q_{f_{i}^{(r)}}} + \overrightarrow{q_{f_{j}^{(c)}}})$. Here, we take $\overrightarrow{q_{m}} = \overrightarrow{q_m'}$ for all $m > m'$ and $m'$ is a hyper-parameter. Size of $\overrightarrow{q_m}'s$ is also a hyper-parameter.
    
%    \item \textit{Boolean Regex Feature}: We use this feature while classifying Single-cell composition tables. The feature is set to true for a table cell if that cell contains a composition that can be parsed using any of our regular expressions. We map true and false to different embeddings and concatenate them with $\overrightarrow{x_{ij}}'s$ to obtain new $\overrightarrow{z_{ij}}'s$.

%\end{enumerate}

%\subsubsection{Caption node}
%Sometimes, table captions can be useful to differentiate composition tables from non-composition tables. Therefore, we add a node in the graph corresponding to table caption for Multi-cell composition tables. We represent the caption node by $(0, 0)$ and add edges from caption node to all row and column nodes. To propagate the information further to table cells, edges are added from row and column nodes to corresponding table cell nodes.


==> sections_old_v3/5_experiments.tex <==
% !TEX root = main.tex
\section{Experiments} 
\label{sec:experiments}
%\subsection{Dataset}
%\begin{wraptable}{R}{0.4\textwidth}
%\vspace{-0.15in}
%\centering
%\caption{\small Statistics of table types in all three splits}
%\begin{tabular}{lccc}
%    \toprule &
%    \multicolumn{3}{c}{ \textbf{Splits}}\\
%    \cmidrule(lr){2-4}
%    \textbf{Table Type} &  \textbf{Train} & \textbf{Dev} & \textbf{Test} \\
%    \midrule
%    SCC & 704 & 110 & 113 \\
%    MCC-CI & 626 & 132 & 132 \\
%    MCC-PI & 317 & 109 & 112 \\
%    NC & 2761 & 387 & 380 \\
%    \midrule
%    Total & 4408 & 738 & 737 \\
%    \bottomrule
%\end{tabular}
%\label{tab:dataset_stats}
%\vspace{-0.2in}
%\end{wraptable}
% \textbf{Dataset construction:} % moved to appendix
% \textbf{Dataset details:} We match a manually-curated KB of materials and compositions with tables in the relevant papers, to automatically provide distantly-supervised labels for extraction (hand-annotated for dev/test sets). This results in 5,883 tables from 2536 publications, of which 2,355 express compositions, with 16,729 materials, and a total of 58,481 (material ID, constituent, composition percentage, unit) tuples.\\

\textbf{Baseline models: }
% We implement \sys\ with $LM$ as \textsc{MatSciBERT} \cite{gupta_matscibert_2022}, and the GNNs as Graph Attention Networks \cite{velickovic2018graph}. We compare \sys\ with six non-GNN baseline models. Our first baseline is \textsc{TaPas} \cite{herzig-etal-2020-tapas}, a state-of-the-art table QA system, which flattens the table, adds row and column index embeddings, and passes as input to a language model. To use TaPas for our task, we use table caption as proxy for the input question. All the model parameters in this setting are initialized randomly. Our second baseline is \textsc{TaPas-Adapted}, with the goal of providing the benefit of \textsc{MatSciBERT} to  \textsc{TaPas} -- it initializes language model weights by \textsc{MatSciBERT}. For the input to remain consistent with \textsc{MatSciBERT}, we add row and column index embeddings to \textsc{MatSciBERT} \emph{output}, instead of input as in original \textsc{TaPas} model. The third baseline model is \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation. Similar to \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} uses \textsc{MatSciBERT} as the LM instead of \textsc{BERT}. 
% \tabltextcolor{red}{We use TABBIE as our fifth baseline model, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. It's architecture mainly consists of two transformers that independently encode information across rows and columns and their representations are pooled after each layer for getting the overall table information. Likewise, \textsc{TABBIE-ADAPTED} uses \textsc{MatSciBERT} as the LM}. 
% Further details on baselines in App.~\ref{app:baseline}.
We implement \sys\ with $LM$ as \textsc{MatSciBERT} \cite{gupta_matscibert_2022}, and the GNNs as Graph Attention Networks \cite{velickovic2018graph}. We compare \sys\ with six non-GNN baseline models. Our first baseline is \textsc{TaPas} \cite{herzig-etal-2020-tapas}, a state-of-the-art table QA system, which flattens the table, adds row and column index embeddings, and passes as input to a language model. To use TaPas for our task, we use table caption as proxy for the input question. All the model parameters in this setting are initialized randomly. 
Next, we use \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation.
Finally, we use \textsc{TABBIE}, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. 
% It's architecture consists of two transformers that independently encode information across rows and columns after which representations are pooled at each layer.
Additionally, we replace the LM of all models with \textsc{MatSciBERT} to provide domain specific embeddings to obtain the respective \textsc{Adapted} versions. Further details on baselines in App.~\ref{app:baseline}.
% \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} and \textsc{TABBIE-Adapted} with the goal of providing the benefit of \textsc{MatSciBERT} to  \textsc{TaPas} -- it initializes language model weights by \textsc{MatSciBERT}. For the input to remain consistent with \textsc{MatSciBERT}, we add row and column index embeddings to \textsc{MatSciBERT} \emph{output}, instead of input as in original \textsc{TaPas} model. 
% The third baseline model is \textsc{TaBERT} \cite{yin-etal-2020-tabert}, which is a pretrained LM that jointly learns representations for natural (NL) sentences and tables by using pretraining objectives of masked column prediction (MCP) and cell value recovery (CVR). It finds table cell embeddings by passing row linearizations concatenated with the NL sentence into a language model and then applying vertical attention across columns for information propagation. Similar to \textsc{TaPas-Adapted}, \textsc{TaBERT-Adapted} uses \textsc{MatSciBERT} as the LM instead of \textsc{BERT}. 
% \textcolor{red}{We use TABBIE as our fifth baseline model, which is pretrained by corrupt cell detection and learns exclusively from tabular data without any associated text, unlike the previous baselines. It's architecture mainly consists of two transformers that independently encode information across rows and columns and their representations are pooled after each layer for getting the overall table information. Likewise, \textsc{TABBIE-ADAPTED} uses \textsc{MatSciBERT} as the LM}. 
% Further details on baselines in App.~\ref{app:baseline}.



%{$\bullet$ \bf \textsc{TaPas}:} This has the same architecture as proposed by Herzig et al. \cite{herzig-etal-2020-tapas} for Table-QA task. Here, row and column index embeddings are passed as input to $LM$. All the model parameters are initialized randomly. We use table caption as a proxy for the input question.\\
%{\bf $\bullet$ \textsc{TaPas-Adapted}:} Here, we initialize \textsc{TaPas} with $LM$ pre-trained weights for a fair comparison with \sys. Also, for the input to remain consistent with the original $LM$, we add row and column index embeddings to the $LM$ output and we do not include caption in the input. We term this modified model as \textsc{TaPas-Adapted}. 

%The input table is flattened row-wise and passed through these two baseline models. We provide the precise details in Appendix.

\begin{table*}[htb]
\centering
\scalebox{0.85}{
\begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} &  \textbf{CV} \\
    \midrule
    
    \textsc{TaPas} & 80.37 ($\pm$ 4.78) & 71.23 ($\pm$ 0.77) & 49.88 ($\pm$ 0.10) & 543.67 \\
    \textsc{TaPas-Adapted} & \textbf{89.65} ($\pm$ 0.46) & 70.91 ($\pm$ 3.79) & 57.88 ($\pm$ 2.73) & 490.33 \\
    \textsc{TaBERT} & 79.61 ($\pm$ 8.25) & 58.20 ($\pm$ 1.79) & 47.05 ($\pm$ 1.50) & 1729.67 \\
    \textsc{TaBERT-Adapted} & 85.07 ($\pm$ 6.28) & 59.31 ($\pm$ 0.67) & 50.10 ($\pm$ 2.86) & 1195.67 \\
    \textsc{TABBIE} & 80.99 ($\pm$ 2.41) & 50.90 ($\pm$ 3.34) & 47.03 ($\pm$ 2.14) & \textbf{388.00} \\
    \textsc{TABBIE-Adapted} & 80.18 ($\pm$ 5.38) & 53.20 ($\pm$ 5.57) & 48.89 ($\pm$ 2.73) & 728.67 \\
    % \textsc{TaPas-Adapted} & 86.80 ($\pm$ 0.50) & 70.43 ($\pm$ 2.01) & 56.67 ($\pm$ 4.67) & 424.33 \\
    % \textsc{Rule Based System} & 72.64 & 54.44 & 47.38 & 0 \\
    \textsc{v-}\sys & 77.38 ($\pm$ 12.21) & \textbf{76.52} ($\pm$ 2.37) & \textbf{64.71} ($\pm$ 3.45) & 626.33 \\
    \bottomrule
\end{tabular}
}
\caption{Performance of \textsc{v-}\sys{} vs baseline models on MCC-CI and NC table types. Refer to Evaluation metrics (Section 5) for detailed  definitions of these metrics.}
\label{tab:baselines}
\vspace{-0.10cm}
\end{table*}

% \begin{table*}[htb]
% \centering
% %\vspace{-2ex}
% \scalebox{0.85}{
% \begin{tabular}{lccccc}
%     \toprule
%     \textbf{Model} & \textbf{TT Acc.} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
%     \midrule
    
%     \sys & 88.35 ($\pm$ 1.20) & 82.40 ($\pm$ 3.88) & \textbf{70.14} ($\pm$ 0.44) & \textbf{63.51} ($\pm$ 1.90) & 87.33 \\
%     \midrule

% \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 80.80 ($\pm$ 3.24) & 68.60 ($\pm$ 1.26) & 62.53 ($\pm$ 1.89) & 120.11 \\
%     \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 78.71 ($\pm$ 3.66) & 69.28 ($\pm$ 1.11) & 60.94 ($\pm$ 0.98) & 584.78 \\
%     \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.23} ($\pm$ 0.51) & 67.51 ($\pm$ 1.36) & 63.50 ($\pm$ 2.49) & \textbf{19.11} \\
%     \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 68.54 ($\pm$ 9.32) & 65.98 ($\pm$ 1.21) & 59.36 ($\pm$ 2.20) & 541 \\
    
%     \bottomrule
% \end{tabular}
% }
% \caption{Contribution of task specific features and constraints in \sys.}
% \label{tab:ablations}
% \vspace{-0.1in}
% \end{table*}
\begin{table*}[htb]
\centering
%\vspace{-2ex}
\scalebox{0.85}{
\begin{tabular}{lccccc}
    \toprule
    \textbf{Model} & \textbf{TT Acc.} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
    \midrule
    
    % \sys & 88.35 ($\pm$ 1.20) & 82.40 ($\pm$ 3.88) & \textbf{70.14} ($\pm$ 0.44) & \textbf{63.51} ($\pm$ 1.90) & 87.33 \\
    \sys & 88.35 ($\pm$ 1.20) & 84.57 ($\pm$ 2.16) & \textbf{70.04} ($\pm$ 0.69) & \textbf{63.53} ($\pm$ 1.45) & 75.22 \\
    \midrule

    % \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 80.80 ($\pm$ 3.24) & 68.60 ($\pm$ 1.26) & 62.53 ($\pm$ 1.89) & 120.11 \\
    \sys{} w/o features & \textbf{88.84} ($\pm$ 1.00) & 84.15 ($\pm$ 1.61) & 68.31 ($\pm$ 1.45) & 62.47 ($\pm$ 1.98) & 83.11 \\
    % \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 78.71 ($\pm$ 3.66) & 69.28 ($\pm$ 1.11) & 60.94 ($\pm$ 0.98) & 584.78 \\
    \sys{} w/o constraints & 88.47 ($\pm$ 0.31) & 84.07 ($\pm$ 0.83) & 69.68 ($\pm$ 1.21) & 61.44 ($\pm$ 1.00) & 434.44 \\
    % \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.23} ($\pm$ 0.51) & 67.51 ($\pm$ 1.36) & 63.50 ($\pm$ 2.49) & \textbf{19.11} \\
    \sys{} w/o captions & 87.35 ($\pm$ 0.71) & \textbf{84.76} ($\pm$ 0.68) & 66.82 ($\pm$ 1.90) & 62.68 ($\pm$ 3.33) & \textbf{17.89} \\
    % \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 68.54 ($\pm$ 9.32) & 65.98 ($\pm$ 1.21) & 59.36 ($\pm$ 2.20) & 541 \\
    \textsc{v-}\sys & 88.59 ($\pm$ 0.33) & 76.61 ($\pm$ 6.16) & 66.15 ($\pm$ 2.00) & 59.52 ($\pm$ 3.33) & 380.11 \\
    
    \bottomrule
\end{tabular}
}
\caption{Contribution of task specific features and constraints in \sys. Refer to Evaluation metrics (Section 5) for detailed  definitions of these metrics.}
\label{tab:ablations}
\vspace{-0.1in}
\end{table*}

\begin{table}[!htb]
% \vspace{-1.5cm}
\centering
\scalebox{0.75}{
\begin{tabular}{ccccc}
    \toprule
    \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} \\
    \midrule
    
    SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) \\
    
    MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) \\
    
    MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) \\

    \bottomrule
\end{tabular}
}
\caption{\sys{} performance on the table-types.}
\label{tab:perf_table_types}
\vspace{-0.25in}
\end{table}

%\subsection{Evaluation metrics}
\textbf{Evaluation metrics:} 
We compute several metrics in our evaluation. (1) \emph{Table-type (TT) prediction accuracy} -- it computes table-level accuracy on the 4-way table classification as NC, SCC, MCC-CI and MCC-PI. 
(2) \textit{ID F$_1$ score} computes F$_1$ score for Material ID extraction.  
(3) \textit{Tuple-level (TL) F$_1$ score} evaluates performance on the extraction of composition tuples. A gold is considered matching with a predicted 4-tuple if \emph{all} arguments match exactly. 
(4) \textit{Material-level (MatL) F$_1$ score} is the strongest metric. It evaluates whether all predicted information related to a material (including its ID, all constituents and their percentages) match exactly with the gold.
Finally, (5) \textit{constraint violations (CV)} counts the number of violations of hard constraints in the prediction. We consider all four types of constraints, as discussed in Section \ref{sec:constraints}. %\end{enumerate}
%Thus, TL precision means how many, out of all the tuples model predict, are correct. Similarly, TL recall means how many, out of all the gold tuples, were predicted by the model. TL F$_1$ score is the harmonic mean of TL precision and recall.\\
%$\bullet$\textit{Composition-level (CL) metrics}: This set of metrics evaluate model at the composition level. So, CL precision means out of all the compositions (set of tuples) model predict, how many of them were completely correct. Similarly, CL recall means out of all the gold compositions, how many were exactly predicted by the model. CL F$_1$ score is the harmonics mean of CL precision and CL recall.\\  
% \textbf{Implementation details: }
% %In our experiments, we take the $LM$ as MatSciBERT \cite{gupta_matscibert_2022} which is a materials-science domain specific language model and we choose $GNN$ to be 
% For Graph Attention Networks (GATs) \cite{velickovic2018graph}, we use the GAT implementation of Deep Graph Library \cite{dgl_citation_wang2019}. For LMs, \textsc{TaPas}, we use the implementation by Transformers library \cite{transformers_huggingface}. We use \textsc{TaBERT}'s source code from their github repository. We implement and train all models using PyTorch  \cite{pytorch_NEURIPS2019_9015}. We optimize the model parameters using Adam \cite{adam_opt_kingma} and a triangular learning rate \cite{triangle_lr}. We further use different learning rates for $LM$ and non-LM parameters (GNNs, MLPs) (App.~\ref{app:hyperparameter}). To deal with imbalanced labels, we scale loss for all labels by weights inversely proportional to their frequency in the training set. All experiments were run on a machine with one 32 GB V100 GPU. Each model is run with three seeds and the mean and std. deviation are reported. 
Implementation details are mentioned in App.~\ref{app:implementation}. The code and data is available \href{https://anonymous.4open.science/r/DiSCoMaT-EEFB/}{here}.
\vspace{-1ex}
%\vspace{-0.5cm}
\subsection{Results}
%\vspace{-0.2cm}
\emph{How does table linearization compare with a graph-based model for our task?} To answer this question,  we compare \sys{} with four models that use linearization: {\sc TaPas}, \textsc{TaBERT}, and their adapted versions. \textsc{TaPas} and \textsc{TaBERT} do table level and row level linearizations respectively. Since the baselines do not have the benefit of regular expressions, features, and constraints, we implement a version of our model without these, which we call \textsc{v-}\sys. We do this comparison, trained and tested only on the subset of MCC-CI and NC tables, since other table types require regular expressions for processing. As shown in Table \ref{tab:baselines} \textsc{v-}\sys{} obtains 6-7 pt higher F$_1$ on TL and MatL scores, suggesting that a graph-based extractor is likely a better fit for our problem - this led to us choosing a GNN-based approach for \sys. 

%\textsc{TaPas} and \textsc{TaPas-Adapted} as shown in Table \ref{tab:baselines}. For simplicity, we train and evaluate all three models on MCC-CI and NC tables only. We refer to \sys{} without max-frequency feature, constraint loss, and caption node as Vanilla-\sys{} or in short \textsc{V-}\sys.

\emph{How does \sys{} perform on the complete task?}
Table \ref{tab:ablations}, reports \sys{} performance on the full test set with all table types. 
%Here, we have 3 set of parameters for GNN$_1$ and 3 set of parameters for GNN$_2$ corresponding to 3 seeds. Hence, we report results averaged over 9 ordered pair of seeds.
Its ID and tuple F$_1$-scores are 82 and 70, respectively. Since these errors get multiplied, unsurprisingly, its material-level F$_1$-score is lower (63.5). Table \ref{tab:perf_table_types} reports \sys{} performance for different table types. In this experiment, we assume that table type is already known and run only the relevant part of \sys{} for extraction. We find that MCC-PI is the hardest table type, since it requires combining information from text and tables for accurate extraction. A larger standard deviation in ID F$_1$ for MCC-PI is attributed to the fact that material IDs occur relatively rarely for this table type -- the test set for MCC-PI consists of merely 20 material ID rows and columns.

\emph{What is the incremental contribution of task-specific features and constraints?}
Table \ref{tab:ablations} also presents the ablation experiments. \sys{} scores much higher that \textsc{v-}\sys, which does not have these features and constraints. We also perform additional ablations removing one component at a time. Unsurprisingly constrained training helps with reducing constraint violations. Both constraints and features help with ID prediction, due to constraints (2), (3), (4) and max frequency feature. Removal of caption node significantly hurts performance on MCC-PI tables, as these tables require combining caption with table cells. All contribute to the tuple-level metric. 

\emph{What are the typical errors in \sys?} 
Confusion matrix in Figure \ref{fig:confusion} suggests that most table type errors are between MCC-PI and NC tables. This could be attributed to following reasons. (i) \sys{} has difficulty identifying rare compounds like Yb$_2$O$_3$, ErS$_{3/2}$, Co$_3$O$_4$ found in MCC-PI---these aren't present frequently in the training set. (ii) MCC-PI tables specify dopant percentages found in small quantities. %are also a source of error. %Generally the text contains a base composition (summing to 100), in which dopant is added. Finding the base composition in paper text corresponding to dopants mentioned in the table is non-trivial. Sometimes, instead of percentage contributions being expressed as variables, constituents are specified as variables. 
(iii) Completion of composition in MCC-PI tables may require other tables from the same paper. (iv) Finally, MCC-PI composition may contain additional information such as properties that may bias the model to classify it as  NC. Some corner cases are given in App.~\ref{app:corner}. %Yet another case is when caption mentions silicates/phosphates and hence remaining constituent is SiO$_2$/P$_2$O$_5$.
%\vspace{-0.1in}
\begin{wrapfigure}{r}{0.25\textwidth}
    \vspace{-0.1in}
    \centering
    \includegraphics[width=0.25\textwidth]{confusion_matrix.png}
    \vspace{-0.15in}
    \caption{Confusion matrix for all table types}
    \label{fig:confusion}
    \vspace{-0.30in}
\end{wrapfigure}
%Table \ref{tab:perf_table_types} shows the performance of \sys{} (averaged over three seeds) on individual table types. In these experiments, we assume that table type is already known. For SCC, we use GNN$_1$ just for materials ID prediction and Rule-based composition parser to parse compositions from table cells. From CL F$_1$-score, we can observe that \sys performs best on SCC, then MCC-CI, and then MCC-PI. Large standard deviation in Material IDs F$_1$-Score for MCC-PI can be attributed to the fact that Material IDs occur relatively rarely for this table type. Test set for MCC-PI consists of merely 20 Material ID rows and columns.

% \begin{wraptable}{R}{0.6\textwidth}
% \vspace{-1.5cm}
% \centering
% \caption{Performance of \sys{} on different table types}
% \scalebox{0.75}{
% \begin{tabular}{ccccc}
%     \toprule
%     \textbf{Table Type} & \textbf{ID F$_1$} & \textbf{TL F$_1$} & \textbf{MatL F$_1$} & \textbf{CV} \\
%     \midrule
    
%     SCC & 88.81 ($\pm$ 1.54) & 79.89 ($\pm$ 0.18) & 78.21 ($\pm$ 0.14) & 0.67 \\
    
%     MCC-CI & 93.91 ($\pm$ 1.46) & 77.62 ($\pm$ 1.07) & 65.41 ($\pm$ 4.35) & 59.33 \\
    
%     MCC-PI & 70.67 ($\pm$ 11.58) & 50.60 ($\pm$ 2.59) & 51.66 ($\pm$ 2.21) & 26.67 \\

%     \bottomrule
% \end{tabular}
% }
% \label{tab:perf_table_types}
% % \vspace{-0.2cm}
% \end{wraptable}


==> sections_old_v3/6_conclusions.tex <==
\vspace{-0.25cm}
\section{Conclusions} 
\label{sec:conclusions}
\vspace{-0.15cm}
We define the novel task of extracting material compositions from tables in scientific papers. We harvest a dataset using distant supervision, combining information from a MatSci DB with tables in respective papers. We present a strong baseline system, \sys, a pipeline based on LM, GNNs, and task-specific regex, %, which is a pipeline of a material science language model, two graph neural networks along with task-specific regular expressions, features and constraints. Our experiments show 
that outperforms other architectures that linearizes the tables. We plan to extend it to extract material properties as well. \\
\textbf{Limitations and outlook:} \sys\ is a pipelined solution trained component-wise. This raises a research question: can we train one end-to-end trained ML model that not only analyzes a wide variety of table structures, but also combines understanding of regular expressions, extraction of chemical compounds and scientific units, text understanding and some mathematical processing. This defines a challenging ML research question, and one that can have direct impact to the scientific MatSci community. \\
Indeed, automating parts of scientific discovery through such NLP-based approaches has the potential of biases and errors. Note that wrong and biased results can lead to erroneous information about materials. To a great extent this issue is addressed as we rely only on published literature. The issue could be further addresses by considering larger datasets covering wider range of materials.

==> sections_old_v3/7_acknowledgements.tex <==
\section*{Acknowledgements}
\label{sec:checklist}

% This document has been adapted
% by Steven Bethard, Ryan Cotterell and Rui Yan
% from the instructions for earlier ACL and NAACL proceedings, including those for 
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan, 
% NAACL 2017 by Margaret Mitchell, 
% ACL 2012 by Maggie Li and Michael White, 
% ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
% ACL 2002 by Eugene Charniak and Dekang Lin, 
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> sections_old_v3/7_checklist.tex <==
% !TEX root = main.tex
\section*{Checklist}
\label{sec:checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

